Planck 2013 results. XXIII. Isotropy and statistics of the CMB

The two fundamental assumptions of the standard cosmological model - that the initial fluctuations are statistically isotropic and Gaussian - are rigorously tested using maps of the cosmic microwave background (CMB) anisotropy from the Planck satellite. Deviations from isotropy have been found and demonstrated to be robust against component separation algorithm, mask choice and frequency dependence. Many of these anomalies were previously observed in the WMAP data, and are now confirmed at similar levels of significance (about 3 sigma). However, we find little evidence for non-Gaussianity, with the exception of a few statistical signatures that seem to be associated with specific anomalies. In particular, we find that the quadrupole-octopole alignment is also connected to a low observed variance of the CMB signal. A power asymmetry is now found to persist to scales corresponding to about l=600, and can be described in the low-l regime by a phenomenological dipole modulation model. However, any primordial power asymmetry is strongly scale-dependent and does not extend to arbitrarily small angular scales. Finally, it is plausible that some of these features may be reflected in the angular power spectrum of the data, which shows a deficit of power on similar scales. Indeed, when the power spectra of two hemispheres defined by a preferred direction are considered separately, one shows evidence for a deficit in power, while its opposite contains oscillations between odd and even modes that may be related to the parity violation and phase correlations also detected in the data. Although these analyses represent a step forward in building an understanding of the anomalies, a satisfactory explanation based on physically motivated models is still lacking.

==> AuthorList_P09_Isotropy_and_Statistics_authors_and_institutes.tex <==
%This author list corresponds to \title{Author list for SVN P09\_Isotropy\_and\_Statistics, Proj. Ref. 2\_1: Constraints from Planck data on the Isotropy and statistics of the CMB}
%Prepared by R. Leonardi (rleonardi@sciops.esa.int), ESAC/ESA
%This version is from Thu Dec 19 11:47:26 2013 CET
%\subtitle{There are 254 co-authors in this list}
\author{\small
Planck Collaboration:
P.~A.~R.~Ade\inst{92}
\and
N.~Aghanim\inst{63}
\and
C.~Armitage-Caplan\inst{97}
\and
M.~Arnaud\inst{76}
\and
M.~Ashdown\inst{73, 6}
\and
F.~Atrio-Barandela\inst{18}
\and
J.~Aumont\inst{63}
\and
C.~Baccigalupi\inst{91}
\and
A.~J.~Banday\inst{100, 9}
\and
R.~B.~Barreiro\inst{70}
\and
J.~G.~Bartlett\inst{1, 71}
\and
N.~Bartolo\inst{35}
\and
E.~Battaner\inst{101}
\and
R.~Battye\inst{72}
\and
K.~Benabed\inst{64, 99}
\and
A.~Beno\^{\i}t\inst{61}
\and
A.~Benoit-L\'{e}vy\inst{26, 64, 99}
\and
J.-P.~Bernard\inst{100, 9}
\and
M.~Bersanelli\inst{39, 53}
\and
P.~Bielewicz\inst{100, 9, 91}
\and
J.~Bobin\inst{76}
\and
J.~J.~Bock\inst{71, 10}
\and
A.~Bonaldi\inst{72}
\and
L.~Bonavera\inst{70}
\and
J.~R.~Bond\inst{8}
\and
J.~Borrill\inst{13, 94}
\and
F.~R.~Bouchet\inst{64, 99}
\and
M.~Bridges\inst{73, 6, 67}
\and
M.~Bucher\inst{1}
\and
C.~Burigana\inst{52, 37}
\and
R.~C.~Butler\inst{52}
\and
J.-F.~Cardoso\inst{77, 1, 64}
\and
A.~Catalano\inst{78, 75}
\and
A.~Challinor\inst{67, 73, 11}
\and
A.~Chamballu\inst{76, 15, 63}
\and
R.-R.~Chary\inst{60}
\and
H.~C.~Chiang\inst{29, 7}
\and
L.-Y~Chiang\inst{66}
\and
P.~R.~Christensen\inst{87, 43}
\and
S.~Church\inst{96}
\and
D.~L.~Clements\inst{59}
\and
S.~Colombi\inst{64, 99}
\and
L.~P.~L.~Colombo\inst{25, 71}
\and
F.~Couchot\inst{74}
\and
A.~Coulais\inst{75}
\and
B.~P.~Crill\inst{71, 88}
\and
M.~Cruz\inst{20}
\and
A.~Curto\inst{6, 70}
\and
F.~Cuttaia\inst{52}
\and
L.~Danese\inst{91}
\and
R.~D.~Davies\inst{72}
\and
R.~J.~Davis\inst{72}
\and
P.~de Bernardis\inst{38}
\and
A.~de Rosa\inst{52}
\and
G.~de Zotti\inst{48, 91}
\and
J.~Delabrouille\inst{1}
\and
J.-M.~Delouis\inst{64, 99}
\and
F.-X.~D\'{e}sert\inst{56}
\and
J.~M.~Diego\inst{70}
\and
H.~Dole\inst{63, 62}
\and
S.~Donzelli\inst{53}
\and
O.~Dor\'{e}\inst{71, 10}
\and
M.~Douspis\inst{63}
\and
A.~Ducout\inst{64}
\and
X.~Dupac\inst{45}
\and
G.~Efstathiou\inst{67}
\and
F.~Elsner\inst{64, 99}
\and
T.~A.~En{\ss}lin\inst{81}
\and
H.~K.~Eriksen\inst{68}
\and
Y.~Fantaye\inst{68}
\and
J.~Fergusson\inst{11}
\and
F.~Finelli\inst{52, 54}
\and
O.~Forni\inst{100, 9}
\and
M.~Frailis\inst{50}
\and
E.~Franceschi\inst{52}
\and
M.~Frommert\inst{17}
\and
S.~Galeotta\inst{50}
\and
K.~Ganga\inst{1}
\and
M.~Giard\inst{100, 9}
\and
G.~Giardino\inst{46}
\and
Y.~Giraud-H\'{e}raud\inst{1}
\and
J.~Gonz\'{a}lez-Nuevo\inst{70, 91}
\and
K.~M.~G\'{o}rski\inst{71, 102}
\and
S.~Gratton\inst{73, 67}
\and
A.~Gregorio\inst{40, 50}
\and
A.~Gruppuso\inst{52}
\and
F.~K.~Hansen\inst{68}
\and
M.~Hansen\inst{87}
\and
D.~Hanson\inst{83, 71, 8}
\and
D.~L.~Harrison\inst{67, 73}
\and
G.~Helou\inst{10}
\and
S.~Henrot-Versill\'{e}\inst{74}
\and
C.~Hern\'{a}ndez-Monteagudo\inst{12, 81}
\and
D.~Herranz\inst{70}
\and
S.~R.~Hildebrandt\inst{10}
\and
E.~Hivon\inst{64, 99}
\and
M.~Hobson\inst{6}
\and
W.~A.~Holmes\inst{71}
\and
A.~Hornstrup\inst{16}
\and
W.~Hovest\inst{81}
\and
K.~M.~Huffenberger\inst{27}
\and
A.~H.~Jaffe\inst{59}
\and
T.~R.~Jaffe\inst{100, 9}
\and
W.~C.~Jones\inst{29}
\and
M.~Juvela\inst{28}
\and
E.~Keih\"{a}nen\inst{28}
\and
R.~Keskitalo\inst{23, 13}
\and
J.~Kim\inst{87}
\and
T.~S.~Kisner\inst{80}
\and
J.~Knoche\inst{81}
\and
L.~Knox\inst{32}
\and
M.~Kunz\inst{17, 63, 3}
\and
H.~Kurki-Suonio\inst{28, 47}
\and
G.~Lagache\inst{63}
\and
A.~L\"{a}hteenm\"{a}ki\inst{2, 47}
\and
J.-M.~Lamarre\inst{75}
\and
A.~Lasenby\inst{6, 73}
\and
R.~J.~Laureijs\inst{46}
\and
C.~R.~Lawrence\inst{71}
\and
J.~P.~Leahy\inst{72}
\and
R.~Leonardi\inst{45}
\and
C.~Leroy\inst{63, 100, 9}
\and
J.~Lesgourgues\inst{98, 90}
\and
M.~Liguori\inst{35}
\and
P.~B.~Lilje\inst{68}
\and
M.~Linden-V{\o}rnle\inst{16}
\and
M.~L\'{o}pez-Caniego\inst{70}
\and
P.~M.~Lubin\inst{33}
\and
J.~F.~Mac\'{\i}as-P\'{e}rez\inst{78}
\and
B.~Maffei\inst{72}
\and
D.~Maino\inst{39, 53}
\and
N.~Mandolesi\inst{52, 5, 37}
\and
A.~Mangilli\inst{64}
\and
D.~Marinucci\inst{42}
\and
M.~Maris\inst{50}
\and
D.~J.~Marshall\inst{76}
\and
P.~G.~Martin\inst{8}
\and
E.~Mart\'{\i}nez-Gonz\'{a}lez\inst{70}
\and
S.~Masi\inst{38}
\and
M.~Massardi\inst{51}
\and
S.~Matarrese\inst{35}
\and
F.~Matthai\inst{81}
\and
P.~Mazzotta\inst{41}
\and
J.~D.~McEwen\inst{26, 85}
\and
P.~R.~Meinhold\inst{33}
\and
A.~Melchiorri\inst{38, 55}
\and
L.~Mendes\inst{45}
\and
A.~Mennella\inst{39, 53}
\and
M.~Migliaccio\inst{67, 73}
\and
K.~Mikkelsen\inst{68}
\and
S.~Mitra\inst{58, 71}
\and
M.-A.~Miville-Desch\^{e}nes\inst{63, 8}
\and
D.~Molinari\inst{36, 52}
\and
A.~Moneti\inst{64}
\and
L.~Montier\inst{100, 9}
\and
G.~Morgante\inst{52}
\and
D.~Mortlock\inst{59}
\and
A.~Moss\inst{93}
\and
D.~Munshi\inst{92}
\and
J.~A.~Murphy\inst{86}
\and
P.~Naselsky\inst{87, 43}
\and
F.~Nati\inst{38}
\and
P.~Natoli\inst{37, 4, 52}
\and
C.~B.~Netterfield\inst{21}
\and
H.~U.~N{\o}rgaard-Nielsen\inst{16}
\and
F.~Noviello\inst{72}
\and
D.~Novikov\inst{59}
\and
I.~Novikov\inst{87}
\and
S.~Osborne\inst{96}
\and
C.~A.~Oxborrow\inst{16}
\and
F.~Paci\inst{91}
\and
L.~Pagano\inst{38, 55}
\and
F.~Pajot\inst{63}
\and
D.~Paoletti\inst{52, 54}
\and
F.~Pasian\inst{50}
\and
G.~Patanchon\inst{1}
\and
H.~V.~Peiris\inst{26}
\and
O.~Perdereau\inst{74}
\and
L.~Perotto\inst{78}
\and
F.~Perrotta\inst{91}
\and
F.~Piacentini\inst{38}
\and
M.~Piat\inst{1}
\and
E.~Pierpaoli\inst{25}
\and
D.~Pietrobon\inst{71}
\and
S.~Plaszczynski\inst{74}
\and
D.~Pogosyan\inst{30}
\and
E.~Pointecouteau\inst{100, 9}
\and
G.~Polenta\inst{4, 49}
\and
N.~Ponthieu\inst{63, 56}
\and
L.~Popa\inst{65}
\and
T.~Poutanen\inst{47, 28, 2}
\and
G.~W.~Pratt\inst{76}
\and
G.~Pr\'{e}zeau\inst{10, 71}
\and
S.~Prunet\inst{64, 99}
\and
J.-L.~Puget\inst{63}
\and
J.~P.~Rachen\inst{22, 81}
\and
B.~Racine\inst{1}
\and
C.~R\"{a}th\inst{82}
\and
R.~Rebolo\inst{69, 14, 44}
\and
M.~Reinecke\inst{81}
\and
M.~Remazeilles\inst{72, 63, 1}
\and
C.~Renault\inst{78}
\and
A.~Renzi\inst{91}
\and
S.~Ricciardi\inst{52}
\and
T.~Riller\inst{81}
\and
I.~Ristorcelli\inst{100, 9}
\and
G.~Rocha\inst{71, 10}
\and
C.~Rosset\inst{1}
\and
A.~Rotti\inst{58}
\and
G.~Roudier\inst{1, 75, 71}
\and
J.~A.~Rubi\~{n}o-Mart\'{\i}n\inst{69, 44}
\and
B.~Ruiz-Granados\inst{101}
\and
B.~Rusholme\inst{60}
\and
M.~Sandri\inst{52}
\and
D.~Santos\inst{78}
\and
G.~Savini\inst{89}
\and
D.~Scott\inst{24}
\and
M.~D.~Seiffert\inst{71, 10}
\and
E.~P.~S.~Shellard\inst{11}
\and
T.~Souradeep\inst{58}
\and
L.~D.~Spencer\inst{92}
\and
J.-L.~Starck\inst{76}
\and
V.~Stolyarov\inst{6, 73, 95}
\and
R.~Stompor\inst{1}
\and
R.~Sudiwala\inst{92}
\and
F.~Sureau\inst{76}
\and
P.~Sutter\inst{64}
\and
D.~Sutton\inst{67, 73}
\and
A.-S.~Suur-Uski\inst{28, 47}
\and
J.-F.~Sygnet\inst{64}
\and
J.~A.~Tauber\inst{46}
\and
D.~Tavagnacco\inst{50, 40}
\and
L.~Terenzi\inst{52}
\and
L.~Toffolatti\inst{19, 70}
\and
M.~Tomasi\inst{53}
\and
M.~Tristram\inst{74}
\and
M.~Tucci\inst{17, 74}
\and
J.~Tuovinen\inst{84}
\and
M.~T\"{u}rler\inst{57}
\and
L.~Valenziano\inst{52}
\and
J.~Valiviita\inst{47, 28, 68}
\and
B.~Van Tent\inst{79}
\and
J.~Varis\inst{84}
\and
P.~Vielva\inst{70}
\and
F.~Villa\inst{52}
\and
N.~Vittorio\inst{41}
\and
L.~A.~Wade\inst{71}
\and
B.~D.~Wandelt\inst{64, 99, 34}
\and
I.~K.~Wehus\inst{71}
\and
M.~White\inst{31}
\and
A.~Wilkinson\inst{72}
\and
D.~Yvon\inst{15}
\and
A.~Zacchei\inst{50}
\and
A.~Zonca\inst{33}
}
\institute{\small
APC, AstroParticule et Cosmologie, Universit\'{e} Paris Diderot, CNRS/IN2P3, CEA/lrfu, Observatoire de Paris, Sorbonne Paris Cit\'{e}, 10, rue Alice Domon et L\'{e}onie Duquet, 75205 Paris Cedex 13, France\\
\and
Aalto University Mets\"{a}hovi Radio Observatory and Dept of Radio Science and Engineering, P.O. Box 13000, FI-00076 AALTO, Finland\\
\and
African Institute for Mathematical Sciences, 6-8 Melrose Road, Muizenberg, Cape Town, South Africa\\
\and
Agenzia Spaziale Italiana Science Data Center, Via del Politecnico snc, 00133, Roma, Italy\\
\and
Agenzia Spaziale Italiana, Viale Liegi 26, Roma, Italy\\
\and
Astrophysics Group, Cavendish Laboratory, University of Cambridge, J J Thomson Avenue, Cambridge CB3 0HE, U.K.\\
\and
Astrophysics \& Cosmology Research Unit, School of Mathematics, Statistics \& Computer Science, University of KwaZulu-Natal, Westville Campus, Private Bag X54001, Durban 4000, South Africa\\
\and
CITA, University of Toronto, 60 St. George St., Toronto, ON M5S 3H8, Canada\\
\and
CNRS, IRAP, 9 Av. colonel Roche, BP 44346, F-31028 Toulouse cedex 4, France\\
\and
California Institute of Technology, Pasadena, California, U.S.A.\\
\and
Centre for Theoretical Cosmology, DAMTP, University of Cambridge, Wilberforce Road, Cambridge CB3 0WA, U.K.\\
\and
Centro de Estudios de F\'{i}sica del Cosmos de Arag\'{o}n (CEFCA), Plaza San Juan, 1, planta 2, E-44001, Teruel, Spain\\
\and
Computational Cosmology Center, Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.\\
\and
Consejo Superior de Investigaciones Cient\'{\i}ficas (CSIC), Madrid, Spain\\
\and
DSM/Irfu/SPP, CEA-Saclay, F-91191 Gif-sur-Yvette Cedex, France\\
\and
DTU Space, National Space Institute, Technical University of Denmark, Elektrovej 327, DK-2800 Kgs. Lyngby, Denmark\\
\and
D\'{e}partement de Physique Th\'{e}orique, Universit\'{e} de Gen\`{e}ve, 24, Quai E. Ansermet,1211 Gen\`{e}ve 4, Switzerland\\
\and
Departamento de F\'{\i}sica Fundamental, Facultad de Ciencias, Universidad de Salamanca, 37008 Salamanca, Spain\\
\and
Departamento de F\'{\i}sica, Universidad de Oviedo, Avda. Calvo Sotelo s/n, Oviedo, Spain\\
\and
Departamento de Matem\'{a}ticas, Estad\'{\i}stica y Computaci\'{o}n, Universidad de Cantabria, Avda. de los Castros s/n, Santander, Spain\\
\and
Department of Astronomy and Astrophysics, University of Toronto, 50 Saint George Street, Toronto, Ontario, Canada\\
\and
Department of Astrophysics/IMAPP, Radboud University Nijmegen, P.O. Box 9010, 6500 GL Nijmegen, The Netherlands\\
\and
Department of Electrical Engineering and Computer Sciences, University of California, Berkeley, California, U.S.A.\\
\and
Department of Physics \& Astronomy, University of British Columbia, 6224 Agricultural Road, Vancouver, British Columbia, Canada\\
\and
Department of Physics and Astronomy, Dana and David Dornsife College of Letter, Arts and Sciences, University of Southern California, Los Angeles, CA 90089, U.S.A.\\
\and
Department of Physics and Astronomy, University College London, London WC1E 6BT, U.K.\\
\and
Department of Physics, Florida State University, Keen Physics Building, 77 Chieftan Way, Tallahassee, Florida, U.S.A.\\
\and
Department of Physics, Gustaf H\"{a}llstr\"{o}min katu 2a, University of Helsinki, Helsinki, Finland\\
\and
Department of Physics, Princeton University, Princeton, New Jersey, U.S.A.\\
\and
Department of Physics, University of Alberta, 11322-89 Avenue, Edmonton, Alberta, T6G 2G7, Canada\\
\and
Department of Physics, University of California, Berkeley, California, U.S.A.\\
\and
Department of Physics, University of California, One Shields Avenue, Davis, California, U.S.A.\\
\and
Department of Physics, University of California, Santa Barbara, California, U.S.A.\\
\and
Department of Physics, University of Illinois at Urbana-Champaign, 1110 West Green Street, Urbana, Illinois, U.S.A.\\
\and
Dipartimento di Fisica e Astronomia G. Galilei, Universit\`{a} degli Studi di Padova, via Marzolo 8, 35131 Padova, Italy\\
\and
Dipartimento di Fisica e Astronomia, Universit\`{a} degli Studi di Bologna, viale Berti Pichat 6/2, I-40127, Bologna, Italy\\
\and
Dipartimento di Fisica e Scienze della Terra, Universit\`{a} di Ferrara, Via Saragat 1, 44122 Ferrara, Italy\\
\and
Dipartimento di Fisica, Universit\`{a} La Sapienza, P. le A. Moro 2, Roma, Italy\\
\and
Dipartimento di Fisica, Universit\`{a} degli Studi di Milano, Via Celoria, 16, Milano, Italy\\
\and
Dipartimento di Fisica, Universit\`{a} degli Studi di Trieste, via A. Valerio 2, Trieste, Italy\\
\and
Dipartimento di Fisica, Universit\`{a} di Roma Tor Vergata, Via della Ricerca Scientifica, 1, Roma, Italy\\
\and
Dipartimento di Matematica, Universit\`{a} di Roma Tor Vergata, Via della Ricerca Scientifica, 1, Roma, Italy\\
\and
Discovery Center, Niels Bohr Institute, Blegdamsvej 17, Copenhagen, Denmark\\
\and
Dpto. Astrof\'{i}sica, Universidad de La Laguna (ULL), E-38206 La Laguna, Tenerife, Spain\\
\and
European Space Agency, ESAC, Planck Science Office, Camino bajo del Castillo, s/n, Urbanizaci\'{o}n Villafranca del Castillo, Villanueva de la Ca\~{n}ada, Madrid, Spain\\
\and
European Space Agency, ESTEC, Keplerlaan 1, 2201 AZ Noordwijk, The Netherlands\\
\and
Helsinki Institute of Physics, Gustaf H\"{a}llstr\"{o}min katu 2, University of Helsinki, Helsinki, Finland\\
\and
INAF - Osservatorio Astronomico di Padova, Vicolo dell'Osservatorio 5, Padova, Italy\\
\and
INAF - Osservatorio Astronomico di Roma, via di Frascati 33, Monte Porzio Catone, Italy\\
\and
INAF - Osservatorio Astronomico di Trieste, Via G.B. Tiepolo 11, Trieste, Italy\\
\and
INAF Istituto di Radioastronomia, Via P. Gobetti 101, 40129 Bologna, Italy\\
\and
INAF/IASF Bologna, Via Gobetti 101, Bologna, Italy\\
\and
INAF/IASF Milano, Via E. Bassini 15, Milano, Italy\\
\and
INFN, Sezione di Bologna, Via Irnerio 46, I-40126, Bologna, Italy\\
\and
INFN, Sezione di Roma 1, Universit\`{a} di Roma Sapienza, Piazzale Aldo Moro 2, 00185, Roma, Italy\\
\and
IPAG: Institut de Plan\'{e}tologie et d'Astrophysique de Grenoble, Universit\'{e} Joseph Fourier, Grenoble 1 / CNRS-INSU, UMR 5274, Grenoble, F-38041, France\\
\and
ISDC Data Centre for Astrophysics, University of Geneva, ch. d'Ecogia 16, Versoix, Switzerland\\
\and
IUCAA, Post Bag 4, Ganeshkhind, Pune University Campus, Pune 411 007, India\\
\and
Imperial College London, Astrophysics group, Blackett Laboratory, Prince Consort Road, London, SW7 2AZ, U.K.\\
\and
Infrared Processing and Analysis Center, California Institute of Technology, Pasadena, CA 91125, U.S.A.\\
\and
Institut N\'{e}el, CNRS, Universit\'{e} Joseph Fourier Grenoble I, 25 rue des Martyrs, Grenoble, France\\
\and
Institut Universitaire de France, 103, bd Saint-Michel, 75005, Paris, France\\
\and
Institut d'Astrophysique Spatiale, CNRS (UMR8617) Universit\'{e} Paris-Sud 11, B\^{a}timent 121, Orsay, France\\
\and
Institut d'Astrophysique de Paris, CNRS (UMR7095), 98 bis Boulevard Arago, F-75014, Paris, France\\
\and
Institute for Space Sciences, Bucharest-Magurale, Romania\\
\and
Institute of Astronomy and Astrophysics, Academia Sinica, Taipei, Taiwan\\
\and
Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, U.K.\\
\and
Institute of Theoretical Astrophysics, University of Oslo, Blindern, Oslo, Norway\\
\and
Instituto de Astrof\'{\i}sica de Canarias, C/V\'{\i}a L\'{a}ctea s/n, La Laguna, Tenerife, Spain\\
\and
Instituto de F\'{\i}sica de Cantabria (CSIC-Universidad de Cantabria), Avda. de los Castros s/n, Santander, Spain\\
\and
Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, California, U.S.A.\\
\and
Jodrell Bank Centre for Astrophysics, Alan Turing Building, School of Physics and Astronomy, The University of Manchester, Oxford Road, Manchester, M13 9PL, U.K.\\
\and
Kavli Institute for Cosmology Cambridge, Madingley Road, Cambridge, CB3 0HA, U.K.\\
\and
LAL, Universit\'{e} Paris-Sud, CNRS/IN2P3, Orsay, France\\
\and
LERMA, CNRS, Observatoire de Paris, 61 Avenue de l'Observatoire, Paris, France\\
\and
Laboratoire AIM, IRFU/Service d'Astrophysique - CEA/DSM - CNRS - Universit\'{e} Paris Diderot, B\^{a}t. 709, CEA-Saclay, F-91191 Gif-sur-Yvette Cedex, France\\
\and
Laboratoire Traitement et Communication de l'Information, CNRS (UMR 5141) and T\'{e}l\'{e}com ParisTech, 46 rue Barrault F-75634 Paris Cedex 13, France\\
\and
Laboratoire de Physique Subatomique et de Cosmologie, Universit\'{e} Joseph Fourier Grenoble I, CNRS/IN2P3, Institut National Polytechnique de Grenoble, 53 rue des Martyrs, 38026 Grenoble cedex, France\\
\and
Laboratoire de Physique Th\'{e}orique, Universit\'{e} Paris-Sud 11 \& CNRS, B\^{a}timent 210, 91405 Orsay, France\\
\and
Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.\\
\and
Max-Planck-Institut f\"{u}r Astrophysik, Karl-Schwarzschild-Str. 1, 85741 Garching, Germany\\
\and
Max-Planck-Institut f\"{u}r Extraterrestrische Physik, Giessenbachstra{\ss}e, 85748 Garching, Germany\\
\and
McGill Physics, Ernest Rutherford Physics Building, McGill University, 3600 rue University, Montr\'{e}al, QC, H3A 2T8, Canada\\
\and
MilliLab, VTT Technical Research Centre of Finland, Tietotie 3, Espoo, Finland\\
\and
Mullard Space Science Laboratory, University College London, Surrey RH5 6NT, U.K.\\
\and
National University of Ireland, Department of Experimental Physics, Maynooth, Co. Kildare, Ireland\\
\and
Niels Bohr Institute, Blegdamsvej 17, Copenhagen, Denmark\\
\and
Observational Cosmology, Mail Stop 367-17, California Institute of Technology, Pasadena, CA, 91125, U.S.A.\\
\and
Optical Science Laboratory, University College London, Gower Street, London, U.K.\\
\and
SB-ITP-LPPC, EPFL, CH-1015, Lausanne, Switzerland\\
\and
SISSA, Astrophysics Sector, via Bonomea 265, 34136, Trieste, Italy\\
\and
School of Physics and Astronomy, Cardiff University, Queens Buildings, The Parade, Cardiff, CF24 3AA, U.K.\\
\and
School of Physics and Astronomy, University of Nottingham, Nottingham NG7 2RD, U.K.\\
\and
Space Sciences Laboratory, University of California, Berkeley, California, U.S.A.\\
\and
Special Astrophysical Observatory, Russian Academy of Sciences, Nizhnij Arkhyz, Zelenchukskiy region, Karachai-Cherkessian Republic, 369167, Russia\\
\and
Stanford University, Dept of Physics, Varian Physics Bldg, 382 Via Pueblo Mall, Stanford, California, U.S.A.\\
\and
Sub-Department of Astrophysics, University of Oxford, Keble Road, Oxford OX1 3RH, U.K.\\
\and
Theory Division, PH-TH, CERN, CH-1211, Geneva 23, Switzerland\\
\and
UPMC Univ Paris 06, UMR7095, 98 bis Boulevard Arago, F-75014, Paris, France\\
\and
Universit\'{e} de Toulouse, UPS-OMP, IRAP, F-31028 Toulouse cedex 4, France\\
\and
University of Granada, Departamento de F\'{\i}sica Te\'{o}rica y del Cosmos, Facultad de Ciencias, Granada, Spain\\
\and
Warsaw University Observatory, Aleje Ujazdowskie 4, 00-478 Warszawa, Poland\\
}


==> section_1.0/section_1.0.tex <==
\section{Introduction}

This paper, one of a set associated with the 2013 release of
data from the \Planck\footnote{\Planck\ (\url{http://www.esa.int/Planck}) is a
  project of the European Space Agency (ESA) with instruments provided
  by two scientific consortia funded by ESA member states (in
  particular the lead countries France and Italy), with contributions
  from NASA, (USA) and telescope reflectors provided by a
  collaboration between ESA and a scientific conosrtium led and funded
by Denmark} mission \citep{planck2013-p01}\all2013resultspapers
describes a set of studies undertaken to determine the statistical
properties of the cosmic microwave background (CMB).

The standard cosmological model is described well by the {\it
  Friedmann-Lema\^{\i}tre-Robertson-Walker} (FLRW) solution of the Einstein
field equations. This model is characterized by a homogeneous and
isotropic metric and a scale factor of the expanding Universe. At very
early times it is hypothesized that the Universe went through a period
of accelerated expansion, the so-called {\it cosmological inflation},
driven by a hypothetical scalar field, the {\it inflaton}. During
inflation the universe behaves as a de Sitter space, providing the
conditions in which some of the present properties of the universe can
be realized and specifically relaxing the problem of initial
conditions. In particular, the seeds that gave rise to the present
large-scale matter distribution via gravitational instability
originated as quantum fluctuations of the inflaton about its vacuum
state. These fluctuations in the inflaton produce energy perturbations
that are distributed as a homogeneous and isotropic Gaussian random
field. Linear theory relates those energy fluctuations to the
CMB anisotropies, implying a distribution for the anisotropies very
close to that of an isotropic Gaussian random field.

The scope of this work is to use \Planck\ data to test the Gaussianity
and near isotropy of the CMB in intensity, as expected in the standard
cosmology paradigm. Testing these fundamental properties is crucial
for the validation of the standard cosmological scenario, and has
profound implications for our understanding of the physical nature of
the Universe and the initial conditions of structure formation.
Moreover, the confirmation of the isotropic and Gaussian nature of the
CMB is essential for justifying the corresponding assumptions usually made
when estimating the CMB power spectra and other quantities to be
obtained from the \Planck\ data. Conversely, the detection of
significant deviations from these assumptions that are not consistent
with known systematic effects or foreground residuals would
necessitate major revision of current methodological approaches for
derivating the mission's many science results.

Significant deviations from Gaussianity are expected from 
non-linear processes that lead to secondary anisotropies, e.g., the
integrated Sachs-Wolfe (ISW) effect and lensing.
Indeed, these effects are the subject of two companion \Planck\ papers
\citep[][respectively]{planck2013-p12,planck2013-p14}.
However, remarkably, a number of anomalies, by which we mean features
of the observed sky that are not statistically consistent with the
best-fit $\Lambda$CDM model, have been found in the \textit{WMAP}
data. Indeed, the \textit{WMAP} team \citep{spergel2003} themselves
initially proposed some intriguing discrepancies in the form of a lack
of power on large angular scales, which was subsequently reconfirmed
for the three-year data in
\citet{Copi2007}. Further examples include an
alignment of the low-order multipoles 
\citep{Tegmark2003,schwarz2004,bielewicz2005,Land2005},
a north-south asymmetry in both power spectra
\citep{eriksen2004b,hansen2009} and various measures of
non-Gaussianity \citep{eriksen2004c,eriksen2005,raeth07a}, parity
asymmetry in the power spectrum corresponding to large angular scales
\citep{kim2010},
and a region of significant temperature decrement --- the so-called {\it cold spot} \citep{vielva2004, cruz2005}.

Whilst \textit{WMAP} have presented refutations of these anomalies,
either by criticizing the robustness of the statistical methods
employed \citep{bennett2010} or by associating them with systematic
artefacts of the data processing that have been corrected in the
nine-year data release \citep{bennett2012}, \Planck\ represents a
unique opportunity to independently assess their existence.  Its
higher angular resolution and sensitivity and wider frequency range
enable a better understanding and removal of the Galactic and
extragalactic foregrounds thus allowing a larger fraction of the sky
to be useful for performing isotropy and Gaussianity analysis and to
confirm and interpret those anomalies.

Throughout this paper, we quantify the significance of the test
statistic in terms of the {\it p}-value. This is the probability of
obtaining a test statistic at least as extreme as the observed one,
under the assumption that the null hypothesis (i.e., Gaussianity and
isotropy of the CMB) is true. In some tests, where it is very
justified to only use a one-tailed probability, the {\it p}-value is
replaced by the corresponding upper or lower-tail probability. A low
{\it p}-value is indicative of a tension between the data and the assumed
statistical model (the null hypothesis). This can arise either when
the assumed cosmological model is incorrect, if unknown or unmodelled
aspects of the foreground emission or the measurement process exist,
or as a result of a natural statistical fluctuation. The most
interesting possibility, of course, is that a low {\it p}-value is an
indication of new physics.

From the theoretical point of view, there are many variants of
inflation that predict high levels of non-Gaussianity and new
scenarios motivated by string and M-theory. In addition, there are
many physical effects that might give rise to a deviation from
isotropy or the presence of non-Gaussianity. Those deviations may be
classified according to their physical nature and origin as follows:
non-standard inflationary models, geometry and topology of the
Universe, and topological defects.
The main results from these areas, as well as the detailed
descriptions of methodologies and of specific theoretically-motivated
model constraints, are provided in the companion
papers~\citep{planck2013-p09a,planck2013-p19,planck2013-p20}.

This paper covers all relevant aspects related to the phenomenological
study of the statistical isotropy and Gaussian nature of the CMB
measured by the \Planck\ satellite. It is organized as follows.
Section~\ref{sec:data} describes the \Planck\ data used for the
analyses. Section~\ref{sec:simulations} explains the main
characteristics of the simulations that constitute our reference set
of Gaussian sky maps representative of the null hypothesis. In
Sect.~\ref{sec:Gaussian_fluctuations} the null hypothesis is tested
with a number of standard tests that probe different aspects of
non-Gaussianity. The \textit{WMAP} anomalies are revisited in the
light of the \Planck\ data in Sect.~\ref{sec:anomalies_revisited}.
In Sect.~\ref{sec:Cl_implications} the implications of the found
deviations of the null hypothesis on $C_{\ell}$ and cosmological
parameters estimations are discussed. Finally,
Sect.~\ref{sec:conclusions} provides the main conclusions of the
paper.



==> section_2.0/section_2.0.tex <==
\section{Data description}
\label{sec:data}

In this paper, we utilize data from the \Planck-2013 data release
corresponding to the nominal period of the \Planck\ mission.  In part,
this comprises sky maps at nine frequencies, with corresponding ``half-ring'' maps that are generated by separating the data for a given
pointing period into two halves, plus maps generated from data within
the first and second survey periods. 
The maps are provided in 
{\tt HEALPix}\footnote{\url{http://healpix.sourceforge.net}}
format, with a pixel size defined by the $N_{\rm side}$ parameter.
This set of maps allows a variety
of consistency checks to be made, together with estimates of the
instrumental noise contributions to analyses and limits on
time-varying systematic artefacts. Full details are provided in
a series of companion papers~\citep{planck2013-p02,planck2013-p03}.

Our main results are based on the CMB maps resulting from
sophisticated component separation algorithms applied to the frequency
maps, as detailed in \citet{planck2013-p06}. The four methods --- {\tt
  Commander-Ruler}, {\tt NILC}, {\tt SEVEM} and {\tt SMICA} --- are
used to generate estimates of the CMB sky with an effective angular
resolution of around 7$\arcmin$ or better, with accompanying
symmetrized beam profiles, analysis masks, and half-ring 
maps.

In Table~\ref{tab:masks} we list the different masks that have been
used in the analyses described in this paper. These masks have been
produced at full resolution ($N_{\rm side}$=2048) and are described in
papers~\citep{planck2013-p06,planck2013-p08}.  In general, we make use
of a standardized common mask that merges those associated with the
individual methods (listed in Table~\ref{tab:masks} as U73).
Where appropriate, we manipulate the masks for use at lower resolution,
and, in particular, they have been degraded to
lower resolutions ($N_{\rm side}=$1024, 512, 256, 128, 64, 32 and
16). The masks with resolutions $N_{\rm side}$=128--1024 have been
degraded using the following procedure: first, the masks are degraded
to their final resolution using the {\tt ud\_degrade} {\tt HEALPix}
routine, and then, a conservative approach is followed setting to zero
any pixels with a value lower than 0.8. If the masks have to be
degraded to even lower resolutions, $N_{\rm side}=$16--64, the
procedure that has been used is different. First, the full-resolution
mask is smoothed with a Gaussian kernel with a FWHM equal to three
times the pixel size of the low resolution mask that we want to
produce. Then the mask is degraded using {\tt ud\_degrade} to their
final resolution. Finally, those pixels with a value lower or equal
than 0.5 have been set to zero and the rest have been set to 1. This
criterion, less conservative than the one used for the higher
resolution masks, is a compromise between minimizing the amount of sky
that is being masked and the level of contamination left unmasked. 
Note that in some cases the more conservative criterion of a 0.8
threshold has been used for the lower resolutions, as stated in
the corresponding analyses.
\begin{table}
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{List of the  masks that have been used for the analyses described in this paper. All of them have been generated at $N_{\rm side}=2048$, and when needed, they have been degraded to a lower resolution, as explained in the text. The CL masks have been constructed following the procedure described in \citet{planck2013-p08} but for 
different sky coverages.}
\label{tab:masks}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth
   \setbox0=\hbox{\rm 0}
   \digitwidth=\wd0
   \catcode`*=\active
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth
   \setbox0=\hbox{+}
   \signwidth=\wd0
   \catcode`!=\active
   \def!{\kern\signw
idth}
\halign{\hbox to 1.3in{#\leaderfil}\tabskip=2pt&\hfill#\hfill\/\tabskip=0pt\cr                          
\noalign{\doubleline}
   % Table headings go here.
%\noalign{\vskip 3pt\hrule\vskip 5pt}
%\halign{#\hfil\tabskip=2em &\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\tabskip=0pt\cr
%\noalign{\doubleline} \cr
\omit\hfil Mask name \hfil&  Sky coverage\cr
\omit&  [\% of unmasked pixels]\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
CS-SMICA89$^1$&  89.0\cr
U73$^1$& 73.0\cr
CG90$^1$& 90.0\cr
CG80$^1$& 80.0\cr
CG70$^1$& 70.0\cr
CG60$^1$& 60.0\cr
CL65$^2$& 65.1\cr
CL58$^2$& 57.8\cr
CL48$^2$& 48.0\cr
CL37$^2$& 37.3\cr
CL25$^2$& 24.7\cr
%\noalign{\vskip 10pt}
\noalign{\vskip 3pt\hrule\vskip 3pt}
$^1$\citet{planck2013-p06} \cr
$^2$\citet{planck2013-p08} \cr
\noalign{\vskip 3pt}}}
%\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable % this command is defined in Planck.tex.
\endgroup
\end{table}

==> section_3.0/section_3.0.tex <==
\section{Simulations}
\label{sec:simulations}

The derivation of results to be presented in this paper requires extensive
simulations, essential aspects of which include:
1) modelling the \Planck\ instrumental effects that affect the quality of the
data, including instrumental noise and identified systematic effects; 
2) replicating the foreground removal approach and estimating the
extent of foreground residuals; and 
3) modelling the intrinsic statistical properties, Gaussian or otherwise,
of the CMB signals expected from specific models of the Universe.

The full focal plane (FFP6) simulations described in
\citet{planck2013-p28} provide a complete realization of the \Planck\
mission capturing all characteristics of the scanning strategy,
telescope, detector responses, and data reduction pipeline over the
nominal mission period of 15.5 months.  The Planck Sky Model (PSM) is
used as input, encompassing the best current estimate of the microwave
sky at \Planck\ wavelengths including Galactic and extragalactic
astrophysical foreground emission.  The outputs include a complete set
of maps for all detectors with accompanying half-ring and survey
splits generated for a reference CMB sky. These have been used to test
and validate various analysis tools, employed in turn to evaluate the
CMB component separation algorithms as applied to the data set.  This
also allows an FFP6-based estimate of the foreground residuals
remaining in the CMB sky after component separation to be evaluated,
and their impact on various statistical estimators quantified.

An accompanying set of Monte Carlo simulations, that are allowed to
vary within the cosmic variance, provides us with the  
reference set of Gaussian sky maps used for the null tests we employ.
These simulations include {\tt FEBeCoP} \citep{mitra2010} beam
convolution at each of the \Planck\ frequencies, which are then
propagated through the various component separation pipelines using
the same weights as derived from the \Planck\ nominal mission data
analysis.  A fiducial CMB power spectrum has been adopted (and varied 
in the simulations within the cosmic variance) based on an
analysis of the \Planck\ data at an advanced, but not final stage of
processing. Only small changes relative to the final \Planck\ power
spectrum presented in~\citep{planck2013-p08,planck2013-p11} are
observed.

==> section_4.0/section_4.0.tex <==
\section{Are the primordial fluctuations Gaussian?}
\label{sec:Gaussian_fluctuations}
As has been previously established, it is of major interest to
determine whether the statistical properties of the primordial CMB
anisotropies correspond to an isotropic Gaussian random field.
Recent attempts to test this hypothesis have mainly relied on the
\textit{WMAP} data that have less sensitivity and cover a narrower
frequency interval. \Planck\ represents a unique
opportunity to probe fundamental statistical properties of the
Universe with cosmic variance limited sensitivity up to $\ell\approx
2000$ and minimum foreground contamination.

There is no unique signature of non-Gaussianity, however, different
tests can allow us to probe different types of non-Gaussianity. As a
consequence, it is important to subject the data to a variety of
tests, and we do so in this section using a number of non-parametric
tools.
Specific signatures of non-Gaussianity are sought in three companion
papers~\citep{planck2013-p09a,planck2013-p20,planck2013-p19}.

Any signal on the sphere, $T(\vec{x})$, can be  written in terms of the 
following spectral representation:
%
\begin{equation}
\label{eq:T_alm}
  T(\vec{x})=\sum^\infty_{\ell=0}\sum^\ell_{m=-\ell} a_{\ell m}Y_{\ell m}(\vec{x}),
\end{equation}
where $\vec{x}$ is a unit direction vector, $Y_{\ell m}$ the spherical harmonics and 
\begin{eqnarray}
  \label{eq:alm}
   a_{\ell m}=\int \mathrm{d}\vec{x} T(\vec{x})Y^*_{\ell m}(\vec{x}),\\
\nonumber
m=0,\pm1,\dots, \pm \ell, ~~~\ell=1,2,\dots
\end{eqnarray}
For an isotropic random field the $a_{\ell m}$
coefficients are uncorrelated: 
%, are uncorrelated, and in
%the Gaussian case they are also independent with variance:
\begin{equation}
   \langle a_{\ell m} a^*_{\ell' m'}\rangle  =\delta^{\ell}_{\ell'}\delta^{m}_{m'}C_{\ell},
\end{equation}
%
where $\delta$ is the Kronecker delta and $C_{\ell}$ is the angular
power spectrum.  Note that for a Gaussian and isotropic random field,
the $a_{\ell m}$ coefficients are independent and, if the mean is zero, 
the angular power spectrum provides a complete characterization of its 
statistical distribution.

In this paper, we examine the goodness-of-fit of the data to the
\Planck\ best-fit fiducial CMB model, which constitutes our null
hypothesis.
The methods adopted constitute a broad range of statistical tools that
allow the study of complementary statistical properties of the null
hypothesis in both the real and harmonic space data representations.
Claims of either
consistency with the fiducial \Planck\ cosmological model or of
evidence for non-Gaussianity must be demonstrably robust to data
selection and specifics of the data analysis. Residuals from the
diffuse Galactic foreground are likely to be non-Gaussian in nature,
and point-sources can be a source of non-Gaussianity on small angular
scales. In addition, the analysis of multifrequency data must be
considered in order to confirm that any claimed non-Gaussianity has a
thermal (cosmological) spectrum. Moreover, the combined ISW-lensing
effect produces secondary anisotropies that significantly deviate from
Gaussianity and whose effect has been detected in the \Planck\ data
\citep{planck2013-p14}. This non-Gaussian effect has to be considered
when testing the null hypothesis.

We address these issues by %applying a suite of statistical tests to
analysing the cosmologically interesting subset of \Planck\ frequency channels.
Specifically, we analyse the uncorrected sky maps at 70, 100, 143 and
217\,GHz, as a function of Galactic mask, to assess the likely
contamination due to Galactic foregrounds. These tests have direct
relevance for the \Planck\ likelihood approach described in
\citet{planck2013-p08} and the parameter estimation results presented
in \citet{planck2013-p11}. We then consider the foreground cleaned
versions of these maps generated by the \sevem\ algorithm
\citep{planck2013-p06}.  Such a comparison also allows a
semi-independent cross-check of the cosmological signal seen by
\Planck\ LFI (70\,GHz) and HFI (100, 143, 217\,GHz). Although the
cosmological content of the cleaned LFI and HFI data sets are
independent, the cleaning makes use of difference maps generated from
the remaining \Planck\ frequency bands. Nevertheless, since the
calibration and beam responses of the data are well understood over
the ful range of frequencies, there will be no leakage of cosmological
signal between the instrument specific frequencies.

We then continue with analyses of the CMB sky estimates 
provided by four component separation approaches 
({\tt Commander-Ruler}, {\tt NILC}, {\tt SEVEM}, and {\tt SMICA})
described in
\citet{planck2013-p06}, together with the corresponding mask
appropriate for these methods.  The largest sky area possible should
be used for definitive statements about Gaussianity, since, in the
absence of foreground residuals or systematic artefacts, it represents
a superior sample of the Universe. Conversely, overly conservative sky
cuts suffer from a loss of information.

%Tests of the Null hypothesis
\input{./section_4.0/section_4.1/section_4.1}



==> section_4.0/section_4.1/section_4.1.tex <==

\subsection{One dimensional moments}
\label{sec:one_dimensional_moments}

In this section we perform some of the simplest Gaussianity tests,
such as comparing the sample skewness and kurtosis of the data with
simulations.  The skewness, $\gamma$, and kurtosis, $\kappa$, of a
random variable, $X$, are defined as
%
\begin{equation}
\gamma(X) =  \frac{\langle X-\langle X \rangle \rangle^3 }{(\sigma^2(X))^{3/2}},
\label{skewness}
\end{equation}
% 
%
\begin{equation}
\kappa(X) = \frac{ \langle X- \langle X \rangle \rangle^4 }{(\sigma^2(X))^2} -3,
\label{kurtosis}
\end{equation}
% 
where $\sigma^2$, the variance is:
%
\begin{equation}
\sigma^2(X) =  \langle X^2 \rangle - \langle X \rangle^2.
\label{variance}
\end{equation}
% 
Here $X$ represents the pixel temperature at some $N_{\rm side}$ and the averages 
are performed over the sky.
The skewness is a measure of the asymmetry of the probability
distribution of a real-valued random variable.  Qualitatively, a
positive (negative) skew indicates that the tail on the right (left)
side of the probability density function is longer than the left
(right) side. A zero value indicates that the values are relatively
evenly distributed on both sides of the mean, typically but not
necessarily, implying a symmetric distribution.  The kurtosis is a
measure of the peakedness of the distribution and the heaviness of its
tail. A distribution with positive (negative) excess kurtosis
indicates that the distribution has a more acute (wider) peak around
the mean and fatter (thinner) tails.  Normal random variables have
zero skewness and kurtosis.

The sample variance, $\sigma^2$ is also considered in this section as a further
consistency test, although it is not a normality test statistic.
% Results
\input{./section_4.0/section_4.2/section_4.2.1/section_4.2.1}

\subsection{$N$-pdf analysis}
\label{sec:n-pdf}

Under the assumption of Gaussianity, the $N$-probability density
function ($N$-pdf) is given by a multivariate Gaussian function:
%
\begin{equation}
f\left(\vec{T}\right) = \frac{1}{\left(2\pi\right)^{N_{pix}/2}\det{\tens{C}}^{1/2}}
\exp{-\frac{1}{2}\left(\vec{T}\tens{C}^{-1}\vec{T}^{\rm T}\right)},
\label{eq:npdf_npdf}
\end{equation}
%
where $\vec{T}$ is a vector formed from the measured temperatures
$T(\vec{x})$ over all positions allowed by the applied mask,
$N_{\rm pix}$ is the number of pixels in the vector, $\tens{C}$ is the
covariance of the Gaussian field (of size $N_{\rm pix} \times N_{\rm pix}$).

Unfortunately, the calculation of $\vec{T}\tens{C}^{-1}\vec{T}^{\rm T}$ is
computationally unfeasible for the full \Planck\ resolution at {\tt HEALPix}
$N_{\rm side}=2048$.
At a lower resolution, the problem is tractable, and the noise level
can also be considered negligible compared to the CMB signal.  That
implies that under the assumption of isotropy the covariance matrix
$\tens{C}$ is fully defined by the \Planck\ angular power spectrum
($C_\ell$):
%
\begin{equation}
\mathrm{C}_{ij} = \sum_{\ell=0}^{\ell_\mathrm{max}} \frac{2\ell+1}{4\pi} C_\ell b_\ell^2 
P_\ell\left(\cos \theta_{ij}\right),
\label{eq:npdf_C}
\end{equation}
%
where $\mathrm{C}_{ij}$ is the covariance between pixels $i$ and $j$,
and $\theta_{ij}$ is angle between them, $P_\ell$ are the Legendre
polynomials, $b_\ell$ is an effective window function
associated with the $N_{\rm side}$ resolution, and $\ell_\mathrm{max}$ is the
maximum multipole probed.

Under the multivariate Gaussian hypothesis, the argument on the
exponential in equation~\ref{eq:npdf_npdf} should follow a $\chi^2$
distribution with $N_{\rm pix}$ degrees of freedom, or, equivalently (for $N_{\rm pix} \gg 1$) a normal distribution $\mathcal{N}\left(N_{\rm pix},
  \sqrt{N_{\rm pix}}\right)$.  
  
% Results
\input{./section_4.0/section_4.2/section_4.2.2/section_4.2.2}  

\subsection{$N$-point correlation functions} 
\label{sec:npoint_correlation}

In this section we present tests of the non-Gaussianity of the \Planck\
CMB maps using real-space $N$-point correlation functions. While
harmonic-space methods are often preferred over real-space methods for
studying primordial fluctuations, real-space methods may have an
advantage with respect to systematics and foregrounds, since such
effects are usually localized in real space. It is therefore important
to analyse the data in both spaces in order to highlight different
features.

An $N$-point correlation function is by definition the average product
of $N$ temperatures, measured in a fixed relative orientation on the
sky,
\begin{equation}
C_{N}(\theta_{1}, \ldots, \theta_{2N-3}) 
= \left\langle\Delta T(\vec{\hat{n}}_{1})\cdots
\Delta T(\vec{\hat{n}}_{N}) \right\rangle,
\label{eq:npoint_def}
\end{equation}
where the unit vectors $\vec{\hat{n}}_1, \ldots,\vec{\hat{n}}_{N}$ span an
$N$-point polygon on the sky. By assuming statistical isotropy, the
$N$-point functions are only functions of the shape and size of the
$N$-point polygon, and not on its particular position or orientation
on the sky. Hence, the smallest number of parameters that
uniquely determines the shape and size of the $N$-point polygon is
$2N-3$. In practice, the functions are estimated by simple product
averages over all sets of $N$ pixels fulfilling the
geometric requirements set by $\theta_1, \ldots, \theta_{2N-3}$
characterizing the shape and size of the polygon,
\begin{equation}
C_{N}(\theta_{1}, \ldots, \theta_{2N-3}) 
= \frac{\sum_i \left(w_1^i \cdots w_N^i \right) \left(\Delta T_1^i \cdots
\Delta T_N^i \right) }{\sum_i w_1^i \cdots w_N^i}\ .
\label{eq:npoint_estim}
\end{equation}
Pixel weights $w_1^i,\cdots,w_N^i$ can be introduced in order to
reduce noise or mask boundary effects. Here they represent masking by
being set to 1 for included pixels and to 0 for excluded pixels.

The main difficulty with computing $N$-point functions is their
computational scaling. The number of independent pixel combinations
scales as $\mathcal{O}(N_{\rm pix}^N)$, and for each combination
of $N$ pixels, $2N-3$ angular distances must be computed to uniquely
determine the properties of the corresponding polygon. Computing the
full $N$-point function for $N>2$ and $N_{\rm pix} \gtrsim 10^5$
is therefore computationally challenging.  However, it is not
necessary to include all possible $N$-point configurations in order to
produce interesting results. For instance, one may focus only on small angular
scales, or on configurations with some special symmetry properties. By
using the methods described in \citet{eriksen2004a}, the computational
expense then becomes tractable, since no CPU time is spent on excluded
configurations. In this paper several such subsets are computed,
covering three distinct ranges of scales, namely small (up to
$3^{\circ}$), intermediate (up to $10^\circ$) and large angular scales (the full range between $0^{\circ}$ and
$180^{\circ}$). 

The shapes of the polygons selected for the analysis are 
the pseudo-collapsed and equilateral configurations for the 3-point function, and the rhombic configuration for the 4-point function, composed of two
equilateral triangles that share a common side. 
We use the same definition of
  pseudo-collapsed as in \citet{eriksen2005}
  i.e.,~as isosceles triangle where the length of the baseline falls within the
  second bin of the separation angles. The length of the longer edge of
  the triangle, $\theta$, parametrizes its size. Analogously, in the case of
the equilateral triangle and rhombus, the size of the polygon is
parametrized by the length of the edge, $\theta$. Note that these
  functions are chosen because of ease of implementation, not
  because they are better suited for testing Gaussianity than
  other configurations. In the following, all
results refer to the reduced 4-point function, i.e., corrected for the
Gaussian contribution due to Wick's theorem.

% Results
\input{./section_4.0/section_4.2/section_4.2.3/section_4.2.3}

\subsection{Minkowski functionals}
\label{sec:Minkowski_functionals}
%
Minkowski functionals (hereafter MFs) describe the morphology of
fields in any dimension and have long been used as estimators of
non-Gaussianity and anisotropy in the CMB \citep[see
e.g.,][]{mecke1994,schmalzing1997,schmalzing1998,komatsu2003,eriksen2004c,curto2007,troia2007,spergel2007,curto2008,hikage2008,komatsu2009}. They
are additive for disjoint regions of the sky and invariant under
rotations and translations. Traditionally in the literature, the
contours are defined by a threshold $\nu$, usually given in units of
the sky standard deviation ($\sigma_0$). We compute 
MFs for the regions colder and hotter than a given
threshold $\nu$. Thus, the three MFs, the area $V_0(\nu)=A(\nu)$, the
perimeter $V_1(\nu)=C(\nu)$, and the genus $V_2(\nu)=G(\nu)$, are
defined respectively as:
%
\begin{equation} V_0(\nu) = A(\nu) = \frac{N_\nu}{N_{\rm pix}}; \end{equation}
\begin{equation} V_1(\nu)= C(\nu) = \frac{1}{4A_{\rm tot}}\sum_{i}S_i; \end{equation}
\begin{equation} V_2(\nu)=G(\nu) = \frac{1}{2\pi A_{\rm tot}}\big( N_{\rm hot} - N_{\rm cold}\big). \end{equation}
%
Here $N_{\nu}$ is the number of pixels where $\Delta T / \sigma_0 >
\nu$, $N_{\rm pix}$ is the total number of available pixels, $A_{\rm tot}$ is
the total area of the available sky, $N_{\rm hot}$ is the number of
compact hot spots, $N_{\rm cold}$ is the number of compact cold spots,
and $S_i$ is the contour length of each hot spot. We construct a
fourth functional $V_3(\nu)=N_{\rm cluster}(\nu)$ which
corresponds to $N_{\rm cold}$ for negative $\nu$ and $N_{\rm hot}$ for
positive $\nu$ \citep{ducout2012}.  
Analytical expressions for a
Gaussian random field can be derived in terms of $\nu$ \citep[see
  e.g.][]{vanmarcke1983,matsubara2010} and give
%
\begin{equation}
V_{k}(\nu)=A_{k}v_{k}(\nu),
\end{equation} 
%
with
%
\begin{eqnarray}
v_{k}(\nu) &= &\exp(-\nu^{2}/2) H_{k-1}(\nu), \quad k \leq 2 \label{eq:nuk1} \\
v_{3}(\nu) &= & \frac{e^{-\nu^{2}}}{\mathrm{erfc}\left(\nu /\sqrt{2}\right)}, \label{eq:nuk2}
\end{eqnarray}
%
and
%
\begin{equation}
H_{n}(\nu)={\rm e}^{\nu^{2}/2}\left(-\frac{\rm d}{{\rm d}\nu}\right)^{n} {\rm e}^{-\nu^{2}/2}.
\end{equation}
%
The amplitude $A_k$ only depends on the shape of the power spectrum $C_{\ell}$:
%
\begin{eqnarray} 
A_{k} &= &\frac{1}{(2\pi)^{(k+1)/2}}\frac{\omega_{2}}{\omega_{2-k}\omega_{k}}\left( \frac{\sigma_{1}}{\sqrt{2}\sigma_{0}}\right)^{k},\quad k \leq 2 \\
A_{3} &= &\frac{2}{\pi}\left( \frac{\sigma_{1}}{\sqrt{2}\sigma_{0}}\right)^{2}
 \end{eqnarray}
%
where $\omega_{k}\equiv\pi^{k/2}/\Gamma(k/2+1)$, which gives
$\omega_{0}=1$, $\omega_{1}=2$, and $\omega_{2}=\pi$ with $\sigma_{0}$ and
$\sigma_{1}$ beign respectively, the rms of the field and its first
derivatives.
These analytical expressions represent useful descriptions of the MFs
which, for the case of a Gaussian random field, can be factorized as a
function of the threshold and another of the shape of the
$C_{\ell}$. We will use both the unnormalized ($V_k$) and normalized
($\nu_k$) MFs in the Gaussianity tests performed in this section. The
unnormalized functionals are computed with a code that was used for
the analysis of Archeops data \citep{curto2007} and has been
thoroughly validated with \Planck\ simulations, while for the normalized
ones a code adapted to the high resolution \Planck\ data and described
in \cite{ducout2012} is used.


%
% Results with MF
%
\input{./section_4.0/section_4.2/section_4.2.4/section_4.2.4}
%
\subsection{Wavelet statistics}
\label{sec:wavelet_statistics}

A broad range of wavelets have been used in the analysis of CMB data,
but in this paper we specifically consider 
the Spherical Mexican Hat wavelet~\citep[SMHW,][]{martinezgonzalez2002}.

The SMHW is an example of a continuous, non-orthogonal wavelet. Given
a signal on the sky, $T(p)$, where $p$ represents a given
position/pixel wich is a function of the co-latitude $\theta$ and
longitude $\phi$ (also defined by the unit direction vector
$\mathbf{x}$), the SMHW coefficients at a given scale $R$,
$\omega_T\left(R,p\right)$, are obtained by convolution:
%
\begin{equation}
\omega_T\left(R,p\right) = \sum_{\ell = 0}^{\ell_{\rm max}} \sum_{m = -\ell}^{m = \ell} t_{\ell m}
W^{\rm SMHW}_\ell\left(R\right)Y_{\ell m}\left(p\right),
\label{eq:cs_def1}
\end{equation}
%
where $W^{\rm SMHW}_\ell\left(R\right)$ is the window function associated
with the SMHW, $\ell_{\rm max}$ is the maximum multipole allowed by
the corresponding {\tt HEALPix} pixelization, $Y_{\ell m}\left(p\right)$ is
the spherical harmonic basis, and $t_{\ell m}$ are the spherical
harmonic coefficients of the analysed map:
%
\begin{equation}
t_{\ell m} = \int \mathrm{d}\Omega Y^*_{\ell m}\left(p\right) T\left(p\right),
\label{eq:cs_def2}
\end{equation}
%
where $\mathrm{d}\Omega = \mathrm{d}\theta\sin{\theta}\mathrm{d}\phi$
and $^*$ denotes complex conjugation. 

Several statistics can be computed from the wavelet coefficients map, in
particular, the first moments: the dispersion $\sigma_R$, the skewness $S_R$, and the kurtosis $K_R$
(as a function of scale $R$). It is interesting to notice that in the case of Gaussian temperature fluctuations the linear transformation involved in the determination of the wavelet coefficients (eqs.~\ref{eq:cs_def1} and \ref{eq:cs_def2}) guarantees that Gaussianity is preserved.

% Results
\input{./section_4.0/section_4.2/section_4.2.5/section_4.2.5}



\subsection{Bispectrum}
\label{sec:bispectrum}
%
The CMB bispectrum is the three point correlator of the $a_{\ell m}$
coefficients: $B^{m_1 m_2 m_3}_{\ell_1 \ell_2 \ell_3} \equiv
\langle a_{\ell_1 m_1} a_{\ell_2 m_2} a_{\ell_3 m_3} \rangle$. In this
paper, we focus on the bispectrum reconstruction as a blind test of
non-Gaussianity. Therefore, we assume we are seeking a non-trivial
bispectrum that has arisen through a physical process which is
statistically isotropic, that is, we can employ the angle-averaged
bispectrum $\Blll$ and the reduced bispectrum $\blll$. Note that
$\blll$ is defined on a tetrahedral domain of multipole triples
$\{\ell_1 \ell_2 \ell_3\}$ satisfying both a triangle condition and a
limit given by the maximum resolution $\ell_{\rm max}$ of the experiment.  A
much more extensive introduction to the bispectrum can be found in
\citet{planck2013-p09a}.

% Bispectrum
\input{./section_4.0/section_4.2/section_4.2.7/section_4.2.7}


==> section_4.0/section_4.2/section_4.2.1/section_4.2.1.tex <==
%\subsubsection{1-pdf}
We begin by analysing the full resolution combined maps, applying the
U73 mask for the four different component separation methods.  The
results for the variance, skewness, and kurtosis estimators are shown
in Table~\ref{tab:methods_2048}. All four methods show similar
results. The data are consistent with simulations for the skewness and
kurtosis estimators, whereas the variance is anomalously low.  This
inconsistency was already reported for the \textit{WMAP} data in
\citet{monteserin2008} and \citet{2011MNRAS.412.2383C} at resolution
$N_{\rm side}=256$ for a mask allowing slightly less sky coverage.
%TABLE 4 METHODS:
\begin{table}[tmb]                 
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Lower tail probablity for the variance, skewness, and kurtosis
  estimators at $N_{\rm side}=2048$, using the U73 mask  and four different
  component separation methods.}                              
\label{tab:methods_2048}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 1.0in{#\leaderfil}\tabskip=2pt&
\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr                          
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan3 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan3\hrulefill\cr
\omit\hfil Method \hfil& \hfil Variance \hfil& \hfil Skewness \hfil& \hfil Kurtosis\hfil\cr                         % Table headings go here.
\noalign{\vskip 3pt\hrule\vskip 3pt}
{\tt C-R}& 0.021& 0.189& 0.416\cr
{\tt NILC}& 0.020& 0.191& 0.392\cr
{\tt SEVEM}& 0.014& 0.206& 0.419\cr
{\tt SMICA}& 0.017& 0.189& 0.419\cr                                    % Body of table goes here.
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table}                        % table* is a two-column table.  Drop the * for one column.

The mask dependence of our results is studied by recalculating the
estimators using the CL58 and CL37 masks, which allow sky
fractions of $f_{\rm sky}=58\%$ and $f_{\rm sky}=37\%$,
respectively. The \smica\ cleaned maps at full resolution are
considered. The most significant lower tail probability is obtained
for the CL58, mask as can be seen in
Table~\ref{tab:masks_2048}. The lower tail probabilities show a small
dependence on the mask used, which could indicate either the presence
of Galactic foreground residuals with larger sky coverage, or the
increase of the sampling variance, and consequently a less significant
probability, when a smaller fraction of the sky is considered.
\begin{table}[tmb]                 
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Lower tail probablity for the variance, skewness, and kurtosis estimators at $N_{\rm side}=2048$, for the {\tt SMICA} method, using different masks.}                              
\label{tab:masks_2048}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 1.7in{#\leaderfil}\tabskip=1pt&
\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr                          
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan3 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan3\hrulefill\cr
\omit\hfil Mask \hfil& \hfil Variance \hfil& \hfil Skewness \hfil& \hfil Kurtosis\hfil\cr
                         % Table headings go here.
\noalign{\vskip 3pt\hrule\vskip 3pt}
U73, $f_{\rm sky}=73\%$& 0.017& 0.189& 0.419\cr
CL58, $f_{\rm sky}=58\%$& 0.003& 0.170& 0.363\cr
CL37, $f_{\rm sky}=37\%$& 0.030& 0.314& 0.266\cr
Ecliptic North, $f_{\rm sky}=36\%$& 0.001& 0.553& 0.413\cr
Ecliptic South, $f_{\rm sky}=37\%$& 0.483& 0.077& 0.556\cr
%Ecliptic South with extended mask, $f_{\rm sky}=$30\% & 0.095 & 0.282 & 0.575 \\
Galactic North, $f_{\rm sky}=37\%$& 0.001& 0.788& 0.177\cr
Galactic South, $f_{\rm sky}=36\%$& 0.592& 0.145& 0.428\cr
%\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\noalign{\vskip 1pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table}                        % table* is a two-column table.  Drop the * for one column.

In order to identify any foreground contamination, the frequency
dependence of our estimators is analysed. We use the {\tt SEVEM}
cleaned maps and the U73 mask. Note that as the 70\,GHz full
resolution noise is high we do not consider 70\,GHz in this
comparison. As the 100\,GHz noise is not negligible we estimate the
variance taking into account the noise dispersion as described in
\citet{2011MNRAS.412.2383C}. The results are similar to those found
for the combined map, as can be seen in Table~\ref{tab:freq_2048}.
There is a small frequency dependence since the 100\,GHz and 217\,GHz
maps show slightly higher variance and kurtosis than the 143\,GHz
map. However the 143\,GHz map has a dominant contribution to the
combined map, hence the foreground residuals in the combined map are
likely to be small.  The lower tail probabilities for the variance at
100\,GHz, 143\,GHz, and 217\,GHZ are respectively 0.023, 0.014, 0.025,
whereas the skewness and kurtosis are compatible with simulations.
\begin{table}[tmb]                 
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Lower tail probablity for the variance, skewness, and kurtosis estimators at $N_{\rm side}=2048$, for the {\tt SEVEM} cleaned maps at different frequencies.}
\label{tab:freq_2048}                           % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 1.5in{#\leaderfil}\tabskip=1pt&
\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr                          
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan3 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan3\hrulefill\cr
\omit\hfil Map \hfil& \hfil Variance \hfil& \hfil Skewness \hfil& \hfil Kurtosis\hfil\cr                         % Table headings go here.
\noalign{\vskip 3pt\hrule\vskip 3pt}
%70 GHz      & 0.292   & 0.352 & 0.907\cr
100 GHz& 0.023& 0.195& 0.488\cr
143 GHz& 0.014& 0.221& 0.460\cr
217 GHz& 0.025& 0.196& 0.481\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table}                        % table* is a two-column table.  Drop the * for one column.

In order to study the hemispherical asymmetry reported in \citet{2011MNRAS.412.2383C}
we reanalyse the {\tt SMICA} data and simulations considering
independently the northern and southern ecliptic hemispheres outside
the U73 mask. A clear asymmetry is found in the variance, with an
anomalously low value found in the northern hemisphere, as 
seen in Table~\ref{tab:masks_2048}. Hemispherical asymmetries are further analysed 
in Sect. 5.3.

The results for different resolutions using the U73
mask are shown in Table~\ref{tab:lowres}. Note that the $N_{\rm
  side}=2048$ and 512 U73 masks have $f_{\rm sky}=73\%$, while the
low resolution masks at $N_{\rm side}=64$, 32, and 16 have $f_{\rm
  sky}=78\%$. The variance is anomalously low at all the considered
resolutions, whereas at low resolutions, the skewness is anomalously
low and the kurtosis anomalously high. These results will be further
analysed in Sect.~\ref{sec:anomalous_variance}. 
However, it is clear that, except on the largest angular scales, there
is no evidence for non-Gaussian behaviour in the data using these
simple statistical measures.
\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Lower tail probablity for the variance, skewness, and kurtosis estimators at different resolutions, for the four component separation methods, using the U73 mask.}
\label{tab:lowres}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 0.8in{#\leaderfil}\tabskip=1pt&
\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr                           
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan3 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan3\hrulefill\cr
\omit\hfil Method \hfil&  \hfil Variance  \hfil&  \hfil Skewness  \hfil&  \hfil Kurtosis\hfil\cr   
\noalign{\vskip 3pt\hrule\vskip 3pt}
\multispan4\hfil$N_{\rm side}=2048$\hfil\cr
\noalign{\vskip 2pt}
{\tt C-R}& 0.021& 0.189& 0.416\cr
{\tt NILC}& 0.020& 0.191& 0.392\cr
{\tt SEVEM}& 0.014& 0.206& 0.419\cr
{\tt SMICA}& 0.017& 0.189& 0.419\cr
\noalign{\vskip 3pt}
%\noalign{\vskip 3pt\hrule\vskip 3pt}
\multispan4\hfil$N_{\rm side}=512$\hfil\cr
\noalign{\vskip 2pt}
{\tt C-R}& 0.017& 0.207& 0.368\cr
{\tt NILC}& 0.017& 0.198& 0.390\cr
{\tt SEVEM}& 0.013& 0.218& 0.408\cr
{\tt SMICA}& 0.014& 0.196& 0.390\cr
\noalign{\vskip 3pt}
\multispan4\hfil$N_{\rm side}=64$\hfil\cr
\noalign{\vskip 2pt}
{\tt C-R}& 0.011& 0.041& 0.935\cr
{\tt NILC}& 0.011& 0.041& 0.935\cr
{\tt SEVEM}& 0.008& 0.058& 0.900\cr
{\tt SMICA}& 0.011& 0.041& 0.943\cr
\noalign{\vskip 3pt}
\multispan4\hfil$N_{\rm side}=32$\hfil\cr
\noalign{\vskip 2pt}
{\tt C-R}& 0.020& 0.015& 0.968\cr
{\tt NILC}& 0.019& 0.016& 0.960\cr
{\tt SEVEM}& 0.012& 0.026& 0.932\cr
{\tt SMICA}& 0.019& 0.016& 0.967\cr
\noalign{\vskip 3pt}
\multispan4\hfil$N_{\rm side}=16$\hfil\cr
\noalign{\vskip 2pt}
{\tt C-R}& 0.023& 0.013& 0.974\cr
{\tt NILC}& 0.022& 0.022& 0.972\cr
{\tt SEVEM}& 0.019& 0.022& 0.964\cr
{\tt SMICA}& 0.027& 0.021& 0.982\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table}            

\begin{figure}
\centerline{
\includegraphics[width=\hsize]{./section_4.0/section_4.2/section_4.2.1/figs/hist_methods_deltaDX9.pdf}
}
\caption{Variance, skewness, and kurtosis for the combined map of the four different component separation methods. From top row to bottom row {\tt C-R}, {\tt NILC}, {\tt SEVEM}, {\tt SMICA}.}
\label{fig:methods}
\end{figure}



==> section_4.0/section_4.2/section_4.2.2/section_4.2.2.tex <==
%\subsubsection{N-pdf}

We begin by analysing the $\chi^2$ quantity for low resolution maps at
$N_{\rm side}=32$ and filtering with a $5^{\deg}$ FWHM Gaussian. $1\,
\mu\!{\rm K}$ uncorrelated regularization noise is added to the covariance
matrix before inverting it. Regularization noise realizations are
added to the data and simulations for consistency 
\citep[see][for more details]{eriksen2007b}.

We analyse the four cleaned data maps, applying the common, CL58
and CL37 masks. The admitted fraction of the sky is respectively
$78\%, 58\%$ and $37\%$. The northern and southern ecliptic
hemispheres outside the U73 mask are also considered independently 
in order to check for possible hemispherical asymmetries as those analysed in Sect. 5.3.  
The results are shown in Fig.~\ref{fig:npdf-masks} and Table~\ref{tab:npdf-masks}.
In the U73 mask case, the lower tail probabilities are low.
Applying the two CL58 and CL37 masks that permit less sky coverage, gives data
that are consistent with simulations. The low $\chi^2$ value appears to be
localized in the northern ecliptic hemisphere. These results are
directly comparable to the anomalous variance mentioned in
Sect.~\ref{sec:one_dimensional_moments}. Note that the four maps show
similar values, but the differences are larger when using the U73
mask. This could indicate the presence of some residual foreground
contamination near the Galactic plane.
\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Lower tail probablity for the $N$-pdf, using different masks.}
\label{tab:npdf-masks}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 1.6in{#\leaderfil}\tabskip=3pt&
\hbox to 0.4in{\hfil#\hfil}\tabskip=8pt&\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan4 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan4\hrulefill\cr
\omit\hfil Mask \hfil& {\tt C-R}& {\tt NILC}& {\tt SEVEM}& {\tt SMICA}\cr   
\noalign{\vskip 3pt\hrule\vskip 3pt}
U73, $f_{\rm sky}=78\%$& 0.027& 0.028 & 0.019& 0.030\cr
CL58, $f_{\rm sky}=58\%$& 0.137& 0.137 & 0.147& 0.146\cr
CL37, $f_{\rm sky}=37\%$& 0.409& 0.415 & 0.420& 0.436\cr
Ecliptic North, $f_{\rm sky}=39\%$& 0.024& 0.022& 0.021& 0.021\cr
Ecliptic South, $f_{\rm sky}=39\%$& 0.170& 0.196& 0.183& 0.193\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table}            
Therefore, the frequency dependence of our estimator is analysed in
order to identify any possible foreground contamination. The results
are shown in Fig.~\ref{fig:npdf-freq} and Table~\ref{tab:npdf-freq}. A
moderate frequency dependence is found when using the U73 mask,
which could indicate the presence of some foreground residuals near
the Galactic plane. The frequency dependence of the results vanishes
when using the CL58 and CL37 masks that exclude more of the sky from analysis.


%FIGURE MASK DEPENDENCE
\begin{figure}
\centerline{
\includegraphics[width=88mm]{./section_4.0/section_4.2/section_4.2.2/figs/npdf_masks_1000sims_n0032.pdf}
}
\caption{$N$-pdf $\chi^2$ for the U73 mask, CL58, CL37, ecliptic North and ecliptic South. The different colours represent the four component separation methods, namely {\tt C-R} (green), {\tt NILC} (blue), {\tt SEVEM} (red), and {\tt SMICA} (orange). }
\label{fig:npdf-masks}
\end{figure}

%TABLE FREQUENCY DEPENDENCE
\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Frequency dependence of the lower tail probablity for the $N$-pdf, using different masks.}
\label{tab:npdf-freq}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 1.6in{#\leaderfil}\tabskip=2pt&
\hbox to 0.45in{\hfil#\hfil}&\hbox to 0.45in{\hfil#\hfil}&\hbox to 0.45in{\hfil#\hfil}&\hbox to 0.45in{\hfil#\hfil}\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan4 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan4\hrulefill\cr
\omit\hfil Mask \hfil& 70\,GHz& 100\,GHz& 143\,GHz& 217\,GHz\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
U73, $f_{\rm sky}=78\%$& 0.037& 0.058& 0.013& 0.124\cr
CL58, $f_{\rm sky}=58\%$& 0.169& 0.123& 0.111& 0.169\cr
CL37, $f_{\rm sky}=37\%$& 0.422& 0.366& 0.376& 0.386\cr 
Ecliptic North, $f_{\rm sky}=39\%$& 0.028& 0.050& 0.015& 0.083\cr
Ecliptic South, $f_{\rm sky}=39\%$& 0.225& 0.233& 0.166& 0.330\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 
%FIGURE FREQUENCY DEPENDENCE
\begin{figure}
\centerline{
\includegraphics[width=88mm]{./section_4.0/section_4.2/section_4.2.2/figs/npdf_freq_1000sims_n0032.pdf}
}
\caption{Frequency dependence for 70\,GHz (green), 100\,GHz (blue), 143\,GHz (red), and 217\,GHz (orange), for different masks.}
\label{fig:npdf-freq}
\end{figure}












==> section_4.0/section_4.2/section_4.2.3/section_4.2.3.tex <==

We analyse the CMB estimates downgraded to \mbox{$N_{\rm
  side}=64$} and \mbox{$N_{\rm side}=512$} as well as at the original resolution of \mbox{$N_{\rm
  side}=2048$}. In the case of the analysis at \mbox{$N_{\rm
  side}=64$} the maps were additionally smoothed with FWHM of 165\arcmin\,(three times the pixel size for the downgraded map). Due to 
computational limitations, an analysis is possible on
the full sky only in the case of resolution \mbox{$N_{\rm side}=64$}.
For the higher resolution maps, we perform the analysis on
a set of non-overlapping discs. For \mbox{$N_{\rm side}=512$} we uniformly
retain, after masking, part of the sky with approximately $100$
discs of radius $10\deg$. Analogously to the analysis by \citet{eriksen2005}, we
consider two disc sets, A and B, with a relative offset between their grids such
that the centres of the discs of set B are located in parts of the sky not
covered by disc set A (see Fig.~\ref{fig:mask_discs}).
For studies at the original resolution
\mbox{$N_{\rm side}=2048$}, we restrict the analysis to 20 discs with a radius
of $3\deg$ located randomly on an unmasked part of the sky (\fig\ref{fig:mask_discs}).


\begin{figure}[h!tmb]
%\begin{center}
\centerline{
\includegraphics[width=\columnwidth,angle=180]{./section_4.0/section_4.2/section_4.2.3/figs/mask_discs_r10_aset_common_mask_dx9delta.pdf}
}
\vspace{0.2cm}
\centerline{
\includegraphics[width=\columnwidth,angle=180]{./section_4.0/section_4.2/section_4.2.3/figs/mask_discs_r10_bset_common_mask_dx9delta.pdf}
}
\vspace{0.2cm}
\centerline{
\includegraphics[width=\columnwidth,angle=180]{./section_4.0/section_4.2/section_4.2.3/figs/mask_discs_r3_common_mask_dx9delta_n2048.pdf}
}

\caption{Two sets of discs of radius 10\deg\ A (\textit{top}) and B (\textit{middle}),  for the
  $N_{\rm side}=512$  CMB estimates; and a set of 20 randomly placed discs of
  radius 3\deg\ super-imposed on the U73 mask (blue region)
  for the CMB estimates at $N_{\rm side}=2048$ (\textit{bottom}).}
\label{fig:mask_discs}
%\end{center}
\end{figure}


As in \citet{eriksen2005}, we consider the $N$-point correlation
functions averaged over the disc sets.  In order to minimize
correlations between the discs, we subtract from the maps at
resolutions $N_{\rm side}=512$ and $N_{\rm side}=2048$ the best-fit
multipoles computed for the ranges $\ell\leq 18$ and $\ell\leq 60$,
respectively. This procedure corresponds in practice to a high-pass filtering of the
maps. One consequence of
  this procedure is the reduced sensitivity of the method to diffuse
  Galactic foreground residuals, which contribute most significantly
  to the low order multipoles. However, such a contribution is tested for in the analysis at resolution
  $N_{\rm side}=64$, in which high-pass filtering is not employed
  beyond the  removal of the
  monopole and dipole.

In the case of the analysis of the maps at resolution \mbox{$N_{\rm
    side}=512$} the $N$-point correlation functions were averaged over
  all discs for a given set, as well as separately for discs as a
  function of Galactic latitude. Such analysis allows the
study of possible contamination of the maps by diffuse Galactic
foreground residuals distributed symmetrically around the Galactic plane.

The low resolution versions of the U73 mask described earlier were
used as required.  Residual monopole and dipole contributions were
then removed from the maps.

A simple $\chi^2$ test is chosen to quantify the degree
of agreement between the simulations and the observations, where
$\chi^2$  as usual is defined by
\begin{equation}
\chi^2 = \sum_{i,j=1}^{N_{\rm bin}} \left(C_N (\theta_i) -
  \bigl<C_N(\theta_i)\bigr> \right) M_{ij}^{-1} \left( C_N(\theta_j) -
\bigl<C_N(\theta_j)\bigr> \right) \ .
\label{eq:chisquare}
\end{equation}
Here $C_N(\theta_i)$ is the $N$-point correlation function for
the bin of separation angle, $\theta_i$ (corresponding to the length of
  the longest side for the pseudo-collapsed configuration and the length of
  the polygon's side for the equilateral triangle and rhombus), $\bigl<C_N(\theta_i)\bigr>$ is the
corresponding average from the Monte Carlo (MC) ensemble, and
\begin{equation}
M_{ij} = \frac{1}{N_{\rm sim}}\sum_{k=1}^{N_{\rm sim}}
\left( C^{(k)}_N(\theta_i) - \bigl<C_N(\theta_i)\bigr>\right) \left( C^{(k)}_N(\theta_j) -
  \bigl<C_N(\theta_j)\bigr> \right)
\end{equation}
is the covariance matrix. Although the inverse of the covariance matrix
constructed from MC simulations can be biased, it is relatively small for
1000 simulations and has a negligible impact on the significance levels estimated
from the simulations, as described below.

This statistic is optimized for studying Gaussian distributed
data. However, usually it also works quite well for mildly
non-Gaussian distributions, and in particular symmetric
ones. Nevertheless, as for any statistic constructed from MC simulations,
it can also be used for non-Gaussian and asymmetrically distributed
data. Below, we quote the significance level in terms of the fraction
of simulations with a larger $\chi^2$ value than the observed map.


We analyse the mask dependence of the non-Gaussianity of the maps
using the pseudo-collapsed 3-point correlation function. The low
  order multipoles were estimated and subtracted from the maps for
  each mask separately. These estimates thus depend on the specific sky
  coverage employed, so that the comparison of the
  correlation functions for different masks is non-trivial. The
function averaged over disc set A is shown in
Fig.~\ref{fig:npt_discs_mask}. The corresponding probabilities of
obtaining values of the $\chi^2$ statistic for the concordance $\Lambda$CDM
model at least as large as the observed values are given in 
Table~\ref{tab:prob_chisq_mask}.


\begin{figure}[htmp!]

%\centerline{
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9_raw_143GHz_discs_aset_r10.pdf}
%}
%\centerline{
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9_sevem_143GHz_discs_aset_r10.pdf}
%}
\centerline{
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9_raw_143GHz_discs_aset_r10.pdf}
}
\centerline{
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9_sevem_143GHz_discs_aset_r10.pdf}
}

\caption{Pseudo-collapsed 3-point function averaged over disc set
  A for the raw (upper figure) and {\tt SEVEM} foreground corrected
  (lower figure) 143\,GHz map at $N_{\rm side}=512$ for different values of sky coverage ($f_{\rm sky}$). Estimates of the
  multipoles for $\ell \leq 18$ are removed from the sky maps. The
  black solid line indicates the mean for 1000 MC simulations and the
  shaded dark and light grey regions indicate the 68\% and 95\%
  confidence regions, respectively, for the CG90 ($f_{\rm sky}=0.9$)
  mask. See Sect.~\ref{sec:npoint_correlation} for the definition of the separation angle $\theta$.}
\label{fig:npt_discs_mask}
\end{figure}


\begin{table}[h!tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Probabilities of obtaining values of the $\chi^2$ statistic
  for the concordance $\Lambda$CDM model at least as
  large as the observed values of the statistic for the raw 143 GHz
  (first row) and foreground corrected 143\,GHz {\tt SEVEM} CMB maps (second row). In this table $f_{\rm sky}$ is the fraction of unamasked pixels.}
\label{tab:prob_chisq_mask}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{$<$} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 1.1in{#\leaderfil}\tabskip=3pt&
\hbox to 0.5in{\hfil#\hfil}&\hbox to 0.5in{\hfil#\hfil}&\hbox to 0.5in{\hfil#\hfil}&\hbox to 0.5in{\hfil#\hfil}\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan4 \hfil Probability\hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan4\hrulefill\cr
\omit\hfil Map \hfil& $f_{\rm sky}=0.6$& $f_{\rm sky}=0.7$& $f_{\rm sky}=0.8$& $f_{\rm sky}=0.9$\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
Raw& 0.907& 0.889& 0.563& $<$0.001\cr
{\tt SEVEM}& 0.959& 0.959& 0.905& !0.940\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 
In summary, the pseudo-collapsed 3-point function does not show any
significant deviation from Gaussianity for the raw 143\,GHz map masked
with the CG60 ($f_{\rm sky}=0.6$) and CG70 ($f_{\rm sky}=0.7$) masks. To a lesser
extent, this is true also for the CG80 ($f_{\rm sky}=0.8$) mask. We do not see
any significant deviation for any of the analysed masks after cleaning
the 143\,GHz map using the {\tt SEVEM} method.


The correlation functions for the four component separation methods
and resolution parameters $N_{\rm side}=64$, $N_{\rm side}=512$ and
$N_{\rm side}=2048$ are shown in 
Fig.~{\ref{fig:npt_n64}, Fig.~\ref{fig:npt_aset_n512} (disc set A),
Fig.~{\ref{fig:npt_bset_n512} (disc set B). and Fig.~{\ref{fig:npt_n2048}, respectively.
The probabilities of obtaining values of the $\chi^2$
statistic for the \Planck\ fiducial $\Lambda$CDM model at least as 
large as the observed values are given in the
Tables~\ref{tab:prob_chisq_n64},  \ref{tab:prob_chisq_n512}, and
\ref{tab:prob_chisq_n2048}, respectively. In addition, 
Table~\ref{tab:prob_chisq_n512_rings} reports the probabilities for
  the $N$-point functions averaged over sets of discs as a function of
  Galactic latitude for the {\tt SMICA} map at $N_{\rm side}=512$. 


\begin{figure*}[htpm!]
\begin{center}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/twopt_temp_dx9delta_common_mask_n64.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9delta_common_mask_n64.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/threept_eq_temp_dx9delta_common_mask_n64.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/fourpt_red_temp_dx9delta_common_mask_n64.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/twopt_temp_dx9delta_common_mask_n64.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9delta_common_mask_n64.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/threept_eq_temp_dx9delta_common_mask_n64.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/fourpt_red_temp_dx9delta_common_mask_n64.pdf}

\caption{The 2-point (upper left), pseudo-collapsed (upper right),
  equilateral (lower left) 3-point and reduced rhombic 4-point (lower right)
  functions for the $N_{\rm side}=64$ CMB
  estimates. The black solid line indicates the mean for 1000 Monte Carlo
  simulations and the shaded dark and light grey regions indicate the 68\% and 95\%
  confidence regions, respectively. See
    Sect.~\ref{sec:npoint_correlation} for the definition of the separation angle $\theta$.} 
\label{fig:npt_n64}
\end{center}
\end{figure*}


\begin{figure*}[htmp!]
\begin{center}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/twopt_temp_dx9delta_discs_aset_r10_common_mask.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9delta_discs_aset_r10_common_mask.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/threept_eq_temp_dx9delta_discs_aset_r10_common_mask.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/fourpt_red_temp_dx9delta_discs_aset_r10_common_mask.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/twopt_temp_dx9delta_discs_aset_r10_common_mask.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9delta_discs_aset_r10_common_mask.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/threept_eq_temp_dx9delta_discs_aset_r10_common_mask.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/fourpt_red_temp_dx9delta_discs_aset_r10_common_mask.pdf}

\caption{The 2-point (upper left), 
 pseudo-collapsed (upper right), equilateral (lower left) 3-point
 and reduced rhombic 4-point (lower right) 
  functions averaged over disc set A for the $N_{\rm side}=512$ CMB
  estimates. Estimates of the
  multipoles for $\ell \leq 18$ are removed from the sky maps.
  The black solid line indicates the mean for 1000 Monte Carlo
  simulations and the shaded dark and light grey regions indicate the 68\% and 95\%
  confidence regions, respectively. See
    Sect.~\ref{sec:npoint_correlation}  for the definition of the separation angle $\theta$.}  
\label{fig:npt_aset_n512}
\end{center}
\end{figure*}

\begin{figure*}[htmp!]
\begin{center}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/twopt_temp_dx9delta_discs_bset_r10_common_mask.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9delta_discs_bset_r10_common_mask.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/threept_eq_temp_dx9delta_discs_bset_r10_common_mask.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/fourpt_red_temp_dx9delta_discs_bset_r10_common_mask.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/twopt_temp_dx9delta_discs_bset_r10_common_mask.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9delta_discs_bset_r10_common_mask.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/threept_eq_temp_dx9delta_discs_bset_r10_common_mask.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/fourpt_red_temp_dx9delta_discs_bset_r10_common_mask.pdf}

\caption{As Fig.~\ref{fig:npt_aset_n512} for disc set B.}  
\label{fig:npt_bset_n512}
\end{center}
\end{figure*}



\begin{figure*}[htmp!]
\begin{center}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/twopt_temp_dx9delta_discs_r3_common_mask_n2048.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9delta_discs_r3_common_mask_n2048.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/threept_eq_temp_dx9delta_discs_r3_common_mask_n2048.pdf}
%\includegraphics[width=8cm]{./section_4.0/section_4.2/section_4.2.3/figs/fourpt_red_temp_dx9delta_discs_r3_common_mask_n2048.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/twopt_temp_dx9delta_discs_r3_common_mask_n2048.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/threept_coll_temp_dx9delta_discs_r3_common_mask_n2048.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/threept_eq_temp_dx9delta_discs_r3_common_mask_n2048.pdf}
\includegraphics[width=\columnwidth]{./section_4.0/section_4.2/section_4.2.3/figs/fourpt_red_temp_dx9delta_discs_r3_common_mask_n2048.pdf}

\caption{The 2-point (upper left), 
 pseudo-collapsed (upper right), equilateral (lower left) 3-point
 and reduced rhombic 4-point (lower right) 
  functions averaged over the disc set for the $N_{\rm side}=2048$ CMB
  estimates. Estimates of the
  multipoles for $\ell \leq 60$ are removed from the sky maps.
  The black solid line indicates the mean for 1000 Monte Carlo
  simulations and the shaded dark and light grey regions indicate the 68\% and 95\%
  confidence regions, respectively. See
    Sect.~\ref{sec:npoint_correlation} for the definition of the separation angle $\theta$.}  
\label{fig:npt_n2048}
\end{center}
\end{figure*}

\begin{table}[tmp] 
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Probabilities of obtaining values for the $\chi^2$ statistic
  of the $N$-point functions shown in Fig.~\ref{fig:npt_n64} for the
  \Planck\ fiducial $\Lambda$CDM model at least as
  large as the observed values of the statistic for the \Planck\ CMB
  maps with resolution parameter $N_{\rm side}=64$, estimated 
  using the {\tt C-R}, {\tt NILC}, {\tt SEVEM}
  and {\tt SMICA} methods.}
\label{tab:prob_chisq_n64}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 1.6in{#\leaderfil}\tabskip=3pt&
\hbox to 0.38in{\hfil#\hfil}&\hbox to 0.38in{\hfil#\hfil}&\hbox to 0.38in{\hfil#\hfil}&\hbox to 0.38in{\hfil#\hfil}\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan4 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan4\hrulefill\cr
\omit \hfil Function \hfil& {\tt  C-R}& {\tt NILC}& {\tt SEVEM}& {\tt SMICA}\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
Two-pt.& 0.883& 0.859& 0.884& 0.855\cr
Pseudo-coll. three-pt.& 0.922& 0.918& 0.945& 0.908\cr
Equil. three-pt.& 0.962& 0.966& 0.978& 0.968\cr
Four-pt.& 0.975& 0.977& 0.979& 0.977\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 

\begin{table}[h!tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Probabilities of obtaining values of the $\chi^2$ statistic
  of the $N$-point functions shown in Figs.~\ref{fig:npt_aset_n512} and
  \ref{fig:npt_bset_n512} for the \Planck\ fiducial $\Lambda$CDM model at least as
  large as the observed values of the statistic  for \Planck\ CMB
  maps with resolution parameter $N_{\rm side}=512$. estimated using 
  the {\tt C-R}, {\tt NILC}, {\tt SEVEM}
  and {\tt SMICA} methods.
 }
\label{tab:prob_chisq_n512}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 0.9in{#\leaderfil}\tabskip=3pt&
\hbox to 0.36in{\hfil#\hfil}&\hbox to 0.36in{\hfil#\hfil}&\hbox to 0.36in{\hfil#\hfil}&\hbox to 0.36in{\hfil#\hfil}\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan4 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan4\hrulefill\cr
\omit\hfil Set \hfil& {\tt C-R}& {\tt NILC}& {\tt SEVEM}& {\tt SMICA}\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
\multispan5 \hfil Two-pt. \hfil\cr
\noalign{\vskip 2pt}
%\noalign{\vskip 3pt\hrule\vskip 3pt}
A& 0.858& 0.902& 0.886& 0.904\cr
B& 0.351& 0.370& 0.404& 0.376\cr
\noalign{\vskip 3pt}
\multispan5 \hfil Pseudo-coll. three-pt.  \hfil\cr
\noalign{\vskip 2pt}
A& 0.568& 0.565& 0.651& 0.603\cr
B& 0.483& 0.526& 0.550& 0.540\cr
\noalign{\vskip 3pt}
\multispan5 \hfil Equilateral three-pt. \hfil\cr
\noalign{\vskip 2pt}
A& 0.004& 0.032& 0.045& 0.043\cr
B& 0.452& 0.485& 0.443& 0.479\cr
\noalign{\vskip 3pt}
\multispan5 \hfil Four-pt. \hfil\cr
\noalign{\vskip 2pt}
A& 0.104& 0.102& 0.102& 0.107\cr
B& 0.521& 0.569& 0.537& 0.579\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 


\begin{table}[h!tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{ Probabilities of obtaining values of the $\chi^2$ statistic
  of the $N$-point functions shown in Figs.~\ref{fig:npt_aset_n512} and
  \ref{fig:npt_bset_n512} for the \Planck\ fiducial $\Lambda$CDM model at least as
  large as the observed values for {\tt SMICA}  at $N_{\rm side}=512$. The analysis was performed separately for
  every set of discs centred on the Galactic latitudes with the  same absolute
  value. The Galactic latitudes of the disc centres are given in the
  first two rows of the table.
 }
\label{tab:prob_chisq_n512_rings}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{$<$} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 0.9in{#\leaderfil}\tabskip=3pt&
\hbox to 0.36in{\hfil#\hfil}&\hbox to 0.36in{\hfil#\hfil}&\hbox to 0.36in{\hfil#\hfil}&\hbox to 0.36in{\hfil#\hfil}&\hbox to 0.36in{\hfil#\hfil}\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan5 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit\hfil Set \hfil&\multispan5\hrulefill\cr
A & $\pm90\deg$& $\pm70\deg$& $\pm50\deg$&$\pm30\deg$& $\pm10\deg$\cr
B & $\pm80\deg$& $\pm60\deg$& $\pm40\deg$& $\pm20\deg$& !*$0\deg$\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
\multispan6 \hfil Two-pt. \hfil\cr
\noalign{\vskip 2pt}
%\noalign{\vskip 3pt\hrule\vskip 3pt}
A & 0.057 & 0.672 & 0.780 & 0.594 & !0.556\cr
B& 0.158 & 0.401 & 0.741 & 0.667 & $<$0.001 \cr
\noalign{\vskip 3pt}
\multispan6 \hfil Pseudo-coll. three-pt.  \hfil\cr
\noalign{\vskip 2pt}
A& 0.006 & 0.669 & 0.153 & 0.414 & !0.783\cr
B& 0.014 & 0.211 & 0.639 & 0.763 & !0.240\cr
\noalign{\vskip 3pt}
\multispan6 \hfil Equilateral three-pt. \hfil\cr
\noalign{\vskip 2pt}
A& 0.083 & 0.922 & 0.161 & 0.086 & !0.082\cr
B& 0.956 & 0.800 & 0.827 & 0.288 & $<$0.001\cr
\noalign{\vskip 3pt}
\multispan6 \hfil Four-pt. \hfil\cr
\noalign{\vskip 2pt}
A& 0.014 & 0.390 & 0.324 & 0.492 & $<$0.001\cr
B& 0.098 & 0.920 & 0.987 & 0.537 & $<$0.001\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 


\begin{table}[h!tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Probabilities of obtaining values of the $\chi^2$ statistic
  of the N-point functions shown in Fig.~\ref{fig:npt_n2048} for the
  \Planck\ fiducial $\Lambda$CDM model at least as
  large as the observed values of the statistic  for \Planck\ CMB
  maps with resolution parameter $N_{\rm side}=2048$ estimated 
  using the {\tt C-R}, {\tt NILC}, {\tt SEVEM},
  and {\tt SMICA} methods.
}
\label{tab:prob_chisq_n2048}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 1.5in{#\leaderfil}\tabskip=2pt&
\hbox to 0.35in{\hfil#\hfil}&\hbox to 0.35in{\hfil#\hfil}&\hbox to 0.35in{\hfil#\hfil}&\hbox to 0.35in{\hfil#\hfil}\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan4 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan4\hrulefill\cr
\omit\hfil Function \hfil& {\tt C-R}& {\tt NILC}& {\tt SEVEM}& {\tt SMICA}\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
Two-pt.& 0.335& 0.474& 0.573& 0.497\cr
Pseudo-coll. three-pt.& 0.522& 0.463& 0.469& 0.448\cr
Equil. three-pt.& 0.853& 0.789& 0.819& 0.796\cr
Four-pt.& 0.532& 0.534& 0.579& 0.526\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 


The results show consistency between the CMB maps estimated using
the different component separation methods. No statistically
significant deviations of the CMB maps from Gaussianity are found on
any scale, with the exception of some analyses performed
  on sets of discs centred at low Galactic latitudes. However, for
  disc set B the fraction of such
  discs available
  for analysis after masking is very small, reducing the robustness of
  the results. A more intriguing case with very small probability
  arises for the disc set A 4-point function averaged over discs centred at Galactic
  latitude $\pm$10$^\circ$. The fraction of  discs
  available for the analysis is much larger in this case than for
  disc set B, and may
  indicate the presence of Galactic emission residuals. 

It is also worth noticing that the CMB map smoothed and
downgraded to $N_{\rm side}=64$ show the largest deviation, with a
  tendency towards super-Gaussianity, especially
for the 4-point correlation function, in
comparison to the intermediate and small angular 
scale analyses. Since the CMB maps at this
  resolution were not high-pass filtered, they may be more susceptible
  to Galactic foreground residual artefacts that survive the component
  separation processes.



==> section_4.0/section_4.2/section_4.2.4/section_4.2.4.tex <==
By combining the MFs curves into a vector $\vec{y}$ of size $~n=~n_{\rm
  thresholds}\times n_{\rm functionals}$, a null hypothesis test can
be performed using a $\chi^2$ statistic given by
%
\begin{equation}
\chi^2( \vec{y}) = ( \vec{y} - \langle\vec{y}_{\rm G}\rangle)^{\rm T} \tens{C}^{-1} ( \vec{y} -\langle\vec{y}_{\rm G}\rangle)
\label{eq:chi_mf}
\end{equation}
%
where $\vec{y}$ represents the MFs of the data, $\vec{y}_{\rm G}$ those of
the simulations and $\tens{C}$ is the covariance matrix. In order to assure
convergence, in the case of the four normalized MFs $\tens{C}$ is estimated
from $10^4$ Gaussian simulations, drawn from the \Planck\ fiducial
power spectrum, having the same instrumental properties of effective
beam and noise as the data, the same applied mask and which have
been processed in the same way to reach the corresponding
resolution. For the three unnormalized MFs, $\tens{C}$ was estimated from only
$10^3$ FFP6 simulations that proved to be sufficient for convergence.
We compare the $\chi^2_{\rm Planck}$ value obtained from
the data to the $\chi^2$ obtained from those simulations, and report
the probability of having a value of $\chi^2$ larger than the measured
one, $P \left( \chi^2> \chi^2_{\rm Planck}\right)$. We explore different
resolutions represented by the parameter $N_{\rm side}$, different
methods of component separation (\crul, \nilc, \sevem, and \smica) and
different sky coverages.

First, the three unnormalized MFs ($V_k$ as a function of $\nu$,
$k=0,\,1,\,2$) are used to construct a test of the null hypothesis.
The test assesses not only the primordial Gaussian hypothesis, but
also whether the data is correctly represented by the simulations in
terms of power spectrum, systematics and the lensing effect.
A set of $17$ thresholds in units of $T/\sigma_{\rm 0}$ between $-4$ and $+4$ in steps of $0.5$ are
considered.  The comparison between the MFs of the data provided by
the four component separation methods and those corresponding to each
of the four sets of $10^3$ FFP6 simulations representing each method,
for the standard U73 mask, are shown in
Fig.~\ref{fig:minkplots_cs}.  From that figure, a deviation at
a level of about $2\sigma$ can be seen for the contour and genus
curves at a resolution $N_{\rm side} =512$. The situation is very similar for
the analyses performed at other resolutions, $N_{\rm side} =1024$, 256
and 128. Although the deviation is not particularly compelling, because of the correlations 
among neighbouring thresholds, it is worth mentioning that a possible explanation 
is the background of
unresolved sources that has been detected in \Planck\ data with the
bispectrum estimators (see~\cite{planck2013-p09a}). In order to
understand the effect of unresolved sources on the MFs, we added the
point source residuals derived from the FFP6 simulations
as processed by the {\tt SEVEM} algorithm to 100 realizations which
were then analysed.
We conclude that the background of unresolved sources
may be responsible for at least part of the excess signal that is detected.
The corresponding probabilities $P\left( \chi^2> \chi^2_{\rm Planck}\right)$
derived from the MF values for each of the four component
separation methods and resolutions are given in
Table~\ref{tab:mfschi2_nside_compsep}.  The full resolution maps have been degraded to the
lower resolution ones following the procedure described in Sect.~\ref{sec:data}. All the cases considered are
compatible with the null hypothesis.
%
%\begin{figure*}[h!]
\begin{figure}[h!]
\begin{center}
\includegraphics[width=8cm]{./section_4.0/section_4.2/figs/areaDiff_512_LT.pdf}
\includegraphics[width=8cm]{./section_4.0/section_4.2/figs/contourDiff_512_LT.pdf}
\includegraphics[width=8cm]{./section_4.0/section_4.2/figs/genusDiff_512_LT.pdf}
%
\caption{ Difference of the data MFs (unnormalized) with respect to
  the average of the curves obtained with realistic \Planck\ simulations
  for several cleaned maps. From top to bottom: Area, Contour, Genus.
  The error-bars represent the $\pm1\sigma$ (68\%\,CL) dispersions around the
  mean obtained with simulations.}
%
\label{fig:minkplots_cs}
\end{center}
\end{figure}
%\end{figure*}
%
\begin{table}[h!tmb]  % use table for a one-column table 
%\begin{table*}[tmb]	% use table* for a two-column table 
\begingroup	% this + \endgroup at the end keep table things local 
\newdimen\tblskip \tblskip=5pt 
\caption{Non-directional Gaussianity tests using unnormalized MFs: $P\left( \chi^2>\chi^2_{\rm Planck}\right)$ as a function of sky resolution for different component separation methods.} 
\label{tab:mfschi2_nside_compsep}
\nointerlineskip 
\vskip -3mm 
\footnotesize  % good font size for a table, but can be changed 
\setbox\tablebox=\vbox{ 
\halign{\hbox to 0.8in{#\leaderfil}\tabskip=1pt&
\hfil#\hfil&\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan4 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan4\hrulefill\cr
\omit\hfil Method \hfil& \hfil $N_{\rm side}=1024$ \hfil& \hfil $N_{\rm side}=512$ \hfil& \hfil $N_{\rm side}=256$ \hfil& \hfil $N_{\rm side}=128$\hfil\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
\cru& 0.812& 0.299& 0.482& 0.357\cr % table lines go here. 
\noalign{\vskip 3pt}
\nilc& 0.993& 0.567& 0.354& 0.234\cr % table lines go here. 
\noalign{\vskip 3pt}
\sevem& 0.925& 0.911& 0.738& 0.094\cr % table lines go here. 
 \noalign{\vskip 3pt}
\smica& 0.874& 0.675& 0.426& 0.213\cr % table lines go here. 
\noalign{\vskip 3pt\hrule\vskip 3pt}}} %
\endPlancktable		% for a one-column table; defined in Planck.tex. %\endPlancktablewide	% for a two-column table; defined in Planck.tex.
\endgroup %
\end{table}
%\end{table*}
%

In the second case, the four normalized MFs $v_k=V_k/A_k$
($k=0,\,1,\,2,\,3$) are used for the null hypothesis test. 
A set of 26 thresholds equally spaced between $-3.5$ and
$+3.5$, in units of $T/\sigma_{\rm 0}$, are considered. The normalization factor $A_k$ is estimated
directly from the maps, having previously computed the moments $\sigma_0$
and $\sigma_1$.  This normalization minimizes the dependence
of the MFs on the power spectrum, thereby decreasing the cosmic variance and
improving their sensitivity to deviations from Gaussianity.  The
resolutions considered in this case are
$N_{\rm side}=2048,1024,512,256$, and $128$.  For the highest resolution $N_{\rm
  side}=2048$, the map is smoothed with a Gaussian smoothing kernel
with a width $\theta_{\rm FWHM}=5\arcm$, in order to decrease the
noise level. We use the standard U73 mask, inpainting the smallest
point sources. The maps at lower resolution are constructed by the 
standard simple degrading process applied to the original map at $N_{\rm
  side}=2048$, and the corresponding masks are degraded 
following a conservative
procedure such that any degraded pixel with a value $<0.8$ is set to
zero (as explained in Sect.~\ref{sec:data}).  The results of the analysis performed on the {\smica} map at
different resolutions are presented in Table~\ref{tab:mfschi2_nside}.
%
\begin{table}[h!tmb]
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Non-directional Gaussianity tests using normalized Minkowski Functionals: dependence of $P\left( \chi^2>\chi^2_{\rm Planck}\right)$ on resolution.}
\label{tab:mfschi2_nside}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth
   \setbox0=\hbox{\rm 0}
   \digitwidth=\wd0
   \catcode`*=\active
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth
   \setbox0=\hbox{+}
   \signwidth=\wd0
   \catcode`!=\active
   \def!{\kern\signw
idth}
\halign{\hbox to 0.8in{#\leaderfil}\tabskip=1pt&\hfill#\hfill\/\tabskip=0pt\cr                          
\noalign{\doubleline}
   % Table headings go here.
%\noalign{\vskip 3pt\hrule\vskip 5pt}
%\halign{#\hfil\tabskip=2em &\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\tabskip=0pt\cr
%\noalign{\doubleline} \cr
\omit\hfil $N_{\rm side}$\hfil&  Probability\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
2048& 0.358\cr
1024& 0.356\cr
512& 0.245\cr
256& 0.225\cr
128& 0.223\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
%\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable % this command is defined in Planck.tex.
\endgroup
\end{table}
%
The results of the analysis performed on the different component
separation methods at the highest resolution ($N_{\rm side}=2048$) are
presented in Table~\ref{tab:mfschi2_compsep}. The difference of the normalized MFs
with respect to the expected values of the null hypothesis
as a function of the threshold $\nu$ are shown in
Fig.~\ref{fig:minkplots_compsep}. A slight deviation in $N_{\rm cluster}(\nu)$ is noticeable at 
thresholds $\nu\approx 0$, however it is not very compelling, since the values at neighboring 
thresholds are very correlated and this correlation is taken into account in the $\chi^2$ statistics.
%
\begin{table}[h!tmb]
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Non-directional Gaussianity tests using normalized Minkowski Functionals: dependence of $P\left( \chi^2>\chi^2_{\rm Planck}\right)$ on component separation method.}
\label{tab:mfschi2_compsep}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth
   \setbox0=\hbox{\rm 0}
   \digitwidth=\wd0
   \catcode`*=\active
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth
   \setbox0=\hbox{+}
   \signwidth=\wd0
   \catcode`!=\active
   \def!{\kern\signw
idth}
\halign{\hbox to 0.8in{#\leaderfil}\tabskip=1pt&\hfill#\hfill\/\tabskip=0pt\cr                          
\noalign{\doubleline}
   % Table headings go here.
%\noalign{\vskip 3pt\hrule\vskip 5pt}
%\halign{#\hfil\tabskip=2em &\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\tabskip=0pt\cr
%\noalign{\doubleline} \cr
\omit\hfil Method\hfil&  Probability\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
\cru\ & 0.288\cr
\nilc\ & 0.303\cr
\sevem\ & 0.415\cr
\smica\ & 0.358\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
%\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable % this command is defined in Planck.tex.
\endgroup
\end{table}
\begin{figure*}[h!]
\begin{center}
\includegraphics[width=18cm]{./section_4.0/section_4.2/figs/smica_diff_allmfs_compsep.pdf}
%
\caption{ Difference of the normalized MFs obtained from the data with
  respect to the expected values of the null hypothesis, for the
  different component separation methods. From left to right and top
  to bottom: Area, Contour, Genus and $N_{\rm cluster}$.  The grey
  bands represent the $\pm1$ and $\pm2\sigma$ dispersions around zero, based on
  realistic \Planck\ simulations including lensing, for the \cru\ method.}
%
\label{fig:minkplots_compsep}
\end{center}
\end{figure*}
%
Finally, we analyse the dependence of the normalized MFs on the sky
coverage. We use the standard U73 mask 
and then decrease the sky coverage by using 
CL65, CL48 and CL25 masks in combination with a special point source mask that is based on the U73 mask. The fraction of sky left unmasked in the combined masks is 62\%, 46\% and 23\%, respectively.
The point source mask is inpainted previously to the analysis. 
The curves obtained for the
different sky coverages are presented in
Fig.~\ref{fig:minkplots_fsky}, for the {\tt SMICA} method.  Results of
the $\chi^2$ analysis of the data as a function of sky coverage are
compiled in Table~\ref{tab:mfschi2_fsky}. All the cases considered 
are compatible with the null hypothesis.

In summary, we find that the data are globally consistent with the
primordial Gaussian hypothesis, and no strong deviation is found
between the data and realistic simulations for both the unnormalized and
normalized MFs.  We would like to remark that a certain level of
non-Gaussianity is expected from lensing and, in particular, from the
ISW-lensing signal, thus it is important to compare the data to
realistic \textit{lensed} simulations.
%
\begin{table}[h!tmb]
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Non-directional Gaussianity tests using normalized Minkowski Functionals: dependence of $P\left( \chi^2>\chi^2_{\rm Planck}\right)$ on sky coverage.}
\label{tab:mfschi2_fsky}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth
   \setbox0=\hbox{\rm 0}
   \digitwidth=\wd0
   \catcode`*=\active
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth
   \setbox0=\hbox{+}
   \signwidth=\wd0
   \catcode`!=\active
   \def!{\kern\signw
idth}
\halign{\hbox to 0.8in{#\leaderfil}\tabskip=1pt&\hfill#\hfill\/\tabskip=0pt\cr                          
\noalign{\doubleline}
   % Table headings go here.
%\noalign{\vskip 3pt\hrule\vskip 5pt}
%\halign{#\hfil\tabskip=2em &\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\tabskip=0pt\cr
%\noalign{\doubleline} \cr
\omit\hfil $f_{\rm sky}$ \hfil&  Probability\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
0.73& 0.358\cr
0.62& 0.042\cr
0.46& 0.670\cr
0.23& 0.780\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
%\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktable % this command is defined in Planck.tex.
\endgroup
\end{table}
\begin{figure*}[h!]
\begin{center}
\includegraphics[width=18cm]{./section_4.0/section_4.2/figs/smica_diff_allmfs_fsky.pdf}
%
\caption{ Difference of the normalized MFs obtained from the data with
  respect to the expected value of the null hypothesis for several sky
  coverages. The \smica\ map is considered. From left to right and top
  to bottom: Area, Contour, Genus and $N_{\rm cluster}$.  The grey
  bands represent the 1 and $2\sigma$ dispersions around zero, based on
  realistic \Planck\ simulations including lensing, for $f_{\rm
    sky}=0.23$.}
%
\label{fig:minkplots_fsky}
\end{center}
\end{figure*}



==> section_4.0/section_4.2/section_4.2.5/section_4.2.5.tex <==

The study of the moments of the distribution of the CMB temperature
fluctuations, as a function of the scale, is a standard approach to
test the null hypothesis. We have performed a full resolution
multi-scale analysis of the four CMB clean maps 
and computed the quantities
$\sigma_{\rm R}$, $S_{\rm R}$, and $K_{\rm R}$ from the SMHW
wavelet coefficients at 18 scales, $R = \lbrace$2, 4, 7, 14, 25, 50,
75, 100, 150, 200, 250, 300, 400, 500, 600, 750, 900, 1050$\rbrace$,
in arcminutes. These are compared to the standard \Planck\
simulations.

As explained in~\cite{vielva2004}, when
computing the SMHW coefficients of a masked data set,
artefacts are introduced close to the mask that degrade the
performance of any null hypothesis tests.
We therefore 
define a set of \emph{exclusion masks} such
that, at each scale, an extra region of the sky is excluded when
performing any statistical test. The exclusion mask for a
given scale $R$ is defined as follows: we build an auxiliary mask by
removing from the U73 mask all the features associated with compact
objects, and degrade this auxiliary mask to $N_{\rm side}=1024$
(imposing a restrictive cut); a first temporary mask is obtained by
extending the borders of this auxiliary mask by a distance of twice
$R$; a second temporary mask is obtained, first, by convolving the
auxiliary mask with the SMHW at that particular scale $R$ and, second,
by imposing that any pixel of that second temporary mask with an
absolute value lower than 0.1 is masked, whereas the remaining ones
are set to 1; the two temporary masks are multiplied to yield a single mask
that is upgraded to $N_{\rm side}=2048$; and  finally, the final exclusion
mask is obtained by multiplying this mask by the parent
U73 mask.

The comparison of the four CMB maps with the corresponding simulations
is summarized in Fig.~\ref{fig:smhw_moments}. The three panels show
(from left to right) the statistical significance of the standard
deviation, the skewness and the kurtosis (as a function of the SMHW
scale). The points represent the upper tail probability associated to
a given statistic, i.e., the fraction of the simulations that present
a value of a given statistic equal to or greater than the one obtained
for the data. 
In fact, we define a modified upper tail probability: if an upper tail
probability is larger than $0.5$, then a new quantity is defined as
$1$ minus that upper tail probability. Hence, this modified definition
of the upper tail probability is constrained between $10^{-3}$ (the
minimum value that can be imposed with 1\,000 simulations) and $0.5$.
%
\begin{figure*}[h!]
\begin{center}
\includegraphics[width=6cm]{./section_4.0/section_4.2/section_4.2.5/figs/smhw_p_value_std_mk1p00.pdf}
\includegraphics[width=6cm]{./section_4.0/section_4.2/section_4.2.5/figs/smhw_p_value_skw_mk1p00.pdf}
\includegraphics[width=6cm]{./section_4.0/section_4.2/section_4.2.5/figs/smhw_p_value_krt_mk1p00.pdf}
\caption{\label{fig:smhw_moments} Standard deviation (left), skewness
  (centre) and kurtosis (right) of the SMHW coefficients as a function
  of the wavelet scale $R$. Results are given for the four \Planck\
  CMB maps (green, {\tt Commander-Ruler}; light-blue, {\tt NILC}; red, {\tt
    SEVEM}; and yellow, {\tt SMICA}). Modified upper tail probabilities
  (mUTP, see text for details) are obtained by comparing with 1000
  simulations processed through the component separation pipelines.
  Squares represent modified upper tail probabilities that correspond
  to an actual upper tail probability above $0.5$; diamonds represent
  upper tail probabilities below $0.5$.
}
\end{center}
\end{figure*}
%
Overall, the agreement between the four CMB maps is quite good,
showing that all of them provide a consistent estimation of the true
CMB. However, several aspects need to be discussed. Let us clarify
that the differences among the CMB methods for small modified upper
tail probabilities are expected to be larger than for large modified
upper tail probabilities. This is because a small modified upper
tail probability is determined by a small number of simulations
and, therefore, has a relatively large error bar. In other words, the
tails of the distributions of the different statistics are quite
sparsely sampled.

We will distinguish between the small ($R \lesssim 10\arcmin$),
intermediate ($ 10\arcmin \lesssim R \lesssim 500\arcmin$), and large
($R \gtrsim 500\arcmin$) scale regimes. Let us focus on the three
statistics independently. We will highlight the most important
features and, afterwards, we will try to find an explanation for them.

\begin{itemize}
\item On the smallest scales, the four CMB maps show a
  dispersion in SMHW coefficients significantly larger than seen in the
  simulations. However on larger scales, the dispersion is
  systematically below the median of the simulations and, on scales of
  $R \approx 5^\circ$, the modified upper tail probability is approximately $0.015$.
\item Regarding the skewness, all  four maps yield a value that
  is significantly lower (with a modified upper tail probability of
  around $0.004$) than expected from the simulations in the
  small scale regime (except for the smallest one, where the deviation
  is around 0.07). The rest of the scales are fairly compatible
  with the null hypothesis.
\item The kurtosis is also smaller than expected in the small
  scale regime. Overall, the modified upper tail probability is
  about $0.03$. At scales of around 300\arcmin , an anomalously
  large value (modified upper tail probability of approximately 0.01) is
  found.
\end{itemize}

These results are compatible with the values reported for \textit{WMAP}
data \citep{vielva2004,cruz2005}, over the scales  common to both
experiments (i.e., $R > 10\arcmin$). In particular, the large
value of the kurtosis has been associated with the Cold Spot \citep{vielva2004}. We will return to this topic specifically
in Sect.~\ref{sec:cold_spot}. The low variance of
the wavelet coefficients was previously seen in \cite{vielva2004} and \cite{wiaux2008}.
In addition, the low dispersion at scales above a few degrees
is likely to be related to the low variance anomaly detected in
\textit{WMAP} \citep{monteserin2008,2011MNRAS.412.2383C}, that is also
seen in the \Planck\ data (see Sect.~\ref{sec:one_dimensional_moments}).

We have also studied the robustness of the results for different
masking scenarios. In particular, we have investigated variations in
the results when we adopt, as auxiliary masks to define the
exclusion masks, 
the two CG70 and CG60 masks removing 30\% and 40\% of the sky, respectively.
Note that the
auxiliary masks obtained from the U73 mask already cut around 20\%
of the sky. The corresponding results for the  {\tt SMICA} map are presented in
Fig.~\ref{fig:smhw_moments_robust}. 
The conclusions are similar for the other
CMB maps. 
%
\begin{figure*}
\begin{center}
\includegraphics[width=6cm]{./section_4.0/section_4.2/section_4.2.5/figs/smhw_p_value_std_smica.pdf}
\includegraphics[width=6cm]{./section_4.0/section_4.2/section_4.2.5/figs/smhw_p_value_skw_smica.pdf}
\includegraphics[width=6cm]{./section_4.0/section_4.2/section_4.2.5/figs/smhw_p_value_krt_smica.pdf}
\caption{\label{fig:smhw_moments_robust} Standard deviation (left),
  skewness (centre) and kurtosis (right) of the SMHW coefficients as a
  function of the wavelet scale $R$. Results are given for the {\tt
    SMICA} CMB map. Several masking scenarios are compared:
  red, CG60 mask (cutting out 40\% of the sky); green, CG70 mask
  (cutting out 30\% of the sky); and blue, U73 mask. The modified upper
  tail probabilities (\emph{mUTP}) are defined in the text.}
\end{center}
\end{figure*}
%
For the dispersion of the wavelet coefficients, we do not notice any
significant change in the anomalously high value obtained for the {\tt
  SMICA} map at the smallest scales 
However, some changes are observed at larger scales. In this regime,
it seems that the most significant deviation occurs for the CG70
mask (modified upper tail probability of around $0.005$), whereas
similar (and slightly less significant) modified upper tail
probabilities are obtained for both the U73 (modified upper tail
probability of approximately $0.015$) and the CG60 (modified upper tail
probability of about $0.01$) masks. A possible explanation for this
behaviour
would be that a less restrictive mask admits some residual
contamination from Galactic foregrounds, thus increasing the
dispersion of the wavelet coefficients, and artificially increasing
their inconsistency with the null hypothesis. In principle, the
larger the Galactic cut, the lower would be the dispersion of the
wavelet coefficients (assuming that some residual contamination of the
Galactic foregrounds is left) and, therefore, the smaller the upper
tail probability. However, as we already said, the modified upper tail
probability for the dispersion is higher for the CG60 mask than
for the CG70 mask. This apparent contradiction could be
resolved by accounting for
the larger sampling variance for smaller areas, which would
result in a lower significance for the anomaly.

The anomalous kurtosis at scales of $R \approx 300\arcmin$ shows
an overall stable modified upper tail probability of around $0.01$ --
$0.03$. In the small scale regime, the differences are better defined:
the smaller the mask, the more significant the deviation
(characterized by the low value of the kurtosis). In particular, the
modified upper tail probability associated with the CG60 mask is
0.001, around $0.009$ for CG70, and approximately $0.03$ for the U73
mask. A similar pattern is also observed for the skewness on these
scales,
although the three masks results in more similar upper tail
probabilities, between around $0.001$ and 0.007 (except for the
smallest scale).

It is therefore clear that there is some inconsistency between the CMB
data and the corresponding simulations. On intermediate scales, both
the low dispersion and the high kurtosis could be related to
previously known anomalies: the low variance and the Cold Spot.
On the smallest scales, the three statistics report a low upper tail
probability independently of the mask coverage --- it is important to
determine what this inconsistency is due to.
Besides the possibility that it is an intrinsic cosmological
signal, the non-Gaussianity could be caused either by instrumental
systematics or residual foreground contamination.

In the former case, we have considered whether the origin of the
signal could be related to properties of the noise that are
inadequately modelled by the simulations. In particular, we have
studied the statistical properties of the half-ring half-difference maps
generated by the four component separation algorithms as proxies for
the the noise present in the CMB maps. Although in detail there
are some discrepancies between these noise estimates and the simulated
ones, they are not compatible with the inconsistencies observed
between the CMB map and simulations. Therefore, a systematic effect
associated with the instrumental noise does not provide a satisfactory
explanation for the small-scale deviations.

In the latter case, an obvious candidate is due to the contribution
from residual unresolved point sources in the clean CMB maps. Although
the brightest point sources are masked, and the component separation
process itself can suppress the amplitude of the unresolved background
of point sources, some signal will remain. Indeed, in
\cite{planck2013-p09a} it has been determined that the bispectrum of
this contribution is clearly detected in the four CMB \Planck\ maps,
at a significance in excess of $4\sigma$. In addition, the dispersion
of the wavelet coefficients is higher than expected, which is also
compatible with the presence of an additional signal. We therefore
consider this as the most likely non-CMB explanation for the observed
signal.




==> section_4.0/section_4.2/section_4.2.6/section_4.2.6.tex <==

%\subsubsection{Scaling Indices}
{\bf Do we want to include SI results on masking etc, or just focus on
asymmetry and phase correlations later in the draft? }\\*

If required, material (all updated for latest
delta-DX9 and CompSep data) from \\*
\url{http://hfilfi.planck.fr/index.php/WG/MaskImpactOnNGDDX9?action=download&upname=mask_assess.pdf} \\*
\url{http://hfilfi.planck.fr/index.php/WG/AssessmentdDX9?action=download&upname=comp_sep_assess_dx9.pdf} \\*


==> section_4.0/section_4.2/section_4.2.7/section_4.2.7.tex <==
\def\lall{\ell_1 \ell_2 \ell_3}
\def\llist{\ell_1,\ell_2,\ell_3}
\def\kall{k_1k_2k_3}
\def\klist{k_1,k_2,k_3}
%
Modal, wavelet and binned bispectrum estimators filter the CMB map
with separable basis functions
%
\eq
Q_{ijk}(\llist) = q_i(\ell_1)\, q_j(\ell_2)\,  q_k(\ell_3) + \hbox{perms}\,,
\qe
%
to find the corresponding modal coefficients.  For appropriately
orthonormalized basis functions $Q_{ijk}(\llist)$, these coefficients
can be used to reconstruct the CMB bispectrum through a
signal-to-noise weighted expansion \citep{planck2013-p09a}. This
reconstruction method has been extensively validated, showing the
accurate recovery of CMB bispectra from non-Gaussian simulated maps,
and it has been applied to the \textit{WMAP} seven year data to
reconstruct the full 3D CMB bispectrum \citep{Fergusson:2010dm}.  To
quantify whether or not there is a model-independent deviation from
Gaussianity, we can consider the total integrated bispectrum.  By
summing over all multipoles, we use the integrated nonlinearity
parameter $\bar F_{\rm NL}$ defined
in \citet{planck2013-p09a}. For ideal Gaussian CMB maps, the quantity
$\bar F_{\rm NL}^2$ should obey a $\chi^2$-distribution with a mean
given by the number of degrees of freedom (the modes) $\mu = n_{\rm
max}$ and with a variance $\sigma^2 = 2n_{\rm max}$.  Assuming that
the three-point correlator is the leading non-Gaussian contribution,
then $\barFnl$ provides a blind test for the presence of any
integrated CMB bispectrum (once the expected two-point term is
subtracted).  We note that this is less sensitive than targeted
searches for particular bispectrum shapes.
%

First, we discuss reconstructions from the modal estimator which has
passed successfully through the full suite of non-Gaussian bispectrum
validation tests \citep[for further details about bispectrum
estimators, see][]{planck2013-p09a}.  We have applied this to
the \Planck\ temperature maps for the foreground-separation
techniques \nilc\, \sevem\ and \smica, using two alternative sets of
hybrid basis functions in order to cross-check results and identify
particular signal \citep{planck2013-p09a}.  As with all the
other bispectrum analyses based on spherical harmonic coefficients, we
used the U73 mask to which we applied inpainting.  Together with the
foreground separated maps, noise simulations were provided which were
used to calibrate the estimator's linear correction term and to
determine the variance.

The modal coefficients extracted from the \Planck\
\nilc, \sevem, and \smica\ 
maps show remarkable consistency between the different maps, with
shape cross-correlations better than 96\% and the overall amplitudes
to within 7\% agreement \citep[see corresponding figure
in][]{planck2013-p09a}. This demonstrates that the indendent
foreground separation techniques do not appear to be introducing
spurious non-Gaussianity. The corresponding quantity $\bar F_{\rm
NL}^2$ shows consistency with the null hypothesis
\citep{planck2013-p09a}.  Using the modal expansion, we have
reconstructed the full 3D \Planck\ bispectrum
\citep{planck2013-p09a} for \smica\ but also \nilc\ and
\sevem; the reconstructions are visually indistinguishable. 
%
\begin{figure}
\includegraphics[width=8.8cm]{./section_4.0/section_4.2/section_4.2.7/figs/WMAP_vs_Planck_recon.pdf}
\caption[\textit{WMAP} vs \Planck\ bispectra]{\small  Comparison
  between the \textit{WMAP} seven-year bispectrum signal (left)
  (\citep{Fergusson:2010dm}) and the low-$\ell$ signal of \Planck\
  (right) reconstructed from the {\tt SMICA} foreground-separated map
  (in both cases using polynomial modes).  The same basic patterns are
  observed in both bispectra, including an apparent central
  ``oscillatory'' feature. }
\label{fig:WMAPPlanck}
\end{figure}

In Fig.~\ref{fig:WMAPPlanck}, we show a comparison of the $\ell<
500$ \Planck\ bispectrum signal and that reconstructed from
the \textit{WMAP} seven-year data \citep{Fergusson:2010dm}.  Here for
consistency we show the \Planck\ signal using polynomial modes.
The \Planck\ signal pattern correlates well with the \textit{WMAP}
bispectrum obtained previously, despite the different domains used for
the modal analysis of the two different experiments.

Similarly to the modal bispectrum, a wavelet decomposition can be used
to reconstruct the bispectrum. Here we use the continuous,
non-orthogonal Spherical Mexican Hat
Wavelet~\citep[SMHW,][]{martinezgonzalez2002}.  Cubic moments
$q_{ijk}$ are defined in terms of the SMHW coefficients for three
different angular scales $R_i$, $R_j$,
$R_k$ \citep{curto:2009a,curto:2009b,curto:2010,curto:2011a,curto:2011b,curto:2012}. 
See \citet{planck2013-p09a} for more details on the implementation of
this wavelet estimator for \Planck\ data analysis. Considering the
covariance matrix of the $q_{ijk}$ moments,
$\tens{C} \equiv \langle \vec{q} \vec{q}^{\rm T} \rangle$, and its
eigenvector decomposition, $\tens{C} = \tens{R} \tens{D} \tens{R}^{\rm
T}$, with $\tens{R}$ the eigenvector matrix and $\tens{D}$ the
eigenvalue matrix, a new set of quantities
$\vec{y} \equiv \tens{D}^{-1/2}\tens{R}^{\rm T}\vec{q}$ is
defined. Considering the decorrelation produced by the convolution of
the SMHW on the temperature anisotropies and applying the central
limit theorem to the averages defined in $q_{ijk}$, then
these quantities are expected to have a nearly Gaussian
distribution. Therefore, the $\vec{y}$ quantities are nearly
multinormal and satisfy $\langle \vec{y}
\vec{y}^{\rm T} \rangle = \tens{I}$ and $\langle \vec{y} \rangle = \vec{0}$ \citep{curto:2011a}.

We have computed this reconstruction using the \Planck\ data and
compared with the null hypothesis (Gaussian \Planck\ simulations). The
considered data map is the resulting map after foreground cleaning
based on different cleaning procedures: \crul, \nilc, \sevem,
and \smica. The mask used is the U73 one (contrary to the modal reconstruction,
no inpainting of the point sources is made 
in this case). In Fig.~\ref{fig1:sect_wav_bisp_reconstr} the $\vec{y}$
statistics corresponding to the \Planck\ data are plotted and compared
with the 3$\sigma$ error-bars obtained with \Planck\ Gaussian
simulations. From the list of different $q_{ijk}$ statistics
corresponding to the 16 angular scales described
in \citet{planck2013-p09a}, there are 11, 4, 3, 3 statistics with
$|y_i| \ge 3$ (corresponding to \crul, \nilc, \sevem, and \smica,
respectively). The error-bars are obtained with \Planck\ simulations
for each type of component separation cleaned map. The error-bars of
the $y_i$ statistics for low indices $i$ are associated to large
scales where the $\tens{q}$ statistics have a less Gaussian-like shape.
The $\vec{y}$ statistics are combined into a $\chi^2$ test after a
principal component analysis with a threshold of $10^{12}$
\citep{curto:2011a} and compared with the $\chi^2$ statistics obtained 
from \Planck\ Gaussian simulations for each type of component
separation method (see Table~\ref{table:sect_wav_bisp_reconstr}). The
$\chi^2$ statistic corresponding to the data is compatible with the
values obtained from Gaussian simulations according to the cumulative
probability $P( \chi^2 \ge \chi^2_{\rm data} )$, as can be seen in 
Table \ref{table:sect_wav_bisp_reconstr}. Therefore the wavelet
bispectrum reconstruction does not detect a significant amplitude of
bispectrum in the considered data maps. Details on the constraints on
the amplitude of different bispectrum shapes are presented
in \citet{planck2013-p09a}.
%
\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{$\chi^2$ statistics based on the wavelet
  bispectrum reconstruction $y_{i}$ statistics for the foreground
  cleaned data map. Considered data map: combined map cleaned with
  \cru, \nilc, \sevem, and \smica.}  
\label{table:sect_wav_bisp_reconstr}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 1.3in{#\leaderfil}\tabskip=2pt&
\hfil#\hfil\tabskip=9pt&\hfil#\hfil\tabskip=4pt&\hfil#\hfil\tabskip=6pt&\hfil#\hfil\tabskip=6pt&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\omit\hfil Method \hfil& $\chi^2_{\rm data}$& DOF& $\langle \chi^2
\rangle$& $\sigma$& $P( \chi^2 \ge \chi^2_{\rm data} )$\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
{\tt C-R}& 874& 690& 740& 87& 0.074\cr
\nilc\ & 883& 682& 731& 83& 0.045\cr
\sevem\ & 858& 682& 731& 83& 0.070\cr
\smica\ & 878& 682& 732& 83& 0.058\cr
\noalign{\vskip 5pt\hrule\vskip 5pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 

\begin{figure}[h!]
\begin{center}
\includegraphics[width=\hsize]{./section_4.0/section_4.2/section_4.2.7/figs/yi_deltadx9.pdf}
%~~
\end{center}
\caption{Wavelet bispectrum reconstruction $y_{i}$
  statistics for the foreground cleaned \Planck\ data map. Considered
  data map: combined map cleaned with \cru, \nilc, \sevem\ and \smica. The
  solid yellow lines represent the 3$\sigma$ error-bars for \smica\
  (similar error-bars are obtained for \cru, \nilc, and \sevem\ maps).}
\label{fig1:sect_wav_bisp_reconstr}
\end{figure}
%



==> section_4.0/section_4.2/section_4.2.tex <==
\subsection{Results}

% 1pdf:
\input{./section_4.0/section_4.2/section_4.2.1/section_4.2.1}

% n-pdf
\input{./section_4.0/section_4.2/section_4.2.2/section_4.2.2}

% n-pt functions
\input{./section_4.0/section_4.2/section_4.2.3/section_4.2.3}

% Minkowski functionals
\input{./section_4.0/section_4.2/section_4.2.4/section_4.2.4}

% Wavelets
\input{./section_4.0/section_4.2/section_4.2.5/section_4.2.5}

% Scaling indices
%\input{./section_4.0/section_4.2/section_4.2.6/section_4.2.6}

% Bispectrum
\input{./section_4.0/section_4.2/section_4.2.7/section_4.2.7}



==> section_4.0/section_4.3/section_4.3.tex <==

\subsection{Validation}

{\bf Various validation tests could be considered here based on
  simulated noise maps, and the difference
  maps between surveys and half-rings to confirm that the tests are
  not sensitive to noise statistics or residual systematics. The
  dependency on cosmological model might also be explored. \\* 
  As an
  alternative, we can simply specify that such tests have been
  undertaken and state the impact (although they still need to be
  done).   \\*

  Other resources come from FFP6 analyses here (some of which may need
  to be repeated for the CompSep paper): \\*} 

\url{http://hfilfi.planck.fr/index.php/WG/FFP6cleanmapsfNLbispec#needlest} \\*
\url{http://hfilfi.planck.fr/index.php/WG/AssessmentFFP6?action=download&upname=MF_FFP6_Sims.pdf} \\*
\url{http://hfilfi.planck.fr/index.php/WG/AssessmentFFP6?action=download&upname=cmb_assessment_ffp6.pdf} \\*
\url{http://hfilfi.planck.fr/index.php/WG/AssessmentFFP6?action=download&upname=comp_sep_assess_ffp6.pdf} \\*





==> section_5.0/section_5.0.tex <==

\section{Intriguing inconsistencies -- \textit{WMAP} anomalies revisited.}
\label{sec:anomalies_revisited}

In the previous section, we established that the \Planck\ data
show little evidence for non-Gaussianity beyond that expected due to
the ISW-lensing effect (which is accounted for directly by
simulations) and contributions from residual unresolved point
sources. The exceptions are on large-angular scales, where features
consistent with various anomalies previously seen in the \textit{WMAP}
data have been observed. In this section, we explicitly consider
several of the most important anomalies detected in the \textit{WMAP}
data, namely the
quadrupole-octopole alignment (Sect.~\ref{sec:mode_alignment}), 
the low variance (Sect.~\ref{sec:anomalous_variance}), 
the hemispherical asymmetry (Sect.~\ref{sec:hemispherical_asymmetry}), 
phase correlations (Sect.~\ref{sec:scaling_indices}), 
%dipolar power modulation (Sect.~\ref{sec:dipolar_asymmetry}), 
power asymmetry (Sect.~\ref{sec:power_asymmetry}), 
dipolar modulation (Sect.~\ref{sec:dipolar_modulation}), 
generalized power modulation (Sect.~\ref{sec:BipoSH}), 
parity asymmetry (Sect.~\ref{sec:parity_asymmetry}), 
and the Cold Spot (Sect.~\ref{sec:cold_spot}).  
Each of these anomalies may represent different violations of the
fundamental properties of isotropy and/or Gaussianity in the CMB data
that are assumed for the estimation of the CMB power spectrum.

There is an ongoing debate about the significance of these anomalies
in the literature. A critical issue relates to the role of
a~posteriori choices --- whether interesting features in the data bias
the choice of statistical tests, or if arbitrary choices in the
subsequent data analysis enhance the significance of the features.
Indeed, the \textit{WMAP} team \citep{bennett2010} contends that the
anomalies are significantly over-interpreted due to such selections,
whilst other authors claim highly significant and robust detections.
Therefore, care must be taken to address the issue of significance,
since our analyses necessarily follow up tests of the previous \textit{WMAP}
investigations.  However, a careful and fair statistical treatment can
enable us to study possible links among the anomalies and to search for
a physical interpretation.
%\clearpage
%Mode alignment
\input{./section_5.0/section_5.1/section_5.1}


% low variance
\input{./section_5.0/section_5.2/section_5.2.1/section_5.2.1}

% n-point functions
\input{./section_5.0/section_5.2/section_5.2.2/section_5.2.2}

% scaling indices
\input{./section_5.0/section_5.2/section_5.2.3/section_5.2.3}

%Dipole Modulation
%\input{./section_5.0/section_5.3/section_5.3}

% Power asymmetry
\input{./section_5.0/section_5.3/section_5.3.1/section_5.3.1}

% Dipole modulation
\input{./section_5.0/section_5.3/section_5.3.2/section_5.3.2}

%BiPoSh
\input{./section_5.0/section_5.4/section_5.4}

%even-odd multipoles and parity
\input{./section_5.0/section_5.5/section_5.5}

%Cold Spot
\input{./section_5.0/section_5.6/section_5.6}

%interpretation
\input{./section_5.0/section_5.7/section_5.7}




==> section_5.0/section_5.1/section_5.1.tex <==
\subsection{Mode alignment}
\label{sec:mode_alignment}

\cite{Tegmark2003} first reported a significant alignment between the
orientation of the quadrupole and the octopole in the \textit{WMAP}
first year temperature data. We study this quadrupole-octopole
alignment in the \Planck\ data using 
the maximization of the angular momentum dispersion as described in 
\cite{Oliveira-Costa2004}.  Specifically, we determine the orientation of the
multipoles by finding the axis $\vec{n}$ around which the
angular momentum dispersion \be \sum_m m^2 |a_{\ell m}(\vec{n})|^2
\label{eq:ang_mom_disp}
\ee 
is maximized. Here, $a_{\ell m}(\vec{n})$ denotes the
spherical harmonic coefficients of the CMB map in a rotated
coordinate system with its $z$-axis in the $\vec{n}$-direction.
This definition of the multipole-orientation has been devised for
planar multipoles and is simply the direction perpendicular to the
plane in which most of the power of the multipole lies. It is thus
intuitive and easy to use. Note that the value of the statistic in
Eq.~(\ref{eq:ang_mom_disp}) is the same for $-\vec{n}$ as for
$\vec{n}$, i.e., the multipole orientation is only defined up
to a sign.

An alternative method, based on the multipole vector decomposition
of the data 
\citep{copi2004, schwarz2004, bielewicz2005, bielewicz2009},
has also been used to verify the robustness of the results
presented here, and excellent consistency is found.

Residual foregrounds (mostly on the Galactic plane) present in the
four \Planck\ CMB estimates could influence the reconstruction of the
low-order multipoles. However, when a mask is applied, the resulting
mode-coupling can also affect the reconstruction of the low-$\ell$
multipoles. Since our understanding of the relationship between the
size of the mask and the extent to which residual foregrounds and
mode-coupling can affect the result is incomplete, 
%  We therefore utilize Wiener-filtered maps computed from
we therefore utilize Wiener-filtered maps computed from the data to
which the U73 mask has been applied.  Specifically, we utilize the
same implementation of the Wiener filter as used in
\citet{planck2013-p09a}, i.e., a ``messenger'' method, as described by
\citet{elsner2013}.  A direct inversion method for masked data
\citep{efstathiou2004, bielewicz2004, bielewicz2013} is a possible
alternative, but the Wiener-filtered maps result in a significantly
smaller uncertainty in the reconstructed orientation of the
multipoles.

We search for the preferred orientation by explicitly rotating
the CMB map such that the $z$-axis pierces the centres of each of the low
resolution pixels defined at $N_{\rm side}=16$, and then subsequently
refine the search by testing the $N_{\rm side}=2048$ pixels that lie
within the preferred lower resolution pixel. The angular
resolution for the orientation of the multipoles is thus given by the
distance between the pixel centres of the $N_{\rm side}=2048$ map,
which is of order 1.94\arcmin.  Figure~\ref{fig:wf_smica} shows the
Wiener-filtered \smica\ CMB sky, with the corresponding
reconstruction of the quadrupole 
and octopole moments. The
reconstructed orientations are quite robust with respect to the
component separation method used for reconstructing the CMB.  The
significance of the alignment between the quadrupole and the octopole
is assessed from the scalar product of their orientations, compared to
values derived from the standard set of 1000 MC simulations.  The
orientation, the angular distance, the scalar-product between
quadrupole and octopole, and the probability of at least as strong an
alignment to occur in an isotropic universe, are summarized in Table
\ref{tab:quadrupole_octopole_align_ang_mom} for each CMB map. 

\begin{figure}[h!]
%\begin{center}
\centerline{
\includegraphics[width=\columnwidth]{./section_5.0/section_5.1/figs/wiener_filt_smica_amp400.pdf}
}
\vspace{0.2cm}
\centerline{
\includegraphics[width=\columnwidth]{./section_5.0/section_5.1/figs/wiener_filt_smica_amp35_l2.pdf}
}
\vspace{0.2cm}
\centerline{
\includegraphics[width=\columnwidth]{./section_5.0/section_5.1/figs/wiener_filt_smica_amp35_l3.pdf}
}
\caption{
  {\it Upper}: Wiener-filtered \smica\ CMB sky (temperature range
  $\pm$ 400 $\mu$K). 
  {\it Middle}: derived quadrupole  (temperature range $\pm$ 35 $\mu$K). 
  {\it Lower}: derived octopole (temperature range $\pm$ 35 $\mu$K). 
  The plus and star symbols indicate the axes of the quadrupole and octopole, respectively, around
  which the angular momentum dispersion is maximized. The diamond
  symbols correspond to the quadrupole axes after correction for the kinematic quadrupole. 
} 
\label{fig:wf_smica}
%\end{center}
\end{figure}

We find that, depending on the component separation method, the
quadrupole and octopole orientations are misaligned by an amount
between 9\deg\ and 13\deg. Such a range of results is reasonable
given the observed differences, typically of order 5$\microK$ in
amplitude at high Galactic latitudes, between the CMB estimates, as
shown in figures~5 and 6 of \citet{planck2013-p06}.
This then implies that it may not be possible to determine the
alignment with a precision of better than a few degrees, due to uncertainties
related to component separation.

Note that the misalignment determined from the \Planck\ data is larger
than the 3\deg\ reported\footnote{Although \citet{bennett2012}
used a variant on the estimator adopted in this paper, we also
find a 3\deg\ misalignment of the quadrupole and octopole
determined from the ILC map.} recently by \citet{bennett2012}
for the 9-year \emph{WMAP} ILC map. However, when considering the
plausible range of errors introduced by the covariance between the CMB
and foregrounds and their impact on the derived ILC map,
\citet{bennett2012} cite a median misalignment angle of 6\deg.

Finally, as noted by \citet{Tegmark2003}, the observed quadrupole
includes a contribution due to our motion relative to the CMB rest
frame. This kinematic quadrupole (hereafter KQ) has a well-defined
morphology and frequency dependence, as described in
\citet{kamionkowski2003}. The latter is of particular importance for
the HFI channels. \citet{schwarz2004} have demonstrated that
correcting for the KQ contribution can be relevant for the
evaluation of the significance of the alignment between the
cosmological quadrupole and octopole.  We therefore apply map-based
corrections to the {\tt NILC}, {\tt SEVEM}, and {\tt SMICA} maps,
taking into account both the weighted contributions of each
\textit{Planck} frequency to the final CMB maps and the
corresponding KQ scaling factors. Such corrections are possible for
these maps, since, unlike for {\tt Commander-Ruler}, the frequency
weights used to generate them do not vary locally on the scales of
interest.
As seen in Table~\ref{tab:quadrupole_octopole_align_ang_mom},
after KQ-correction the three estimates of the quadrupole-octopole
alignment are more consistent, with the misalignment angle
decreasing to approximately 8\deg, and the significance increasing
to 99\%.

\begin{table*}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Orientations of the quadrupole and octopole components
  extracted from the four \textit{Planck} CMB maps, as determined by a
  maximization of the angular momentum dispersion (see
  Eqn.~\ref{eq:ang_mom_disp}). 
  The absolute value of the
  scalar-product between the orientation vectors of the quadrupole 
  and the octopole are provided in the fifth column.
  For an isotropic universe, this is uniformly
  distributed on the interval $[0,1]$. The last column gives the
  probability for such an alignment (or stronger) to occur, as
  determined from the FFP6 simulations.
  Results computed after correction for the kinematic quadrupole (KQ)
  are denoted by ``KQ corrected''.  In practice, we multiply the usual
  expression for the angular dependence of the KQ
  \citep[see][]{kamionkowski2003} in the
  Rayleigh-Jeans regime by factors that account for both its frequency
  dependence and the relative contributions of the different
  \textit{Planck} frequencies to the component separated maps. 
  For {\tt NILC}, {\tt SEVEM}, and {\tt SMICA} these
  factors are 1.7, 1.5, and 1.7, respectively. 
}

\label{tab:quadrupole_octopole_align_ang_mom}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 1.5in{#\leaderfil}\tabskip=2pt&
\hfil#\hfil\tabskip=5pt&\hfil#\hfil\tabskip=5pt&\hfil#\hfil\tabskip=4pt&\hfil#\hfil\tabskip=4pt&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\omit\hfil Method  \hfil& ($l$,$b$) quadrupole [\deg]& ($l$,$b$) octopole [\deg]& Ang. distance [\deg]& Scalar product& Probability\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
{\tt C-R}& (228.2,60.3)& (246.1,66.0)& 9.80& 0.985& 0.019\cr
{\tt NILC}& (241.3,77.3)& (241.7,64.2)& 13.1& 0.974& 0.033\cr
{\tt SEVEM}& (242.4,73.8)& (245.6,64.8)& 9.08& 0.988& 0.016\cr
{\tt SMICA}& (238.5,76.6)& (239.0,64.3)& 12.3& 0.977& 0.032\cr
{\tt NILC, KQ corrected}& (225.6,69.7)& (241.7,64.2)& 8.35& 0.989& 0.011\cr
{\tt SEVEM, KQ corrected}& (228.3,68.3)& (245.6,64.8)& 7.69& 0.991& 0.009\cr
{\tt SMICA, KQ corrected}& (224.2,69.2)& (239.0,64.3)& 7.63& 0.991& 0.009\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table*} 



==> section_5.0/section_5.2/section_5.2.1/section_5.2.1.tex <==
\subsection{Variance, skewness, and kurtosis anomalies}
\label{sec:anomalous_variance}

A low value for the variance on the CMB sky was previously observed in
the \textit{WMAP} data by \citet{monteserin2008} and
\citet{2011MNRAS.412.2383C}, and confirmed for \Planck\ in
Sect.~\ref{sec:one_dimensional_moments}.  Furthermore, the effect has
also been seen in the wavelet analysis of
Sect.~\ref{sec:wavelet_statistics}, where the variance of the SMHW
coefficients is low at scales between 400 and 600 arcmin
(Fig. \ref{fig:smhw_moments}).  In addition, anomalous behaviour was
also observed for the skewness and kurtosis in low resolution maps at
$N_{\rm side}=16$. Here, we reassess these results and determine their
robustness to masking and data selection. The former will allow us to
determine whether a particular region is causing the anomalous
behaviour, whilst the latter can establish whether foreground
residuals could be responsible.

Table~\ref{tab:1pdf-masks} and Fig.~\ref{fig:1pdf-masks} present the
results for the variance, skewness and kurtosis determined from the
four CMB maps with the U73, CL58 and CL37 masks
applied. Results are also computed for data within the ecliptic
hemispheres surviving the U73 mask. The variance is low in all
cases, with only small differences in significance observed
for the different maps. Interestingly, the low
variance seems to be localized in the northern ecliptic hemisphere. Conversely,
anomalous values for the skewness and kurtosis only are apparent for the
southern ecliptic hemisphere.  

Since these results might be indicative of the presence of Galactic
foreground residuals near the Galactic plane, we analyse the
frequency dependence of the statistics as summarized in
Table~\ref{tab:1pdf-freq} and Fig.~\ref{fig:1pdf-freq}.
The variance shows little frequency dependence for the considered
masks and regions, whereas the
skewness and kurtosis show a moderate frequency dependence 
when the U73 mask is applied,
as also seen for the $N$-pdf analysis in Sect.~\ref{sec:n-pdf}. 
\citet{2011MNRAS.412.2383C} found that a small region of the sky
localized to both the ecliptic and Galactic south and near to the
Galactic plane (their so-called ``gp10'' region)
exhibited particularly high variance. Thus, since the skewness is
negative, we consider a prominent cold spot at $b=-8^\circ$, $l=
32^\circ$, partially masked by the Galactic plane. However, when
masking the seven coldest pixels of the spot, the significance of the
skewness and kurtosis only drops slightly, with lower tail
probabilities of approximately $0.03$ and $0.93$ respectively. If the
whole ``gp10'' region ($f_{\rm sky}=7\%$) is masked, the skewness and
kurtosis drop drastically and have lower tail probabilities of
approximately $0.30$ and $0.50$, respectively, whereas the variance is
highly significant since none of the 1000 simulations has a variance
below that of the data.  In order to check the possible leakage of Galactic
contamination due to the Gaussian smoothing applied to the low
resolution data, we repeated our calculations for the Wiener filtered
maps used in Sect.~\ref{sec:mode_alignment}, but found little variation to the
existing results. Therefore, it is unlikely that any leakage impacts
the estimators.



The incompatibility of the observed variance with simulations based on
a cosmological model that has been determined from the same data set
might appear puzzling at first, but can be understood as follows. The
map-based variance is dominated by contributions from large angular
scales on the sky, whilst the cosmological parameter fits are
relatively insensitive to these low-order $\ell$-modes, and are
instead largely dominated by scales corresponding to $\ell > 50$.
Thus, the best-fit spectrum in the context of a 6-parameter
$\Lambda$CDM model can have a mismatch with the data on these scales,
so that the corresponding simulations will not adequately capture the
dearth of power at low-$\ell$.  The results presented here do indeed
imply that the large-angular scale power is low relative to the
fiducial sky model.
In fact, when subtracting the quadrupole and octupole from both the
data and simulations outside the U73 mask, the results are more
consistent.  In this case, the lower tail probabilities for the
variance, skewness and kurtosis are $0.192$, $0.637$ and $0.792$,
respectively. This result was already found in
\citet{2011MNRAS.412.2383C}.
It is then plausible that the low multipole alignment could have the
same cause as the anomalies considered here. 
Interestingly, \citet{sarkar2011} have demonstrated that the
low-variance and mode alignment is very unlikely to have a common
origin in Gaussian random and statistically isotropic CMB anisotropies.
However, when subtracting
the quadrupole and octupole outside the CL58 mask, the lower tail
probability for the low variance is 0.036, which remains rather low.
The connection with the very low power in the ecliptic northern
hemisphere also remains to be explored.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%TABLE MASK DEPENDENCE
\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Lower tail probablity for the variance, skewness, and kurtosis at $N_{\rm side}=16$, using different masks.}
\label{tab:1pdf-masks}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 1.7in{#\leaderfil}\tabskip=2pt&
\hfil#\tabskip=10pt\hfil&\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan4 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan4\hrulefill\cr
\omit\hfil Mask \hfil& \hfil {\tt C-R} \hfil& \hfil {\tt NILC} \hfil& \hfil{\tt SEVEM} \hfil& \hfil {\tt SMICA}\cr
\noalign{\vskip 3pt\hrule\vskip 4pt}
\multispan5 \hfil Variance \hfil\cr
\noalign{\vskip 1pt}
U73, $f_{\rm sky}=78\%$& 0.019& 0.017& 0.014& 0.019\cr
CL58, $f_{\rm sky}=58\%$& 0.004& 0.003& 0.003& 0.003\cr
CL37, $f_{\rm sky}=37\%$& 0.028& 0.017& 0.018& 0.016\cr
Ecliptic North, $f_{\rm sky}=39\%$& 0.001& 0.001& 0.001& 0.002\cr
Ecliptic South, $f_{\rm sky}=39\%$& 0.464& 0.479& 0.454& 0.490\cr
\noalign{\vskip 3pt}
\multispan5\hfil Skewness\hfil\cr
\noalign{\vskip 1pt}
U73, $f_{\rm sky}=78\%$& 0.016& 0.015& 0.023& 0.012\cr
CL58, $f_{\rm sky}=58\%$& 0.208& 0.139& 0.162& 0.147\cr
CL37, $f_{\rm sky}=37\%$& 0.517& 0.467& 0.503& 0.469\cr
Ecliptic North, $f_{\rm sky}=39\%$& 0.502& 0.526& 0.526& 0.521\cr
Ecliptic South, $f_{\rm sky}=39\%$& 0.004& 0.006& 0.008& 0.004\cr
\noalign{\vskip 3pt}
\multispan5\hfil Kurtosis\hfil\cr
\noalign{\vskip 1pt}
U73, $f_{\rm sky}=78\%$&  0.972& 0.973& 0.966& 0.982\cr
CL58, $f_{\rm sky}=58\%$&  0.630& 0.726& 0.711& 0.711\cr 
CL37, $f_{\rm sky}=37\%$&  0.069& 0.135& 0.130& 0.124\cr
Ecliptic North, $f_{\rm sky}=39\%$&  0.094& 0.229& 0.196& 0.245\cr
Ecliptic South, $f_{\rm sky}=39\%$&  0.933& 0.916& 0.886& 0.948\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                % ends two-column \halign
\endgroup
\end{table} 

%FIGURE MASK DEPENDENCE
\begin{figure}
\centerline{
\includegraphics[width=\hsize]{./section_5.0/section_5.2/section_5.2.1/figs/hist_masks_n0016.pdf}
}
\caption{Variance, skewness and kurtosis at $N_{\rm side}=16$, for the U73
  mask, CL58, CL37, ecliptic North, and ecliptic South (from
  top to bottom). The different lines represent the four component
  separation methods  {\tt C-R} (green), {\tt
    NILC} (blue), {\tt SEVEM} (red), and {\tt SMICA} (orange).} 
\label{fig:1pdf-masks}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Frequency dependence of the lower tail probablity for the variance skewness and kurtosis at $N_{\rm side}=16$, using different masks.}
\label{tab:1pdf-freq}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 1.6in{#\leaderfil}\tabskip=0pt&
\hfil#\hfil\tabskip=2pt&\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan4 \hfil Probability\hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan4\hrulefill\cr
\omit\hfil Mask\hfil& \hfil 70\,GHz\hfil& \hfil 100\,GHz\hfil& \hfil 143\,GHz\hfil& \hfil 217\,GHz\hfil\cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
\multispan5 \hfil Variance\hfil\cr
\noalign{\vskip 1pt}
U73, $f_{\rm sky}=78\%$& 0.019& 0.013& 0.014& 0.016\cr
CL58, $f_{\rm sky}=58\%$& 0.003& 0.003& 0.003& 0.003\cr 
CL37, $f_{\rm sky}=37\%$& 0.024& 0.020& 0.018& 0.020\cr
Ecliptic North, $f_{\rm sky}=39\%$& 0.001& 0.002& 0.001& 0.001\cr
Ecliptic South, $f_{\rm sky}=39\%$& 0.446& 0.436& 0.455& 0.455\cr
\noalign{\vskip 3pt}
\multispan5\hfil Skewness\hfil\cr
\noalign{\vskip 1pt}
U73, $f_{\rm sky}=78\%$& 0.045& 0.016& 0.024& 0.015\cr
CL58, $f_{\rm sky}=58\%$& 0.254& 0.205& 0.162& 0.157\cr 
CL37, $f_{\rm sky}=37\%$& 0.503& 0.471& 0.468& 0.515\cr
Ecliptic North, $f_{\rm sky}=39\%$& 0.505& 0.447& 0.541& 0.352\cr
Ecliptic South, $f_{\rm sky}=39\%$& 0.015& 0.006& 0.009& 0.006\cr
\noalign{\vskip 3pt}
\multispan5\hfil Kurtosis\hfil\cr
\noalign{\vskip 1pt}
U73, $f_{\rm sky}=78\%$&  0.962& 0.981& 0.965& 0.974\cr
CL58, $f_{\rm sky}=58\%$&  0.619& 0.684& 0.710& 0.725\cr
CL37, $f_{\rm sky}=37\%$&  0.114& 0.091& 0.130& 0.121\cr
Ecliptic North, $f_{\rm sky}=39\%$&  0.180& 0.096& 0.203& 0.180\cr
Ecliptic South, $f_{\rm sky}=39\%$&  0.902& 0.920& 0.882& 0.909\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 
%

%FIGURE FREQUENCY DEPENDENCE
\begin{figure}
\centerline{
\includegraphics[width=\hsize]{./section_5.0/section_5.2/section_5.2.1/figs/hist_freq_n0016.pdf}
}
\caption{Variance, skewness and kurtosis at $N_{\rm side}=16$, for the U73
  mask, CL58, CL37, ecliptic North, and ecliptic South (from
  top to bottom). The different lines represent the four considered frequencies, namely 70\,GHz (green), 100\,GHz (blue), 143\,GHz (red), and 217\,GHz (orange). }
\label{fig:1pdf-freq}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






==> section_5.0/section_5.2/section_5.2.2/section_5.2.2.tex <==
\subsection{Hemispherical Asymmetry}
\label{sec:hemispherical_asymmetry}

In \cite{eriksen2004b} and \cite{hansen2004} it was discovered that
the angular power spectrum of the first year \textit{WMAP} data, when
estimated locally at different positions on the sphere, appears not to
be isotropic. In particular, the power spectrum calculated for a
hemisphere centred at 
$(l,b)=(237\deg,-20\deg)$ (in Galactic longitude and latitude) 
was larger than when calculated in
the opposite hemisphere over the multipole range $\ell=2$--40.
Simultaneously, \citet{Park2004} also presented evidence for the
existence of such hemispherical asymmetry --- in which a particular
statistical measure is considered to change discontinuously between
two hemispheres on the sky --- with the application of Minkowski
functionals to the \textit{WMAP} data.  Since the preferred direction
of \cite{eriksen2004b} lies close to the ecliptic plane, it was also
demonstrated that the large-angular scale $N$-point correlation
functions showed a difference in behaviour when computed on ecliptic
hemispheres.  Many studies have subsequently been undertaken focusing
on hemispheres in the ecliptic coordinate system, with
\citet{schwarz2004} particularly emphasizing the
connection. Hemispherical asymmetry has also been seen with other
measures of non-Gaussianity \citep{eriksen2004c,eriksen2005,raeth07a}.

Here, we repeat the analysis of \citet{eriksen2005} on the \Planck\
component separated data, smoothed and then downgraded to $N_{\rm
  side}=64$, as described in Sect.~\ref{sec:data}. However,
in this section the $N$-point correlation
functions are not averaged over the full sky and depend on 
a choice of specific direction, thus, they constitute tools to study
statistical isotropy rather than non-Gaussianity
\citep{Ferreira1997}. 
The latter study was already presented in Sect.~\ref{sec:npoint_correlation},
where it was found that the results for the low resolution
maps are the most deviant relative to the MC simulations based on the
\Planck\ fiducial model. 

The $N$-point correlation functions computed on the northern and
southern hemispheres determined in the ecliptic coordinate frame and 
using the U73 mask are
shown in \fig\ref{fig:npt_asymmetry_n64}. The correlation functions
for the four \Planck\ maps are very consistent, and the observed
behaviour is in agreement with that seen in the \emph{WMAP} data
\citep{eriksen2004b}. Specifically, the northern hemisphere
correlation functions are relatively featureless (both the 3- and 4-point
functions lie very close to zero), whereas the southern hemisphere
functions exhibit a level of structure that is in good agreement with
the confidence regions computed from the Gaussian simulations.

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=\columnwidth]{./section_5.0/section_5.2/section_5.2.2/figs/twopt_temp_dx9delta_common_mask_ecl_n64.pdf}
\includegraphics[width=\columnwidth]{./section_5.0/section_5.2/section_5.2.2/figs/threept_coll_temp_dx9delta_common_mask_ecl_n64.pdf}
\includegraphics[width=\columnwidth]{./section_5.0/section_5.2/section_5.2.2/figs/threept_eq_temp_dx9delta_common_mask_ecl_n64.pdf}
\includegraphics[width=\columnwidth]{./section_5.0/section_5.2/section_5.2.2/figs/fourpt_temp_dx9delta_common_mask_ecl_n64.pdf}
%\includegraphics[width=7.5cm]{./section_5.0/section_5.2/section_5.2.2/figs/twopt_temp_dx9delta_common_mask_ecl_n64.pdf}
%\includegraphics[width=7.5cm]{./section_5.0/section_5.2/section_5.2.2/figs/threept_coll_temp_dx9delta_common_mask_ecl_n64.pdf}
%\includegraphics[width=7.5cm]{./section_5.0/section_5.2/section_5.2.2/figs/threept_eq_temp_dx9delta_common_mask_ecl_n64.pdf}
%\includegraphics[width=7.5cm]{./section_5.0/section_5.2/section_5.2.2/figs/fourpt_temp_dx9delta_common_mask_ecl_n64.pdf}

\caption{The 2-point (upper left), pseudo-collapsed (upper right),
  equilateral 3-point (lower left), and rhombic 4-point (lower right)
  correlation functions (\mbox{$N_{\rm side}=64$}). Correlation functions are shown for the analysis performed on northern (blue) and
  southern (red) hemispheres determined in the Ecliptic coordinate
  frame. The shaded dark and light grey bands
  indicate the 68\% and 95\% confidence regions, respectively. See
    Sect.~\ref{sec:npoint_correlation} for the definition of the separation angle $\theta$.} 
\label{fig:npt_asymmetry_n64}
\end{center}
\end{figure*}


\begin{figure*}[h!]
\begin{center}
\includegraphics[width=\columnwidth]{./section_5.0/section_5.2/section_5.2.2/figs/twopt_temp_dx9delta_common_mask_db_n64.pdf}
\includegraphics[width=\columnwidth]{./section_5.0/section_5.2/section_5.2.2/figs/threept_coll_temp_dx9delta_common_mask_db_n64.pdf}
\includegraphics[width=\columnwidth]{./section_5.0/section_5.2/section_5.2.2/figs/threept_eq_temp_dx9delta_common_mask_db_n64.pdf}
\includegraphics[width=\columnwidth]{./section_5.0/section_5.2/section_5.2.2/figs/fourpt_temp_dx9delta_common_mask_db_n64.pdf}
%\includegraphics[width=7.5cm]{./section_5.0/section_5.2/section_5.2.2/figs/twopt_temp_dx9delta_common_mask_db_n64.pdf}
%\includegraphics[width=7.5cm]{./section_5.0/section_5.2/section_5.2.2/figs/threept_coll_temp_dx9delta_common_mask_db_n64.pdf}
%\includegraphics[width=7.5cm]{./section_5.0/section_5.2/section_5.2.2/figs/threept_eq_temp_dx9delta_common_mask_db_n64.pdf}
%\includegraphics[width=7.5cm]{./section_5.0/section_5.2/section_5.2.2/figs/fourpt_temp_dx9delta_common_mask_db_n64.pdf}

\caption{The 2-point (upper left), pseudo-collapsed (upper right),
  equilateral 3-point (lower left), and rhombic 4-point (lower right)
  correlation functions for the {\tt SMICA} map (\mbox{$N_{\rm side}=64$}). Correlation functions are shown for the analysis
  performed on negative (blue) and positive (red) hemispheres determined in the Ecliptic, Galactic,
  Doppler boost (DB), dipole modulation (DM), and power asymmetry (PA) coordinate
  frames. The shaded dark and light grey bands indicate the 68\% and
  95\% confidence regions, respectively.  See
  Sect.~\ref{sec:npoint_correlation} for the definition
    of the separation angle $\theta$.} 
\label{fig:npt_asymmetry_n64_frames}
\end{center}
\end{figure*}


The probabilities of obtaining a value for the $\chi^2$ statistic for
the \Planck\ fiducial $\Lambda$CDM model at least as large as the
observed values for different CMB component-separated maps are presented in
Table \ref{tab:prob_chisq_asymm}.  The probabilities for the 3-point
and 4-point functions in the northern ecliptic hemisphere are
especially large, and in the case of the pseudo-collapsed
configuration all simulations yielded a larger value of the $\chi^2$
than observed. This suggests that the tendency to super-Gaussianity in
  the maps downgraded to $N_{\rm side}=64$, as noted previously in
  Sect.~\ref{sec:npoint_correlation}, is associated with the northern
  hemisphere. Nominally, this value is even more remarkable than that
found with the \emph{WMAP} data \citep{eriksen2004b}, although to
interpret it correctly one has to keep in mind that the analysis
presented here is an example of an a posteriori
statistic. Specific choices have been made about the smoothing scale
used for downgrading the data, and, in particular, for the reference
direction that defines the hemispheres. This results in a tendency to overestimate
the significance of the results. Nevetheless, the observed properties
of the \Planck\ data are consistent with a remarkable lack of power in
a direction towards the north ecliptic pole, consistent with the
simpler one-point statistics presented in Sect.~\ref{sec:anomalous_variance}.

\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Probabilities of obtaining values of the $\chi^2$ statistic
  for the \Planck\ fiducial model at least as large as the observed
  values of the statistic for the \Planck\ maps with resolution
  parameter \mbox{$N_{\rm side}=64$}, estimated using the {\tt C-R}, {\tt
    NILC}, {\tt SEVEM}
  and {\tt SMICA} methods.} 
\label{tab:prob_chisq_asymm}\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{$>$} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 1.3in{#\leaderfil}\tabskip=0pt&
\hfil#\hfil\tabskip=14pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan4 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan4\hrulefill\cr
\omit \hfil Hemisphere \hfil& {\tt C-R}& {\tt NILC}& {\tt SEVEM}& {\tt SMICA}\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
\multispan5 \hfil Two-point function \hfil\cr
\noalign{\vskip 2pt}
Northern Ecliptic & !0.935 & !0.924&!0.927&!0.932\cr
Southern Ecliptic & !0.633 & !0.599&!0.639&!0.592\cr
\noalign{\vskip 3pt}
\multispan5 \hfil Pseudo-collapsed 3-point function\hfil\cr
\noalign{\vskip 2pt}
 Northern Ecliptic & $>$0.999 & $>$0.999 & $>$0.999 & $>$0.999\cr
 Southern Ecliptic & !0.349 & !0.310 & !0.381 & !0.301\cr
\noalign{\vskip 3pt}
\multispan5 \hfil Equilateral 3-point function \hfil\cr
\noalign{\vskip 2pt}
Northern Ecliptic & !0.996 & !0.999 & !0.999 & !0.999\cr
Southern Ecliptic & !0.627 & !0.644 & !0.678 & !0.656\cr
\noalign{\vskip 3pt}
\multispan5 \hfil  Rhombic 4-point function \hfil\cr
\noalign{\vskip 2pt}
Northern Ecliptic & !0.999 & !0.999 & !0.999 & !0.999\cr
Southern Ecliptic & !0.559 & !0.548 & !0.574 & !0.553\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 

We have also carried out the corresponding calculations in
  Galactic coordinates, as well as 
in reference frames preferred by other 
analyses, such as
the power asymmetry (PA, reference frame for $\ell_{\rm max}=1500$, see Sect.~\ref{sec:power_asymmetry}),
the dipole modulation (DM, see Sect.~\ref{sec:dipolar_modulation}),
and the Doppler boost 
\citep[DB, see][]{planck2013-pipaberration}. 
The corresponding $N$-point
correlation functions are shown in
\fig\ref{fig:npt_asymmetry_n64_frames}. 
Note that the positive hemispheres for the ecliptic and Galactic
reference frames correspond to the southern hemispheres in other tables/figures.
Interestingly, the largest 
asymmetry is seen for the hemispheres determined in ecliptic coordinates. 

In Table \ref{tab:prob_chisq_asymm_frames} we show the
  corresponding probabilities for
the $N$-point functions of the {\tt SMICA} map in these reference
frames. 
Whilst the largest asymmetry is seen
for ecliptic coordinates, 
a substantial asymmetry is present also for Galactic
coordinate hemispheres and, to a lesser extent, for the DM
direction. The asymmetry for the latter can be explained by the fact
that the DM direction is relatively close to the ecliptic pole. For
the PA and DB directions we do not find any significant
asymmetry. 
In the latter case, this is not surprising, since the Doppler boost
effect
is significant only for small angular
scales, while the map used in our analysis was smoothed and downgraded
to much lower resolution.


\begin{table}[h!tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Probabilities of obtaining values of the $\chi^2$ statistic
  for the \Planck\ fiducial model at least as large as the observed
  values for the {\tt SMICA} map at $N_{\rm side}=64$. The probabilities were computed for
hemispheres determined in the ecliptic, Galactic, Doppler boost (DB),
dipole modulation (DM), and power asymmetry (PA) frames.} 
\label{tab:prob_chisq_asymm_frames}\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{$<$} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 1.0in{#\leaderfil}\tabskip=0pt&
\hfil#\hfil\tabskip=14pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan5 \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan5\hrulefill\cr
\omit \hfil Hemisphere \hfil& Ecl.& Gal.& DB& DM& PA\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
\multispan6 \hfil Two-point function\hfil\cr
\noalign{\vskip 2pt}
 Negative& !0.932& !0.974& 0.573& 0.735& 0.747\cr
 Positive& !0.592& !0.275& 0.918& 0.913& 0.882\cr
\noalign{\vskip 3pt}
\multispan6 \hfil Pseudo-collapsed 3-point function\hfil\cr
\noalign{\vskip 2pt}
 Negative& $>$0.999& !0.998& 0.978& 0.912& 0.826\cr
 Positive& !0.301& !0.768& 0.698& 0.300& 0.452\cr
\noalign{\vskip 3pt}
\multispan6 \hfil Equilateral 3-point function\hfil\cr
\noalign{\vskip 2pt}
 Negative& !0.999& !0.994& 0.844& 0.893& 0.492\cr
 Positive& !0.656& !0.379& 0.917& 0.583& 0.425\cr
\noalign{\vskip 3pt}
\multispan6 \hfil  Rhombic 4-point function\hfil\cr
\noalign{\vskip 2pt}
 Negative& !0.999& $>$0.999& 0.771& 0.970& 0.784\cr
 Positive& !0.553& !0.568& 0.993& 0.525& 0.548\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 


Since the largest asymmetry is seen in ecliptic coordinates, we
  might conjecture an association with the peculiar configuration of
  the quadrupole and octopole (although the \textit{Planck} results
  from Sect.~\ref{sec:mode_alignment} do not favour as significant
  an alignment as with the \textit{WMAP} data). In order to study the
  influence of the lowest order multipoles on the hemispherical
  asymmetry,
  we therefore re-analysed the {\tt SMICA} map corrected for multipoles of
  order $\ell \le 3$ and $\ell \le 5$ and present the results in
  Table \ref{tab:prob_chisq_asymm_removed}. It should be apparent
  that, in general, the asymmetry is less significant after removing
  the lowest order multipoles. However, in a few cases, such as for the
  4-point function computed in the ecliptic and DM frames, we do
  not see such behaviour.  Furthermore, in all cases, with the
  exception of the DB frame, we observe a tendency to
  super-Gaussianity for the negative hemisphere. This presumably
  indicates that the hemispherical asymmetry is not only related to
  the
  properties of the very lowest order multipoles, but also extends beyond
  this.

\begin{table*}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Probabilities of obtaining values of the $\chi^2$ statistic
  for the \Planck\ fiducial model at least as large as the observed
  values of the statistic for the \Planck\ {\tt SMICA} map with resolution
  parameter $N_{\rm side}=64$ and removed multipoles of order $\ell
  \le 3$ (columns denoted as ``$\ell >3$'') or order $\ell \le 5$ (columns
  denoted as ``$\ell >5$'') . The probabilities were computed for
hemispheres determined in the ecliptic, Galactic, Doppler boost (DB),
dipole modulation (DM), and power asymmetry (PA) frames.} 
\label{tab:prob_chisq_asymm_removed}\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{$>$} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 1.3in{#\leaderfil}\tabskip=0pt&
\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\tabskip=10pt&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan{10} \hfil Probability \hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan{10}\hrulefill\cr
\omit&\multispan2 \hfil Ecl. \hfil& \multispan2 \hfil Gal. \hfil&
\multispan2 \hfil DB \hfil&\multispan2 \hfil DM\hfil& \multispan2\hfil PA\hfil\cr
\omit \hfil Hemisphere \hfil& $\ell > 3$& $\ell > 5$& $\ell > 3$& $\ell > 5$ & $\ell > 3$ & $\ell > 5$& $\ell > 3$& $\ell > 5$& $\ell > 3$& $\ell > 5$\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
\multispan{11} \hfil Two-point function \hfil\cr
 Negative& 0.886& !0.951& 0.875& 0.957& 0.344& 0.509& 0.746& 0.869& 0.745& 0.819\cr
 Positive& 0.609& !0.906& 0.123& 0.330& 0.824& 0.973& 0.811& 0.979& 0.756& 0.947\cr
\noalign{\vskip 3pt}
\multispan{11} \hfil Pseudo-collapsed 3-point function\hfil\cr
 Negative& 0.985& !0.999& 0.981& 0.978& 0.965& 0.879& 0.966& 0.948& 0.986& 0.872\cr
 Positive& 0.262& !0.643& 0.468& 0.789& 0.807& 0.989& 0.132& 0.390& 0.224& 0.516\cr
\noalign{\vskip 3pt}
\multispan{11} \hfil Equilateral 3-point function \hfil\cr
Negative& 0.984& !0.997& 0.963& 0.952& 0.531& 0.790& 0.945& 0.998& 0.536& 0.943\cr
Positive& 0.776& !0.790& 0.347& 0.727& 0.966& 0.991& 0.358& 0.694& 0.485& 0.649\cr
\noalign{\vskip 3pt}
\multispan{11} \hfil  Rhombic 4-point function \hfil\cr
 Negative& 0.951& $>$0.999& 0.998& 0.992& 0.482& 0.842& 0.991& 0.997& 0.929& 0.989\cr
 Positive& 0.677& !0.584& 0.746& 0.870& 0.994& 0.966& 0.334& 0.368& 0.314& 0.359\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table*} 


==> section_5.0/section_5.2/section_5.2.3/section_5.2.3.tex <==
\subsection{Phase correlations}
\label{sec:scaling_indices}

The statistical properties of a Gaussian
random field on the sphere can be fully described by its two-point
correlation function (or power spectrum) and should exhibit Fourier phases
that are independent and identically distributed (i.i.d.) and follow
a uniform distribution in the interval $\left[ - \pi, \pi \right]$.
Thus, demonstrating the existence of Fourier phase correlations in CMB
maps could indicate the presence of non-Gaussianities in the
primordial density fluctuations.

One could search for phase correlations using different approaches.
However, without there being a specific model for the origin of any
such correlations, one would like to test for scale-dependent
non-Gaussianity and deviations from isotropy in a completely
model-independent (``blind'') way.  One such approach is offered through the
method of ``scaling indices'' and ``surrogates'' (which we explain below).

Previous studies using these methods,
based on the \textit{WMAP} three-, five- and seven-year data
\citep{raeth09a,raeth11a,rossmanith12a,modest13a}, showed significant
evidence for intrinsic phase correlations at low $\ell$ values in the
CMB. The signal was demonstrated to be robust with respect to the
\textit{WMAP} data release, to the component separation methods and to
the selected test statistics.  In this section we apply these methods
to the \Planck\ component separated data sets.

The scaling index method represents one way to estimate the local
scaling properties of a point set in an arbitrary $d$-dimensional
embedding space. The technique provides the possibility of revealing
local structural characteristics of a given point distribution.  
A number of analyses have used scaling indices to test the Gaussian
nature and statistical isotropy of the CMB as represented by the
\textit{WMAP} data \citep{raeth07a,raeth09a,rossmanith09a,raeth11a}.

In general, the method is a mapping that calculates, for each member
$\vec{p}_i, i=1,\dots, N_{\rm pix}$ of a point set $P$, a single value 
that depends on the spatial position of $\vec{p}_i$ relative to the
group of other points in its neighbourhood, in which the point under
consideration is embedded. A three-dimensional point set $P$ 
is generated for two-dimensional spherical CMB-data by
transforming the temperature values $T(\theta_i,\phi_i)$ of each pixel
to a radial jitter around a sphere of radius $R$ at the position of
the pixel centre $(\theta_i,\phi_i)$.  To obtain scaling indices
the local weighted cumulative point distribution is calculated:
%
\begin{equation}
\rho(\vec{p}_i,r) = \sum_{j=1}^{N_{\rm pix}} s_r(d(\vec{p}_i,\vec{p}_j)).
\end{equation}
%
Here $r$ describes the scaling range, while $s_r$ and
$d$ denote a shaping function and a distance measure,
respectively.  The scaling index
$\alpha(\vec{p}_i,r)$ is then defined as the logarithmic derivative of
$\rho(\vec{p}_i,r)$ with respect to $r$:
%
\begin{equation}
\alpha(\vec{p}_i,r) = \frac{\partial \log \rho(\vec{p}_i,r)}{\partial \log r} \;.
\end{equation}
%
Using a quadratic Gaussian shaping function $s_r(x) =
\exp(-(x/r)^2)$ and an isotropic Euclidian norm
$d(\vec{p}_i,\vec{p}_j) = \| \vec{p}_i - \vec{p}_j \|$ as distance
measure, one obtains the following analytic formula for the scaling
indices:
%
\begin{equation}\label{AlphaFormel}
\alpha(\vec{p}_i,r) = \frac{\sum_{j=1}^{N_{\rm pix}}
 2\big(\frac{d_{ij}}{r}\big) e^{-\big(\frac{d_{ij}}{r}\big)^2}}
 {\sum_{j=1}^{N_{\rm pix}} e^{-\big(\frac{d_{ij}}{r}\big)^2}} \;,
\end{equation}
%
where we use the abbreviation $d_{ij} \equiv d(\vec{p}_i,\vec{p}_j)$.  

As seen from the derivation of the expression for $\alpha$, the
  scaling index analysis can be considered as a structural
  decomposition of the point set under study. Points in
  well-localized, cluster-like structures lead to scaling indices of
  $\alpha \approx 0$ , filamentary structures have $\alpha \approx 1$
  , and sheet-like structures $\alpha \approx 2$ .  A uniform,
  three-dimensional distribution of points would result in $\alpha
  \approx 3$.  One can schematically think of the scaling indices
  applied to CMB data as estimating
  the roughness of the last scattering surface
  on different scales.

As should be clear from equation (\ref{AlphaFormel}), the calculation of
scaling indices depends on the scale parameter $r$.  Ten scaling range
parameters $r_k= 0.05, 0.1,\dots, 0.5$, $k=1,2,\dots, 10$, in the notation
of \citet{raeth07a}, are used in this analysis. In order to calculate
scaling indices on large scales, as in previous studies, we couple the
$r$-jitter $a$ to $r_k$ via $a= 0.5 r_k$.  The mean $\langle
\alpha(r_k) \rangle$ and standard deviation $\sigma_{\alpha (r_k)}$,
derived from the full sky and from a set of 768 rotated
hemispheres, are used to test for non-Gaussianity and deviations from
statistical isotropy. 

In order to quantify the significance of the scaling index results,
and focus the study on the phase properties of the observed CMB sky,
we utilize the method of ``surrogate maps'' \citep{raeth09a}.
This surrogate approach suppresses the sensitivity of the null tests to the
assumed fiducial power spectrum, which
is particularly pertinent, given the potential mismatch of the
\Planck\ data to the fiducial spectrum on large angular scales
\citep{planck2013-p08}.

The basic idea of the method of surrogates is to generate for a given data
  set an ensemble of so-called surrogate data, which mimic some
  properties of the original data being defined by a null hypothesis,
  while all other properties are subject to randomization. Analysing
  both the original and surrogate data sets with test statistics, which
  are sensitive to the complement of the null hypothesis, then reveals
  whether the original data were consistent with the null hypothesis
  or not.  In our case, the null hypothesis is that the CMB map is
  Gaussian and thus fully described by the power spectrum and free of
  any phase correlations. The test statistics being employed are those
  that are sensitive to higher-order correlations (i.e., correlations
  beyond the two-point correlation function) in real
  space. Alternatively, one can think of introducing Fourier phase
  statistics, but those methodologies are currently less developed.

%zero order
However, the Gaussianity of the temperature distribution and the
randomness of the set of Fourier phases of the map to be studied are a
necessary prerequisite for the application of the
surrogate-generating algorithm. Therefore the following pre-processing
steps are applied to generate a zero order surrogate map. First, the
maps are remapped onto a Gaussian distribution in a rank-ordered
way. Then we ensure the randomness of the set of Fourier phases by
making a rank-ordered remapping of the phases onto a set of uniformly
distributed ones.  These two preprocessing steps only have marginal
influence on the maps.  Now the set of surrogates to be used for
assessing the statistical properties of the data sets can be generated
by shuffling the phases in the space of the spherical harmonics, while
exactly preserving the modulus of the $a_{\ell m}$.  Moreover, by
introducing a two-step shuffling scheme for previously specified
$\ell$-ranges, a scale-dependent analysis is made possible.  It is
worth noting that while in all surrogate maps the modulus of each
$a_{\ell m}$ is exactly preserved, null tests involving a comparison
to an assumed fiducial power spectrum only preserve the $C_{\ell}$
values, which are average values of the $\left| a_{\ell m}\right|$
when summed over $m$. Thus, the linear properties of the surrogate
maps are more tightly constrained, and specifically kept constant,
than they would be in tests involving simulated maps generated on the
basis of the $C_{\ell}$s.

So-called first- and second-order surrogate maps are then obtained as
follows. We initially generate a first-order surrogate map, in which
any phase correlations for the scales that are not of interest are
randomized by shuffling the phases
$\phi_{\ell m}$ for $\ell \notin \Delta l = [\ell_{\rm min}, \ell_{\rm max}],
 0 < m \le \ell$.
In a second step, $N$ (=1000)
realizations of second-order surrogate maps are generated from the
first-order surrogate map, in which the remaining phases $\phi_{\ell m}$
with $\ell \in \Delta \ell$, $0 < m \le \ell$ are shuffled, while
the previously randomized phases for the other scales are preserved.
The generation of surrogates is always performed using the maps with
the highest resolution, i.e., $N_{\rm side}=2048$.
Given the evidence for anomalies on the largest angular scales, and to
ensure consistency with the previous \textit{WMAP} analyses, we
perform dedicated scale-dependent tests for the scales defined by
$\Delta \ell = [2,20]$.

The exclusion of the phases belonging to the zonal modes ($m=0$)
  from the shuffling raises the question as to whether the results
  depend on the choice of coordinate system, since these modes are only defined
  with respect to the selected coordinate system. This issue is
  particularly important in the specific case of the CMB when
  analysing data in the Galactic coordinate system, because possible
  residuals in and around the Galactic plane are likely to be
  reflected mostly in these modes. To test the dependence of the
  results on the coordinate system, we repeated the surrogate analysis
  with $N=100$ second-order surrogates for each member of a set of
  $48$ rotated CMB maps, where the rotations, defined by 
  a {\tt HEALPix}  $N_{\rm side}=2$ map, such that the pixel centres
  indicate the orientation of the $z$-axis of the rotated frame, 
  uniformly cover the unit sphere.

Since the methodology in its simplest form requires orthonormality
of the set of basis functions $Y_{\ell m}$, we apply the method to the
full sky foreground-cleaned maps as obtained after component
separation with {\tt Commander-Ruler}, {\tt NILC}, {\tt SEVEM} and
{\tt SMICA}.  For the selected $\ell$-interval $\Delta \ell = [2,20]$,
the generation of the first-order surrogate map removes the phase
signature of the small scale residuals in the data and this can be
interpreted as a form of inpainting procedure for small masked patches
in the Galactic plane. % ({\tt SMICA}).
The differences between the first- and second-order surrogates 
are quantified by the $\sigma$-normalized deviation
%
\begin{equation}
S(Y) = \frac{Y_{{\rm surr1}}- \langle Y_{{\rm surr2}} \rangle}
 {\sigma_{Y_{{\rm surr2}}}}
\end{equation}
%
with $Y= \langle \alpha(r_k) \rangle, \sigma_{\alpha(r_k)}, \chi^2$. 
Here, $\chi^2$ represents either a diagonal combination of the mean
$\langle \alpha(r_k) \rangle$ and standard deviation
$\sigma_{\alpha(r_k)}$ at a certain scale $r_k$, or for the full
scale-independent $\chi^2$ statistics:
%
\begin{equation}
\chi^2  = ( \vec{M} - \langle \vec{M} \rangle)^{\rm T}
   \tens{C}^{-1}  (\vec{M} - \langle \vec{M} \rangle),
\end{equation}
%
where the test statistics to be combined are contained in the vector
$\vec{M}$ and $\tens{C}$ is obtained by cross-correlating the elements of
$\vec{M}$.  With the mean and the standard deviation as input for
$\vec{M}$ we obtain $\chi^2_{\langle \alpha \rangle}$ and
$\chi^2_{\sigma_{\alpha}}$ statistics with $\vec{M}^{\rm T}=( \langle \alpha
(r_1) \rangle, \dots, \langle \alpha (r_{10}) \rangle)$ and
$\vec{M}^{\rm T}=( \sigma_{\alpha (r_1)}, \dots, \sigma_{\alpha (r_{10})})$,
respectively.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=8.5cm]{./section_5.0/section_5.2/section_5.2.3/figs/smap_mean_smica.pdf}
\includegraphics[width=8.5cm]{./section_5.0/section_5.2/section_5.2.3/figs/smap_mean_smica_rot.pdf}
\caption{\label{fig:s-maps0} Deviations $S(\langle \alpha \rangle)$ of the
rotated hemispheres derived from
the mean of the scaling indices for the scale $r_{5}$ determined from the
{\tt SMICA} map. {\it Upper panel}: Result for the
calculations with respect to the Galactic coordinate system.
{\it Lower panel}: Result obtained after averaging over $48$ 
rotated coordinate systems. }
\end{center}
\end{figure}

 Figure~\ref{fig:s-maps0} shows the deviation $S(\langle
  \alpha(r_{5} \rangle)$ values for the set of rotated hemispheres for
  the {\tt SMICA} map. Each pixel of the full sky map with a {\tt
    HEALPix} resolution of $N_{\rm side}=8$ specifies one of the 768
  $S$-values for a rotated hemisphere, where the pixel position
  indicates the orientation of the $z$-axis of the rotated coordinate
  system. We find a large number of hemispheres for which
  $\left|S\right|$ is larger than $3$, indicating a significant
  difference between the first- and second-order surrogate
  maps. Therefore, one has to conclude that the low-$\ell$ phases are
  correlated.
  In addition, one can clearly see that the
  deviation $S$ goes in opposite directions for a number of pairs of
  opposite hemispheres. This indicates the presence of pronounced
  anisotropy in the CMB.  We further find that the $S$-map derived for
  the Galactic coordinate system and the $S$-map from the average of
  rotated coordinate systems are nearly indistinguishable. This shows
  that the zonal modes are not special and that the choice of Galactic
  coordinates as reference frame does not induce any bias. Therefore,
  all of the results that follow are only shown for Galactic coordinates.  We
  also find very similar yet less significant patterns of asymmetry
  when considering the standard deviation of the scaling indices
  $\sigma_{\alpha}$, which leads to a significant detection of
  anomalies when combining both quantities into a $\chi^2$-statistic
  (see Fig.~\ref{fig:s-maps1}).
The results are consistent for
{\tt Commander-Ruler}, {\tt NILC}, {\tt SEVEM} and {\tt SMICA}.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=8.5cm]{./section_5.0/section_5.2/section_5.2.3/figs/smap_smica.pdf}
\caption{\label{fig:s-maps1} Deviations $S(\chi^2)$ of the rotated hemispheres
derived from a combination of the mean and the standard deviation of the
scaling indices for the scale $r_{5}$ 
determined from the {\tt SMICA} map.}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\hspace*{-0.9cm}\vspace*{-0.4cm}\includegraphics[width=10.1cm]{./section_5.0/section_5.2/section_5.2.3/figs/dx9_smica_r_ext_2_20.pdf}

\caption{\label{fig:s-plots1} 
  Deviations $|S(r)|$ for the {\tt SMICA} map as a function of the
  scale parameter $r$ for the full sky (black) and positive (red) and 
  negative (blue) rotated hemisphere. The reference frame for defining 
  the positive  and negative hemisphere is chosen such that
  the difference $\Delta S = S_{pos} - S_{neg}$ becomes maximal 
  for $\langle \alpha (r_{5}) \rangle$. The plus signs denote 
  the results for the mean $\langle \alpha (r_{k}) \rangle$, the 
  star-signs represent the standard deviation  $\sigma_{\alpha (r_{k})} $. 
  The dashed (dotted) line indicates the $1$ ($3$) $\sigma$ significance
  level.
}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\begin{center}
\hspace*{-0.9cm}\vspace*{-0.4cm}\includegraphics[width=10.1cm]{./section_5.0/section_5.2/section_5.2.3/figs/prob_dens_mean_0_20.pdf}

\caption{\label{fig:prob_dens1} Probability density $P(\langle \alpha
  (r_{5}) \rangle)$ for the second-order surrogates using the {\tt
    SMICA} map for the positive (red) and negative (blue) rotated
  hemispheres. The vertical lines show the respective values for
  $\langle \alpha (r_{5}) \rangle$ for the first-order surrogates.  }
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{
  Deviations $S$ and empirical probabilities $p$  for the scale-independent
  $\chi^2$-statistics
  derived from the {\tt C-R}, {\tt NILC}, {\tt SEVEM}, and {\tt SMICA} maps.} 
\label{sim_table1}\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{$>$} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 1.0in{#\leaderfil}\tabskip=0pt&
%\hbox to 0.8in{\hfil#\hfil}&\hbox to 0.7in{\hfil#\hfil}&\hbox to 0.7in{\hfil#\hfil}\/\tabskip=0pt\cr
\hfil#\hfil\tabskip=8pt&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\multispan3 \hfil $S$\,/\,$p$ [\%]\hfil\cr
\noalign{\vskip -4pt}
\omit&\multispan3\hrulefill\cr
\omit& \omit&\hfil  Positive\hfil&\hfil Negative\hfil\cr 
\omit\hfil Model\hfil& \hfil Full Sky\hfil& \hfil Hemisphere\hfil& \hfil Hemisphere\hfil\cr 
\noalign{\vskip 3pt\hrule\vskip 3pt}
{\tt C-R}, $\chi^2_{\langle \alpha \rangle}$&  0.86 / 82.6& 4.21 / 99.7& 3.18 / !99.0\cr
{\tt C-R}, $\chi^2_{\sigma_{\alpha}}$& 0.88 / 85.2& 3.94 / 99.5& 3.10 /!99.2\cr 
{\tt NILC}, $\chi^2_{\langle \alpha \rangle}$& 0.86 / 81.8& 3.74 / 99.6& 4.41 / $>$99.9\cr
{\tt NILC}, $\chi^2_{\sigma_{\alpha}}$& 0.79 / 78.8& 3.69 / 99.6& 4.49 / $>$99.9\cr
{\tt SEVEM}, $\chi^2_{\langle \alpha \rangle}$& 0.00 / 58.0& 3.22 / 99.3& 5.02 / $>$99.9\cr
{\tt SEVEM}, $\chi^2_{\sigma_{\alpha}}$ & 0.05 / 60.8& 3.20 / 99.0& 5.11 / !99.9\cr
{\tt SMICA}, $\chi^2_{\langle \alpha \rangle}$ & 0.75 / 80.1& 3.80 / 99.8& 4.70 / !99.8\cr
{\tt SMICA,} $\chi^2_{\sigma_{\alpha}}$ & 0.01 / 54.4& 3.64 / 99.3& 4.81 / $>$99.9\cr
\noalign{\vskip 2pt\hrule\vskip 3pt}}}
\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 



In Fig.~\ref{fig:s-plots1}, the deviations $S(Y)$ are displayed for
the mean and standard deviation. We only show the results for the {\tt
  SMICA} map.  The other three maps yield very similar results. For
all four maps the values for $S(\langle \alpha \rangle)$ extend
beyond 3 for $r = 0.2$--0.25 when rotated hemispheres are
considered separately. Since the effect in the separate hemispheres
goes in opposing directions, no signal is observed for the full sky.
The results for the scale-independent $\chi^2$ statistics are
summarized in Table~\ref{sim_table1}.  The results suggest a
significant detection of both non-Gaussianity and anisotropy in
the \Planck\ data, consistent with those obtained previously with
\textit{WMAP} data \citep[for comparison see][]{modest13a}.

Figure \ref{fig:prob_dens1} presents results that allow us to
  attempt to elucidate the origin of the detected asymmetry and its
  relationship to other anomalies.  Considering the first-order
  surrogate maps, in which the low-$\ell$ phases are unchanged by the
  shuffling procedure, there is a clear shift between the mean of the
  scaling indices for the positive (red) and negative (blue)
  hemispheres.  If we now examine the probability density of the mean
  of the scaling indices for the positive and negative rotated
  hemispheres, as determined from the set of second-order surrogates,
  again a systematic shift is observed. Since the phases are
  uncorrelated in the second-order surrogate maps, the effect can only
  be attributed to properties of the distribution of $\left| a_{lm}
  \right|$, i.e., to power asymmetries. However, it should be apparent
  that the shift in mean values is in the opposite sense to the first-order
  surrogates, implying that an additional pattern of asymmetry
  is induced solely by correlations in the phases.

Finally, it should be noted that certain choices made in the analysis,
  e.g., the selection of specific values for $r_k$ and $a$
parameters,  together with the decision to make an analysis on
hemispheres using the method of surrogates,
constitute a posteriori selections and can lead to an overestimate of the
significance of the results. Nevertheless, the claimed asymmetry is
certainly consistent with results presented in the following sections.
The analysis involving surrogate maps reveals that there {\it are} phase
correlations at low $\ell$.


==> section_5.0/section_5.2/section_5.2.tex <==
\subsection{Hemispherical asymmetry}
\label{sec:hemispherical_asymmetry}

In \cite{eriksen2004b} and \cite{hansen2004} it was discovered that
the angular power spectrum of the first year \textit{WMAP} data, when
estimated locally at different positions on the sphere, appears not to
be isotropic. In particular, the power spectrum calculated for a
hemisphere centered at $(\theta,\phi)=(110\deg,237\deg)$ (in
Galactic co-latitude and longitude) was larger than when calculated in
the opposite hemisphere over the multipole range $\ell=2$--40. A
similarly strong asymmetry was found only in $0.9\%$ of simulated maps
of the CMB sky. Simultaneously, \citet{Park2004} also demonstrated the
existence of such hemispherical asymmetry --- in which a particular
statistical measure is considered to change discontinuously between
two hemispheres on the sky --- with the application of Minkowski
functionals to the \textit{WMAP} data. Since the preferred direction
from \cite{eriksen2004b} lies close to the ecliptic plane, many
studies have also been undertaken focusing on hemispheres in that
coordinate system, with \citet{schwarz2004} particularly emphasizing
the connection. Subsequently, such asymmetry
has also been seen with other measures of non-Gaussianity
\citep{eriksen2004c,eriksen2005,raeth07a}. 
Here, we consider a subset of statistical measures 
as applied to the \Planck\ data.

%could be 1pdfs or MFs
\input{./section_5.0/section_5.2/section_5.2.1/section_5.2.1}

%n-point correlations on large angular scales
\input{./section_5.0/section_5.2/section_5.2.2/section_5.2.2}

%scalling indices
\input{./section_5.0/section_5.2/section_5.2.3/section_5.2.3}



==> section_5.0/section_5.3/section_5.3.1/section_5.3.1.tex <==
\subsection{Power asymmetry}
%\subsubsection{Power asymmetry}
\label{sec:power_asymmetry}

In their analysis of the 5-year \textit{WMAP} data, \citet{hansen2009}
specifically searched for dipolar power asymmetry on the sky.  In
particular, a simple test was performed in which the power spectrum on
discs was computed and binned into independent blocks of 100
multipoles from $\ell=2$ to $\ell=600$, then each block fitted for a
dipolar asymmetry in the power distribution. The six $\ell$ ranges
considered showed evidence of a consistent dipole direction. The
significance of this was shown by the fact that not a single
realization in a set of 10,000 simulations showed a similarly strong
asymmetry. A further extension of the analysis introduced a model
selection procedure taking into account the statistical penalty for
introducing an asymmetric model with additional parameters (direction
of asymmetry, amplitude of asymmetry and asymmetric multipole
ranges). Even in this case, the asymmetry was found to be highly
significant for the whole range $\ell=2$ to $600$.

Unfortunately, this procedure is highly CPU-intensive. Given the
increased sensitivity and angular resolution of the \Planck\ data, we
have therefore chosen to focus on the simpler test, following the
modified approach of \citet{axelsson2013} as applied to the 9-year
\textit{WMAP} data.  Specifically, we estimate
the power spectrum amplitude on 12 non-overlapping patches of the sky
in $\ell$-bins of 16 multipoles each, and fit a dipole to the spatial
distribution of the amplitude for each $\ell$-bin. This allows us to
probe further into a previously unexplored high-$\ell$ range and to
answer at least in part any a posteriori criticisms of the
study. Since the analysis is power-spectrum based, the half-ring data
sets for the different CMB estimators are used.\footnote{In fact, the
  simulated half-ring noise maps were generated by adjusting the
  properties of the existing 1000 noise simulations appropriately,
  thus explaining why only 500 simulations are used in this analysis.}
  The approach is as follows.

\begin{enumerate} 

\item We apodize the U73 Galactic, and point source mask by smoothing
 it twice with a 30\arcmin\ Gaussian beam followed by a 10\arcmin\ smoothing
 that is repeated three times. The apodized mask is multiplied with the
  original mask between each of the smoothing operations, thus all
  pixels which are zero in the U73 mask remain so in order to continue
  to fully eliminate foreground residuals.  In addition, a smooth
  transition between masked and unmasked regions is created.  The
  power spectrum estimation method has been shown to take into account
  the mode couplings introduced by sharp edges in the
  mask. Nevertheless, we have adopted an apodized mask, since the error
  bars at high $\ell$ decrease slightly due to the reduced
  couplings. The effective sky fraction of the U73 mask falls from
  73\% to 69\% due to this procedure.
\item The {\tt MASTER} technique \citep{hivon2002} is used to estimate
  local cross power spectra between the two half-ring maps on 12
  non-overlapping patches on the sky. A given patch corresponds to one
  of the twelve base pixels of an $N_\mathrm{side}=1$ {\tt HEALPix}
  map, masked as appropriate by the apodized U73 Galactic and point
  source mask. This results in usable sky coverages of approximately
  7\% for each of the eight patches surrounding the poles, and of order 3\%
  for each of the four patches aligned with the Galactic plane.  This approach
  differs from that of the earlier
  analysis of \citet{hansen2009} in which 3072 highly overlapping
  discs were used, but correlations were ignored.  The revised method
  results in weaker correlations between the non-overlapping patches.
\item Following \citet{hansen2009} the 12 local spectra are estimated in bins of 16 multipoles.
  The highest multipole included in the
  analysis is $\ell_{\tt max}=1500$, since both noise and high-$\ell$
  foregrounds become important at higher multipoles
  \citep{planck2013-p06,planck2013-p08,planck2013-p11}.  For some
  comparisons, it is useful to follow \citet{hansen2009} and further
  combine these 16-multipole bins into blocks containing approximately
  100 multipoles. Although no single block contains exactly 100
  multipoles, they will be referred to as such.  However, our main
  results are based on the 16-multipole blocks, which offer improved
  statistics over the more coarsely binned data for our statistic of
  choice.
\item Each 16-multipole block now has an associated local power map at
  $N_\mathrm{side}=1$. The {\tt HEALPix} routine {\tt remove\_dipole}
  is then used with inverse variance weighting  (with the
  weight for each region determined from the variance of the local
  power spectra derived from simulations) 
  to obtain the dipole direction of the power distribution for each map.
\item The alignment of the dipole directions between the different
  multipole blocks is then used to construct a measure of the power spectrum
  asymmetry. Despite the mask-induced correlations between adjacent
  multipoles, the power spectra estimated in 16-multipole blocks
  should be highly independent and the dipole directions determined
  for a Gaussian, isotropic CMB realization should be random, as
  confirmed by simulation.
\item The same procedure is then applied to a set of 500 simulated
  maps of the CMB and noise to derive significance.
\end{enumerate}

\begin{figure*}[htmp!]
\begin{center}
%\includegraphics[angle=0,width=\columnwidth]{./section_5.0/section_5.3/section_5.3.1/figs/ap3_smica_original_asymm_dir_mean_bwhite_120.pdf}
\includegraphics[angle=0,width=2\columnwidth]{./section_5.0/section_5.3/section_5.3.1/figs/ap3_smica_original_asymm_dir_mean_bwhite_120.pdf}
\caption{Dipole directions for 100-multipole bins of the local power
  spectrum distribution from $\ell=2$ to $1500$ in the {\tt SMICA} map with
  the apodized U73 mask applied.  We also show the total direction for
  $\ell_{\tt max}=600$ determined from \textit{WMAP}-9, as well as the
  preferred dipolar modulation axis (labelled as low-$\ell$) derived in
  Sect.~\ref{sec:dipolar_modulation}. \label{fig:dipoles}}
\end{center}
\end{figure*}

In order to assess the significance of the asymmetry, it is necessary to
compare the clustering of the dipole directions evaluated for the
different scales to that observed in simulated maps. For this purpose,
we compute the mean separation angle, $\theta_{\rm mean}$, between all
possible pair-wise combinations of the 16-multipole dipole directions
up to a given $\ell_{\rm max}$. The expectation value for this
statistic is 90\deg\ when determined from the dipole directions
computed on the full sky for an isotropic, Gaussian realization of the
CMB.  We have shown that this remains true for an analysis when
applying the apodized U73 mask.  We determine $\theta_{\rm mean}$ for
the data as well as for all 500 simulated maps.  The fraction of
simulations with a higher value for $\theta_{\rm mean}$ than the data
defines a $p$-value for the measurement.  One advantage of this
directional analysis is that it focuses on a central issue for tests
of deviation from isotropy -- whether there is a preferred
direction. Moreover, as noted by \citet{Bunn2000}, the CMB may exhibit
a pattern that cannot be identified from the power spectrum, but
which would indicate some non-trivial large-scale structure. In the
context of our analysis this means that the amplitudes of the power
dipoles may not be discernible, in a frequentist sense, from the
distribution of values expected for an ensemble of Gaussian, isotropic
CMB realizations. However, evidence for the close correlation and
alignment of directions on different angular scales presents a clear
signature of power asymmetry, since in the standard model, these
directions should all be independent random variables.  Our claims
about power asymmetry in this section are based \emph{solely} on this
statistic.


In Fig.~\ref{fig:dipoles} we show the dipole directions of the 15
lowest 100-multipole bins for the {\tt SMICA} map.
The preferred direction for \textit{WMAP}-9 over the range $\ell=2$ to
$600$ is also indicated,
as is the preferred low-$\ell$ modulation direction determined in
Sect.~\ref{sec:dipolar_modulation}.  Similar behaviour is seen for all
of the \Planck\ foreground-cleaned maps.

In Table~\ref{tab:dipole_summary} we present a summary of the power
asymmetry results from the \Planck\ data processed by all four Planck
foreground cleaning methods --- {\tt Commander-Ruler}, {\tt NILC},
{\tt SEVEM}, and {\tt SMICA} --- computed on the apodized U73 mask.
For comparison, we also include the latest \textit{WMAP} 9-year 
result\footnote
{ Note that the \textit{WMAP} direction and $p$-value is slightly different 
  from the numbers found in \cite{axelsson2013}, due to small
  differences in the analysis. Here, we use 16-multipole bins and the 
  direction is determined from the mean dipole
  direction of all bins in the specified multipole range rather than from one
  single bin spanning  the full multipole range.
}
computed with their KQ85 mask (which has a usable sky fraction of
74.8\%). 
It should be apparent that the
clustering seen visually in Fig.~\ref{fig:dipoles} is both significant 
and consistent for
all foreground subtraction methods. 

\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
  \caption{
  Summary of the best-fit power dipole directions on the sky
  up to $\ell_{\rm max} = 600/1500$, for each of the
  four component separation methods, together with the 143\,GHz map
  cleaned using the {\tt SEVEM} method and denoted {\tt SEVEM-143}.
  These are determined from maps of the power spectrum estimated on 12
  non-overlapping patches in bins of 16 multipoles.
  The preferred direction 
  is the mean of the separate 16-multipole dipole directions in the
  range $\ell=2$ to $\ell_\mathrm{max}$.
  The angle $\theta_{\rm mean}$ is the mean separation angle between all
  possible pair-wise combinations of these 16-multipole dipoles over
  the same $\ell$ range.
  The $p$-value for the power asymmetry is
  given by the fraction of simulations with a larger mean separation
  angle, $\theta_{\rm mean}^{\rm sim}$, than the observed data, $\theta_{\rm mean}^{\rm data}$. 
  {\tt SEVEM-143DB} corresponds to data corrected for Doppler
  boosting, while all other results are derived without this correction.
  In fact, due to the frequency dependence of this effect,
  deboosting is not important for the \textit{WMAP} data.
  For the \textit{Planck} analysis, 500 FFP6 simulations were analysed, while
  10\,000 Gaussian simulations were used to study the \textit{WMAP} data.
\label{tab:dipole_summary}}
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{$-$} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 0.95in{#\leaderfil}\tabskip=0pt&
\hfil#\hfil\tabskip=7pt&\hfil#\hfil&\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
 \omit&\omit& \omit& \omit&  Frac.& \omit\cr
\omit\hfil Method\hfil&  Mask& $(l,b)$\,[\deg]& $\theta_{\rm
  mean}^{\rm data}$ [\deg]&  $\theta_{\rm mean}^{\rm sim} > \theta_{\rm
  mean}^{\rm data}$& $\ell_\mathrm{max}$\cr
%\noalign{\vskip 3pt\hrule\vskip 5pt}
%\multispan4 \hfil\textbf{$\ell_{\rm max} = 1500$ } \hfil\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
 {\tt C-R} & U73 &(231,*$-$2) & $86.7$ & 493/500&1500\cr
 {\tt NILC} & U73 &(214,**4) & $85.7$ & 500/500&1500\cr
 {\tt SEVEM} & U73 & (215,**9) & $85.8$ & 500/500&1500\cr
 {\tt SMICA} & U73 & (220,**4) &  $86.2$ & 499/500&1500\cr
 {\tt SEVEM-143} & U73 & (228,*$-$1) & 86.7 & 496/500&1500\cr
 {\tt SEVEM-143DB} & U73 & (218,$-$21) & $87.6$ & 487/500&1500\cr
 \textit{WMAP}-9 & KQ85 &(209,$-$24) & $82.3$ & 9966/10000&600\cr
 {\tt C-R} & U73 &(192,*$-$5) & $81.7$ & 500/500&600\cr
 {\tt NILC} & U73 &(194,*$-$3) & $80.8$ & 500/500&600\cr
 {\tt SEVEM} & U73 & (195,*$-$2) & $81.2$ & 500/500&600\cr
 {\tt SMICA} & U73 & (196,*$-$2) &  $81.9$ & 500/500&600\cr
 {\tt SEVEM-143} & U73 & (195,**3) & 81.6 & 500/500&600\cr
 {\tt SEVEM-143DB} & U73 & (189,$-$10) & $81.9$ & 500/500&600\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table}
 
However,  Doppler boosting, due to
our motion with respect to the CMB rest frame, is expected to induce
both a dipolar modulation of the temperature anisotropies, 
and an aberration that corresponds to a change in the apparent arrival directions of
the CMB photons \citep{challinor2002}. Both of these effects
are aligned with the CMB dipole.
In a companion paper \citep{planck2013-pipaberration}, a statistically
significant detection of 
such an effect at small angular scales is reported. 
From an inspection of
Fig.~\ref{fig:dipoles} it should be apparent that whilst the asymmetry
direction on large and intermediate angular scales are in general
tightly clustered around the same direction as found for
\textit{WMAP}, 
weak indications of this second preferred power asymmetry direction
might be seen. However, we have determined that our
statistic of choice is unable to cleanly separate a Doppler dipolar
modulation from a power asymmetry imprinted on the data. 

In order to investigate the power asymmetry further, it is necessary
to analyse data that have been corrected for the Doppler modulation
effect. 
%We do not attempt to de-aberrate the CMB sky maps, since the
%effect is not significant on the scales that are found to be of
%interest here.
As shown in \citet{planck2013-pipaberration}, the modulation
amplitude is frequency dependent. It is therefore difficult to correct
for the effect in the component separated maps used in this paper, since they are
constructed from frequency maps to which both scale-dependent and
spatially varying weighting schemes are applied. The {\tt SEVEM}
approach, however, adopts a single weight per frequency. In what
follows, we utilize a version of the 143\,GHz data cleaned using this
method (which we will refer to as {\tt SEVEM-143}), with the weights
summarized in Table~C.1. of \citet{planck2013-p06}. The Doppler
modulation can then be removed using the prescription and weights
derived in \citet{planck2013-pipaberration}. 
We will refer to this process as deboosting, even though a correction
for aberration is not performed.
Such a de-aberration is not needed since the FFP6
simulations used in this analysis contain the aberration effect, but
not the Doppler modulation of the CMB anisotropies. However, in order to match the noise
properties of the demodulated data, the noise component of each
simulation is separately demodulated.


\begin{figure*}[htpm!]
\begin{center}
%\includegraphics[angle=0,width=\columnwidth]{./section_5.0/section_5.3/section_5.3.1/figs/ap3_sevem143_deboost_asymm_dir_mean_bwhite_120.pdf}
\includegraphics[angle=0,width=2\columnwidth]{./section_5.0/section_5.3/section_5.3.1/figs/ap3_sevem143_deboost_asymm_dir_mean_bwhite_120.pdf}
\caption{Dipole directions for 100-multipole bins of the local power
  spectrum distribution from $\ell=2$ to $1500$ in the deboosted {\tt SEVEM} 
  143\,GHz map ({\tt SEVEM-143DB}) with
  the apodized U73 mask applied.  We also show the direction for
  $\ell_{\tt max}=600$ determined from \textit{WMAP}-9, as well as the
  preferred dipolar modulation axis (labelled as low-$\ell$) derived in
  Sect.~\ref{sec:dipolar_modulation}. \label{fig:sevem143}}
\end{center}
\end{figure*}

\begin{figure}[htbp!]
\begin{center}
\includegraphics[width=\hsize]{./section_5.0/section_5.3/section_5.3.1/figs/sig_flmax_ap3_nband1_deboost_frode_vs_originalclustering.pdf}

\caption{Derived $p$-values as a function of $\ell_\mathrm{max}$,  
          for the {\tt SEVEM} 143\,GHz foreground-cleaned map,
          determined both before and after deboosting. The $p$-values are computed
          using 500 FFP6 simulated maps. 
          \label{fig:significance}}
\end{center}
\end{figure}



 In Fig.~\ref{fig:sevem143} we show the dipole directions of the
  100-multipole bins after the deboosting correction. As compared to
  Fig.~\ref{fig:dipoles}, the dipole directions have now moved away
  from the Doppler dipole direction and cluster more around the
  \textit{WMAP}-9 and low multipole asymmetry directions. The mean
  dipole direction for $\ell=2$ to $1500$ is now
  $(l,b)=(218\deg,-21\deg)$, displaced by about 25\deg\
  compared to the non-deboosted directions in
  Table~\ref{tab:dipole_summary}. Note that the mean asymmetry
  directions for the $\ell=2$ to $600$ range for the deboosted {\tt
    SEVEM-143} and \textit{WMAP}-9 data differ by about 20\deg,
  most likely due to the differences in the masks used and noise
  properties.

Fig.~\ref{fig:significance} presents the $p$-values (the fraction of simulations 
with a larger mean separation angle than that determined from the 
real sky) as a function of
$\ell_\mathrm{max}$.
It is certainly the case that power asymmetry is observed to 
$\ell_\mathrm{max}\sim 600$, even for deboosted data.
Cursory inspection may lead to the conclusion
that asymmetry at a significance level of 98--99\% persists to
at least $\ell_\mathrm{max}=1300$. 
However, this is a consequence of the cumulative nature of the
statistic. Investigation of $\theta_{\rm
  mean}$ for individual multipole ranges (see below) does not indicate the
presence of asymmetry above $\ell_\mathrm{max}\sim600$. Similar conclusions 
were reached by \citet{flender2013} and \citet{notari2013}, although they only looked at 
the power ratio which is not directly related to the test performed here.

\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
 \caption{ Significance of the asymmetry using several global significance 
measures. The numbers in the table reflect the number of simulations 
that have clustering $p$-values of $100\%$ and $>99\%$ for less
$\ell_\mathrm{max}$ values than the data, as well as the number of 
simulations with lower mean $p$-values (as determined over all
$\ell_\mathrm{max}$) than the data. 
These values are calculated for the $\ell_\mathrm{max}$ range 2--600 and
2--1500. 
The  last two columns show the corresponding values when only multipoles 
$\ell>100$ are considered in the analysis.
\label{tab:significance_table1}}
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{$-$} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 1.15in{#\leaderfil}\tabskip=0pt&
\hbox to 0.6in{\hfil#\hfil}\tabskip=5pt&\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\omit\hfil Significance measure\hfil& $[2,600]$& $[2,1500]$& $[100,600]$& $[100,1500]$\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
 {No. of $p$=100\%}& 496/500& 496/500& 494/500& 496/500\cr
 {No. of $p>99\%$}& 499/500& 498/500& 496/500& 498/500\cr
{Mean $p$-value}& 490/500& 500/500& 498/500& 500/500\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table}

\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
  \caption{Significance of the correlations of dipole directions between 
high and low multipoles. Significance levels are defined similarly to
Table~\ref{tab:significance_table1}, but here 
$\theta_\mathrm{mean}$ is defined as the mean 
of the angular distances between all pairs of dipole directions where 
one is computed for 
$\ell_\mathrm{min}<\ell<\ell_\mathrm{lim}$
and the second direction for
$\ell_\mathrm{lim}<\ell<\ell_\mathrm{max}$.
Note that the global significance levels are only based on
$\ell_\mathrm{max}$ values selected over the full range 2--1500, since
high values of $\ell_\mathrm{lim}$ yield poor statistics for the 
smaller range 2--600.
The two last rows give significance levels 
for the case where we consider $\ell_\mathrm{min}=100$ in the analysis.
In some cases the data do not have any $p=100\%$ or $p>99\%$ occurences
in the given range. This is denoted by NA, as the given statistic
is not applicable for these cases. 
\label{tab:significance_table2}}
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{$-$} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{\hbox to 1.1in{#\leaderfil}\tabskip=20pt&
\hfil#\hfil\tabskip=13pt&\hfil#\hfil&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\omit&\hfil No. of\hfil&\hfil No. of\hfil&\hfil Mean\hfil\cr
\omit\hfil $\ell_\mathrm{lim}$\hfil& $p=100\%$& $p>99\%$& $p$-value\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
 100& 494/500& 500/500& 500/500\cr
 200& 499/500& 500/500& 500/500\cr
 300& 497/500& 500/500& 500/500\cr
 400& 496/500& 500/500& 500/500\cr
 500& NA& 473/500& 489/500\cr
 600& NA& NA& 317/500\cr
 200 ($\ell_\mathrm{min}=100$)& 500/500& 500/500& 500/500\cr
 300 ($\ell_\mathrm{min}=100$)& 492/500& 500/500& 500/500\cr
 400 ($\ell_\mathrm{min}=100$)& NA& 490/500& 492/500\cr
 500 ($\ell_\mathrm{min}=100$)& NA& 470/500& 487/500\cr
 600 ($\ell_\mathrm{min}=100$)& NA& NA& 267/500\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table}

We have also attempted to assess the degree to which the
significance of the asymmetry depends on a specific choice for
$\ell_{\rm max}$ by implementing several global statistics. 
Values for these are determined as follows.
\begin{enumerate}
\item The angle $\theta_{\rm mean}$ is calculated as a function of
  $\ell_\mathrm{max}$ both for the data and the simulations.
\item For a given $\ell_\mathrm{max}$, the fraction of simulations
  (out of 500) with a larger mean separation angle than for the real
  data is defined as the $p$-value for that $\ell_\mathrm{max}$.
\item This procedure is then repeated, treating each of the 500
  simulations in turn as if it were the real data, and computing a
  corresponding $p$-value from the fraction of the other 499 simulations
  that gives a larger $\theta_\mathrm{mean}$ than the selected
  simulation. Examples of such $p$-values as a function of
  $\ell_\mathrm{max}$ for the data are shown in
  Figs.~\ref{fig:significance} and \ref{fig:significance_llim500}.
\item We define three global statistics in the following manner.
  \begin{itemize}

  \item ``number of $p=100\%$'': for certain values of
    $\ell_\mathrm{max}$, each of the 500 simulations is found to have
    a larger mean separation angle than is determined for the real
    data, implying a corresponding $p$-value of 100\%. We then
    evaluate the number of $\ell_\mathrm{max}$ values for which this
    is the case.  Each of the simulations is then treated in turn as
    if it were the real data, and effectively the same quantity is
    determined by comparison to the other 499 simulations.  The
    fraction of all simulations that yield a smaller ``number of
    $p=100\%$'' than the real data is then used as a global statistic, shown
    in the first row in Table~\ref{tab:significance_table1}.

  \item ``number of $p>99\%$'': for certain values of
    $\ell_\mathrm{max}$, more than $99\%$ of the simulations exhibit
    larger mean separation angles than the data, implying a $p$-value
    of $>99\%$. We count the number of $\ell_\mathrm{max}$ values for
    which this applies. The same quantity is then evaluated for each
    simulation, treated in turn as if it were the real data (as
    above).  The fraction of all simulations that yield a smaller
    ``number of $p>99\%$'' than the real data is used as a second
    global statistic.

  \item ``mean $p$-value'': the mean $p$-value for the data is
    computed as an average over the set of $p$-values determined for
    each $\ell_\mathrm{max}$ (as in 2 above). A corresponding quantity
    is evaluated for each simulation, treated in turn as if it were
    the real data. The fraction of simulations with a lower ``mean
    $p$-value'' than for the data then forms the third global
    statistic.

  \end{itemize}
\end{enumerate}
We provide results for all three global statistics, since they reflect
different aspects of the significance of the asymmetry. The fact that
the global statistics indicate similar significance levels is evidence for
the robustness of the results.  We determine their values both for all
$\ell_\mathrm{max}$ available ($\ell_\mathrm{max}=2$--1500) and after
restricting $\ell_\mathrm{max}$ to 2--600, since we do not claim
any asymmetry beyond this value. The results are shown in
Table~\ref{tab:significance_table1}.
In addition, significance levels are also provided for the case when only
multipoles $\ell>100$ are included in the analysis. In this case,
strong evidence ($>99\%$) is still found for asymmetry from all global
measures.

We can also study the range of scales over which the asymmetry
persists using these global statistics and a modified definition of
$\theta_{\rm mean}$.  Here, this is computed as the mean of the
angular separations determined between all pairs of dipole directions
where one direction corresponds to the range
$\ell_\mathrm{min}<\ell<\ell_\mathrm{lim}$ and the second direction to
$\ell_\mathrm{lim}<\ell<\ell_\mathrm{max}$.
Figure~\ref{fig:significance_llim500} shows an example of the $p$-values
corresponding to this definition of $\theta_{\rm mean}$ for
$\ell_\mathrm{lim}=500$.  The high $p$-values indicated in the figure
for multipoles in the range $\ell=500$--600 show that the
corresponding dipole directions are strongly correlated with the
dipoles in the range $\ell=2$--500.
For most of the calculations, $\ell_\mathrm{min}=2$ and
$\ell_\mathrm{max}=1500$.  Table~\ref{tab:significance_table2}
presents the global significance levels for
$\ell_\mathrm{lim}=100,200,300,400,500$, and 600. We find that the dipole
directions at high and low multipoles are strongly correlated
up to $\ell=600$, although the significance is weakening for $\ell>500$. 
Indeed, when we consider multipoles
$\ell>600$ and $\ell_\mathrm{lim}>600$, we find no evidence for
asymmetry.  The table also provides similar significance levels 
for the case $\ell_\mathrm{min}=100$.

Although the global significance values in
Table~\ref{tab:significance_table2} show that the asymmetry is almost
insignificant for $\ell_\mathrm{lim}=500$, we must take into account
the fact that the global statistics look at the entire range
2--1500.  If the asymmetry disappears at, for example, $\ell=600$, then
the statistics would be too poor in the interval $\ell=500$--600 for this to
show up in the global significance measure for
$\ell_\mathrm{lim}=500$. For this reason we show in 
Fig.~\ref{fig:significance_llim500} the plot of $p$-values as a function of
$\ell_\mathrm{max}$ for $\ell_\mathrm{lim}=500$, showing that there is
a strong signal all the way to $\ell_\mathrm{max}=600$, after which it
disappears.  The continued evidence for asymmetry excludes the
possibility that the results in Fig.~\ref{fig:significance} are
dominated by the known low-$\ell$ signal, and supports the claim for
asymmetry persisting over the range $\ell=100$ to $600$. 


\begin{figure}[htbp!]
\begin{center}
\includegraphics[width=\hsize]{./section_5.0/section_5.3/section_5.3.1/figs/sig_flmax_ap3_nband1_deboost_frode_vs_originalclustering_llim500.pdf}

\caption{Derived $p$-values as a function of $\ell_\mathrm{max}$  
          for the deboosted {\tt SEVEM} 143\,GHz foreground-cleaned map.
         The $p$-values in this plot are based on the the mean of the
         angular separations determined between all pairs of dipole directions
         where one direction falls in the range $[\ell_{\lim}=500,\ell_\mathrm{max}]$
         and the second direction in the range  $[2,\ell_{\lim}=500]$.
         The significance is computed using 500 FFP6 simulated maps. 
          \label{fig:significance_llim500}}
\end{center}
\end{figure}

An alternative approach to studying power asymmetry is to determine
the ratio of the local power spectra computed in two opposing
directions on the sky \citep[e.g.,][]{eriksen2004b}.  Here, we
consider such a ratio defined for the two hemispheres centred on the
positive and negative poles of the power dipole fitted over a given
$\ell$ range.  A statistic can then be defined through the fractional
power ratio as follows:
\begin{equation}
\frac{\Delta C_{\ell}}{C_{\ell}} =
2\frac{C_{\ell}^{\rm{positive}}-C_{\ell}^{\rm{negative}}}{
C_{\ell}^{\mathrm{positive}}+C_{\ell}^{\mathrm{negative}}},
\end{equation}
where $C_{\ell}^{\mathrm{positive}}$ corresponds to the power spectrum
computed for the hemisphere centred on the positive pole, and
$C_{\ell}^{\mathrm{negative}}$ to the spectrum in the antepodal
direction. This can be compared to an ensemble of isotropic and
Gaussian simulations to determine whether significant excess power is
observed.  Figure~\ref{fig:cl} presents this quantity, binned into
blocks of 100 multipoles, for the hemispheres centred on the preferred
dipole direction determined for the {\tt SEVEM} 143\,GHz map over the
$\ell$ range $2$ to $600$, both before and after deboosting. It should
be apparent that, although the ratio lies systematically above zero
for $\ell<600$, only a few bins lie significantly outside the range of
values generated from simulations. The most significant bins are those
centred on $\ell = 50$ and $150$. Note that the observed values are
not directly comparable to the explicit dipolar modulation fits in
Sects.~\ref{sec:dipolar_modulation} and \ref{sec:BipoSH}. The ratio on
other scales is of smaller amplitude and lower significance.  We
re-emphasize that the claims of significant asymmetry presented in
this section are based on the alignment of the power distribution as a
function of angular scale, not on the corresponding amplitudes, nor on
the ratio of power in the antipodal hemispheres.  The ratio of power in the 
antipodal hemispheres is shown here for only illustrative purposes.


\begin{figure}[h!]
\begin{center}
\includegraphics[width=\hsize]{./section_5.0/section_5.3/section_5.3.1/figs/clratio_ap3_r90_meanl600_sevem143_deboost.pdf}
\caption{ Fractional power ratio, $\Delta C_{\ell}/C_{\ell}$, from
  antipodal sky regions, computed from the SEVEM 143\,GHz map before
  and after deboosting along the mean dipole direction for
  $\ell=2$ to $600$.  All spectra are evaluated on hemispheres using an
  apodized mask.  The grey lines show the same quantity evaluated for
  each of the 500 FFP6 simulations along their respective asymmetry
  axes. The green band shows the $68\%$ confidence region from these
  simulations.\label{fig:cl}}
\end{center}
\end{figure}

 In summary, we have presented evidence for power asymmetry in the
  \textit{Planck} data.  At high $\ell$, this is expected, since a
  dipolar modulation of the temperature anisotropy due to Doppler
  effects has been predicted, and subsequently detected, as detailed
  in a companion paper \citep{planck2013-pipaberration}.  When this is
  taken into account, significant power asymmetry can be claimed up to
  $\ell \sim 600$.




==> section_5.0/section_5.3/section_5.3.2/section_5.3.2.tex <==


\subsection{Dipole modulation}
%\subsubsection{Dipole modulation}
\label{sec:dipolar_modulation}

In Sect.~\ref{sec:power_asymmetry} it was shown that power asymmetry
is observed over a large range of angular scales in the \Planck\ data,
with a fairly consistent preferred axis.  No explicit parametric model
was assumed in the analysis. In this section, however, we only consider
large angular scales and revisit the
phenomenological model due to \citet{Gordon2005}, 
who proposed that the power asymmetry could be
described in terms of a multiplicative dipole modulation model of the
form $\mathbf{d} = (1 + A\,\vec{p}\cdot\vec{n}) \mathbf{s}_{\rm iso} +
\mathbf{n} \equiv \tens{M} \mathbf{s}_{\rm iso} + \mathbf{n}$, where
$A$ is the dipole amplitude, $\vec{p}$ is the dipole direction,
$\mathbf{n}$ denotes instrumental noise, and $\mathbf{s}_{\rm iso}$ is
an underlying isotropic CMB field. Both $\mathbf{s}_{\rm iso}$ and
$\mathbf{n}$ are assumed to be Gaussian random fields with covariance
matrices $\tens{S}$ and $\tens{N}$, respectively. Since
$\mathbf{s}_{\rm iso}$ is assumed to be isotropic, its covariance may
be fully specified by some angular power spectrum $C_{\ell,{\rm
    iso}}$.

\begin{figure}

\includegraphics[width=85mm]{./section_5.0/section_5.3/section_5.3.2/figs/modulation_amplitude_scale_88mm}\\

\includegraphics[width=85mm]{./section_5.0/section_5.3/section_5.3.2/figs/power_spectrum_amplitude_scale_88mm}\\

\includegraphics[width=85mm]{./section_5.0/section_5.3/section_5.3.2/figs/power_spectrum_tilt_scale_88mm}

\caption{Marginalized dipole modulation amplitude (top), power spectrum
  amplitude (middle) and power spectrum tilt (bottom) probability distributions as a function of smoothing 
  scale, shown for the {\tt Commander} CMB solution. 
}
\label{fig:dipmod_qn}
\end{figure}

 \begin{figure}
\includegraphics[width=85mm]{./section_5.0/section_5.3/section_5.3.2/figs/power_spectrum_contours_88mm}\\

\includegraphics[width=85mm]{./section_5.0/section_5.3/section_5.3.2/figs/modulation_amplitude_88mm}\\

\includegraphics[width=88mm]{./section_5.0/section_5.3/section_5.3.2/figs/mod_direction_colombi1_python_88mm}
\caption{Consistency between component separation algorithms as
measured by the dipole modulation likelihood. The top panel shows the
marginal power spectrum amplitude for the 5\deg\ smoothing scale,
the middle panel shows the dipole modulation amplitude, and the bottom
panel shows the preferred dipole directions. The coloured area
indicates the 95\% confidence region for the {\tt Commander} solution, while
the dots shows the maximum-posterior directions for the other maps. }
\label{fig:dipmod_n32_5deg}
\end{figure}


In the following we present the results from a direct likelihood
analysis of this model, similar to those described by
\citet{eriksen2007} and \citet{Hoftuft2009} for the 3- and 5-year \textit{WMAP} data,
respectively. Since this method requires matrix inversions and
determinant evaluations, the computational expense scales as
$\mathcal{O}(N_{\rm pix})$, and it is therefore only feasible at
low resolution. Specifically, we consider maps downgraded to a
{\tt HEALPix} pixel resolution of $N_{\rm pix}=32$, smoothed to angular
resolutions ranging from $5$\deg \, to $10$\deg, ensuring sufficient
bandwidth limitation at this pixelization. All four \Planck\ CMB map
solutions are included in the analysis; however, note that the
Galactic plane is handled differently in each of the four
approaches. Specifically: for the {\tt Commander} map the region inside the
corresponding analysis mask has been replaced with a Gaussian
constrained realization, eliminating the possibility that bright
Galactic foreground residuals might leak outside the mask during
degradation \citep{planck2013-p08}; for {\tt SMICA} and {\tt NILC} a smaller
region is replaced with Wiener filtered data; and for {\tt SEVEM} no special
precautions are taken.

%--------------------------------
\begin{table*}[tmb] % table* does a two-column table
\begingroup % this + \endgroup at the end keep table things local
\newdimen\tblskip \tblskip=5pt
\caption{Summary of dipole modulation likelihood results as a function of
scale for all four \Planck\ CMB solutions.
}%@
\label{tab:dipmod_results}
%\nointerlineskip
\vskip -3mm
\footnotesize % good font size for a table, but can be changed
\setbox\tablebox=\vbox{ %
\newdimen\digitwidth % see \S\,16.12 for the purpose of the next 10 lines
\setbox0=\hbox{\rm 0}
\digitwidth=\wd0
\catcode`*=\active
\def*{\kern\digitwidth}
%
\newdimen\errwidth
\setbox0=\hbox{$\!pm 22$}
\errwidth=\wd0
\catcode`?=\active
\def?{\kern\errwidth}
% 
\newdimen\signwidth
\setbox0=\hbox{$^{+0.020}_{-0.021}$}
\signwidth=\wd0
\catcode`!=\active
\def!{\kern\signwidth}
% 
\halign{ \hbox to 1.7in{#\leaderfil}\tabskip=2pt& \hfil
  #\hfil \hspace{0.2cm}& \hfil #\hfil\hspace{0.2cm}& \hfil
  #\hfil \hspace{0.2cm}& \hfil #\hfil \hspace{0.2cm}& \hfil #\hfil\tabskip=0pt\cr
% template goes here. See examples.
\noalign{\doubleline}
\omit \hfill Data set \hfill& FWHM [\deg]& $A$& $(l,b)$ [\deg]& $\Delta\ln\mathcal{L}$& Significance\cr
\noalign{\vskip 2pt\hrule\vskip 2pt}
{\tt Commander}& $*5.0$& $0.078^{+0.020}_{-0.021}$&
$(227,-15)\pm 19$& 8.8& $3.5\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt NILC}& $*5.0$& $0.069^{+0.020}_{-0.021}$&
$(226,-16)\pm 22$& 7.1& $3.0\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt SEVEM}& $*5.0$& $0.066^{+0.021}_{-0.021}$&
$(227,-16)\pm 24$& 6.7& $2.9\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt SMICA}& $*5.0$& $0.065^{+0.021}_{-0.021}$&
$(226,-17)\pm 24$& 6.6& $2.9\,\sigma$\cr
\noalign{\vskip 4pt}
\textit{WMAP}-5 {\tt ILC}& $*4.5$& $0.072^{+0.021}_{-0.021}$&
$(224,-22)\pm 24$& 7.3& $3.3\,\sigma$  \cr
\noalign{\vskip 8pt}
{\tt Commander}& $*6.0$& $0.076^{+0.024}_{-0.025}$&
$(223,-16)\pm 25$& 6.4& $2.8\,\sigma$ \cr
\noalign{\vskip 4pt}
{\tt NILC}& $*6.0$& $0.062^{+0.025}_{-0.026}$&
$(223,-19)\pm 38$& 4.7& $2.3\,\sigma$ \cr
\noalign{\vskip 4pt}
{\tt SEVEM}& $*6.0$& $0.060^{+0.025}_{-0.026}$&
$(225,-19)\pm 40$& 4.6& $2.2\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt SMICA}& $*6.0$& $0.058^{+0.025}_{-0.027}$&
$(223,-21)\pm 43$& 4.2& $2.1\,\sigma$\cr
\noalign{\vskip 8pt}
{\tt Commander}& $*7.0$& $0.062^{+0.028}_{-0.030}$& $(223,
*-8)\pm 45$& 4.0& $2.0\,\sigma$ \cr
\noalign{\vskip 4pt}
{\tt NILC}& $*7.0$& $0.055^{+0.029}_{-0.030}$&
$(225,-10)\pm 53$& 3.4& $1.7\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt SEVEM}& $*7.0$& $0.055^{+0.029}_{-0.030}$&
$(226,-10)\pm 54$& 3.3& $1.7\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt SMICA}& $*7.0$& $0.048^{+0.029}_{-0.029}$&
$(226,-11)\pm 58$& 2.8& $1.5\,\sigma$\cr
\noalign{\vskip 8pt}
{\tt Commander}& $*8.0$& $0.043^{+0.032}_{-0.029}$&
$(218,-15)\pm 62$& 2.1& $1.2\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt NILC}& $*8.0$& $0.049^{+0.032}_{-0.031}$&
$(223,-16)\pm 59$& 2.5& $1.4\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt SEVEM}& $*8.0$& $0.050^{+0.032}_{-0.031}$&
$(223,-15)\pm 60$& 2.5& $1.4\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt SMICA}& $*8.0$& $0.041^{+0.032}_{-0.029}$&
$(225,-16)\pm 63$& 2.0& $1.1\,\sigma$\cr
\noalign{\vskip 8pt}
{\tt Commander}& $*9.0$& $0.068^{+0.035}_{-0.037}$&
$(210,-24)\pm 52$& 3.3& $1.7\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt NILC}& $*9.0$& $0.076^{+0.035}_{-0.037}$&
$(216,-25)\pm 45$& 3.9& $1.9\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt SEVEM}& $*9.0$& $0.078^{+0.035}_{-0.037}$&
$(215,-24)\pm 43$& 4.0& $2.0\sigma$\cr
\noalign{\vskip 4pt}
{\tt SMICA}& $*9.0$& $0.070^{+0.035}_{-0.037}$&
$(216,-25)\pm 50$& 3.4& $1.8\,\sigma$\cr
\noalign{\vskip 4pt}
\textit{WMAP}-3 \tt{ILC}& $*9.0$& 0.114!&
$(225,-27)$?& 6.1& $2.8\,\sigma$\cr
\noalign{\vskip 8pt}
{\tt Commander}& $10.0$& $0.092^{+0.037}_{-0.040}$&
$(215,-29)\pm 38$& 4.5& $2.2\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt NILC}& $10.0$& $0.098^{+0.037}_{-0.039}$&
$(217,-29)\pm 33$& 5.0& $2.3\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt SEVEM}& $10.0$& $0.103^{+0.037}_{-0.039}$&
$(217,-28)\pm 30$& 5.4& $2.5\,\sigma$\cr
\noalign{\vskip 4pt}
{\tt SMICA}& $10.0$& $0.094^{+0.037}_{-0.040}$&
$(218,-29)\pm 37$& 4.6& $2.2\,\sigma$\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
}}
\endPlancktable % this command is defined in Planck.tex.
\endgroup
\end{table*}

After degrading each map to the appropriate resolution, we add random
uniform Gaussian noise of $1\,\mu{\rm K}$ rms to each pixel to
regularize the covariance matrix. All pixels inside the U73 mask
are excluded, and we adopt the difference maps between the raw
\Planck\ LFI 30\,GHz and HFI 353\,GHz maps and the {\tt SMICA} CMB
solution as two foreground templates, tracing low- and high-frequency
foregrounds, respecively. We marginalize over these Galactic
foreground templates, $\vec{f}$, as well as four monopole and
dipole templates, by adding corresponding terms of the form $\alpha
\vec{f}\vec{f}^{\rm T}$ to the total data covariance matrix, where
$\alpha$ is set to a numerically large value.

Before writing down the likelihood for $A$ and $\vec{p}$, a choice has
to be made for the power spectrum,$C_{\ell,{\rm iso}}$. We follow
\citet{eriksen2007}, and adopt a simple two-parameter model of the form $C_{\ell,{\rm iso}} =
q\left(\ell/\ell_{\rm pivot}\right)^n C_{\ell,{\rm fid}}$, where  the fiducial spectrum, $C_{\ell,{\rm fid}}$, is
the best-fit \Planck\ spectrum, and $q$ and $n$ describe an amplitude scaling
and spectral tilt with respect to this. The full model therefore includes five
free parameters, namely three dipole parameters and two power spectrum
parameters. 
Introducing the two parameters $q$ and $n$ addresses the known issue
that the low-$\ell$ power spectrum is low by about 2--2.5$\,\sigma$
compared with the overall best-fit $\Lambda$CDM spectrum
\citep{planck2013-p08,planck2013-p11}.  Ignoring this creates a
tension with the underlying isotropic model that
results in the analysis measuring a combination of both asymmetry and power
mismatch.

Taking advantage of the fact that both the signal and noise are
assumed Gaussian, the exact likelhiood may be written down in a
convenient closed form:
\begin{equation}
\mathcal{L}(A, \vec{p},q,n) \propto
\frac{e^{-\frac{1}{2}\vec{d}^{\rm T}\left(\tens{M}^{\rm T}\tens{S}\tens{M}+\tens{N}
    + \alpha \sum_i \vec{f}_i\vec{f}_i^{\rm T}\right)^{-1}\vec{d}}}
  {\sqrt{|\tens{M}^{\rm T}\tens{S}\tens{M}+\tens{N}+ \alpha \sum_i \vec{f}_i\vec{f}_i^{\rm T}|}}.
\end{equation}
This expression is the basis of all calculations presented in the
rest of this section.

Due to the high computational expense associated with these
evaluations, we do not compute the full joint five-parameter model in
this analysis, only conditionals of it. However, we iterate once in a
Gibbs-sampling like approach, by maximizing each conditional to obtain
an approximation to the full maximum-likelihood solution. That is, we
first map out the dipole likelihood for the 5\deg\ FWHM case,
fixing the power spectrum at the fiducial spectrum,
$\mathcal{L}(A,\vec{p}|q=1,n=0)$, and locate the maximum-likelihood
dipole parameters. Then we map out the corresponding power spectrum
conditional,
$\mathcal{L}(q,n|A_{m\ell},\vec{p}_{m\ell})$. Finally, we
update the dipole likelihood with these power spectrum parameters, and
evaluate the final results. Note that the power spectrum and dipole
modulation parameters are only weakly correlated, and this procedure
is therefore close to optimal. Furthermore, the approach is also
conservative, in the sense that it will always underestimate the
significance of the dipole modulation model; the derived
maximum-likelihood value will always lie slightly below the true
maximum-likelihood point.

 \begin{figure}
\includegraphics[width=88mm]{./section_5.0/section_5.3/section_5.3.2/figs/log_likelihood_difference_88mm}
\caption{Log-likelihood difference between the best-fit dipole modulation model
  and the fiducial isotropic model as a function of smoothing
  scale. Horizontal dashed lines indicate 1, 2, and $3\,\sigma$
  thresholds.}
\label{fig:dipmod_dlnL}
\end{figure}

The results from these calculations are summarized in
Table~\ref{tab:dipmod_results}, listing results for all four \Planck\ CMB maps
at angular scales between 5 and 10\deg\ FWHM. For easy reference,
we also list the results from the corresponding 3- and 5-year \textit{WMAP}
analyses \citep{eriksen2007,Hoftuft2009}. Note that the former was
performed at a {\tt HEALPix} resolution of $N_{\rm side}=16$ and the
latter at an angular resolution of 4.5\deg\ FWHM.

Fig.~\ref{fig:dipmod_qn} shows marginals for $A$, $q$ and $n$,
as derived from the {\tt Commander} CMB solution for all smoothing
scales. At least two interesting points can be seen here. First, while
there is clearly significant scatter in the derived dipole modulation
amplitude for different smoothing scales, as originally pointed out by
\citet{Hanson2009b}, all curves appear to be consistent with a single
value of $A \sim 0.07$. No other single value fits all scales equally
well. Second, it is interesting to note that the low-$\ell$ power
spectrum derived here is consistent, but not without some tension,
with the fiducial spectrum, $(q,n) = (1,0)$, around 1.5--$2\,\sigma$. In
particular, there appears to be a slight trend toward a steeper positive spectral index as more weight is put on the larger scales, a
result already noted by \textit{COBE}-DMR. The same conclusion is reached using
the low-$\ell$ \Planck\ likelihood, as described
in \citet{planck2013-p08}. 

In Fig.~\ref{fig:dipmod_n32_5deg} we compare the results from all four
CMB solutions for the 5\deg\ FWHM smoothing scale. Clearly the
results are consistent, despite the use of different algorithms and
different treatments of the Galactic plane, demonstrating robustness
with respect to the details of the analysis methods. Further, we also
note that these results are consistent with those derived from the
5-year \textit{WMAP} {\tt ILC} map by \citet{eriksen2007},
demonstrating robustness across experiments. On the other hand, it is
notable that a higher dipole amplitude was found for
the 3-year \textit{WMAP} {\tt ILC} map using a
larger mask at 9\deg\ FWHM.

In Fig.~\ref{fig:dipmod_dlnL} we show the log-likelihood difference
between the derived maximum-likelihood point and the isotropic model,
$A=0$, as a function of smoothing scale. The power spectrum parameters
are kept fixed at the best-fit values for both points, leaving three
additional parameters for the dipole model. The dashed horizontal
lines indicate the 1, 2, and $3\,\sigma$ confidence regions for three
degrees of freedom. As has been noted previously in the literature,
these significance levels vary with smoothing scale. Taken at face value,
the results presented here are suggestive but clearly not decisive,
resulting in an unchanged situation with respect to earlier
reports. This is of course not unexpected, given that \textit{WMAP} is already
strongly cosmic variance limited at these angular scales. 

The critical question is whether the trend seen at smaller angular
scales in Fig.~\ref{fig:dipmod_dlnL} continues, or if the apparent
likelihood peak at 5\deg\ FWHM happens to be a local
maximum. \citet{Hanson2009b}, and later \citet{bennett2010}, address
this question through a computationally cheaper quadratic estimator,
allowing them to extend a similar analysis to small scales.  In doing
so, they claim that the apparent likelihood peak at 5\deg\ is
indeed a local maximum, and the evidence for the modulation model
falls off when more data are included.

In this respect, it should be noted that the dipole modulation model
was originally proposed by \citet{Gordon2005} as a simple
phenomenological characterization of the more general power
asymmetry. In particular, it assumes that the modulation amplitude,
$A$, is equally strong on all scales. 
From both the results presented
by \citet{Hanson2009b}\,and \citet{bennett2010} and qualitatively shown in
Fig.~\ref{fig:cl},
this appears not to hold, as the
fractional hemispherical power difference is clearly smaller at $\ell
> 300$ than at $\ell<100$. 
Furthermore, an alternative power modulation analysis in
\citet{planck2013-p09a} finds that the asymmetry on these scales 
has an amplitude of order $1\%$.
The data, therefore, are not consistent with a simple constant-amplitude
dipole modulation of the power. On the other hand, the preferred direction
derived from the current low-$\ell$ analysis is remarkably consistent
with the high-$\ell$ direction derived in
Sect.~\ref{sec:power_asymmetry}. A proper modulation model may
therefore need additional spatial structure beyond that
proposed by \citet{Gordon2005}, as already suggested
by \citet{Hoftuft2009} and \citet{Moss2011}.

Finally, Doppler boosting as presented in \citet{planck2013-pipaberration}
creates a signature similar to that observed here. However, the present
effect is clearly distinct from this, both because the magnitudes of
the two effects are very different --- $A_{\rm{boost}}\sim\, 0.002$
versus $A_{\rm{asym}}\sim\, 0.07$ --- and because the two preferred
directions are different --- $(l,b)_{\rm{boost}} =
(264\deg,48\deg)$ versus
$(l,b)_{\rm{asym}}=(227\deg,-15\deg)$. We have
analysed the 143 and 217\,GHz frequency maps, cleaned from
foregrounds using the {\tt SEVEM} algorithm and de-boosted using the best-fit
parameters from \citet{planck2013-pipaberration}, and consistently find
(very slightly) higher significance levels for these data. The best-fit
axis moves by approximately 5\deg\ and 2\deg\ at 143 and 217\,GHz,
respectively. The results presented here, therefore,
are conservative with respect to boosting corrections.





==> section_5.0/section_5.3/section_5.3.tex <==
\subsection{Dipolar asymmetry}
\label{sec:dipolar_asymmetry}

%In Sect.~\ref{sec:hemispherical_asymmetry} 
In previous sections, we have seen evidence for a break in isotropy
related to the discontinuous distribution of power in hemispheres on
the sky. \citet{bennett2010} distinguishes between such an asymmetry
and one where the CMB signal is modulated across the sky by a dipolar
term. Studies of such a dipolar asymmetry have been motivated by the
phenomenological proposal of \citet{Gordon2005} that the power
asymmetry could be described in terms of a multiplicative dipole
modulation model. In addition, Doppler boosting due to
our motion with respect to the CMB rest frame is expected to induce a
dipolar modulation aligned with the CMB dipole at the
$\mathcal{O}(10^{-3})$ level; a statistically significant detection of
this effect by \Planck\ is presented by
\citet{planck2013-pipaberration}.

%power spectrum asymmetry
\input{./section_5.0/section_5.3/section_5.3.1/section_5.3.1}

% Dipole modulation
\input{./section_5.0/section_5.3/section_5.3.2/section_5.3.2}

%BiPoSh
%\input{./section_5.0/section_5.3/section_5.3.3/section_5.3.3}


==> section_5.0/section_5.4/section_5.4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NEW COMMANDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cg}[6]{\mathcal{C}^{#1 #2}_{#3 #4 #5 #6}}
\newcommand{\ncap}{\mathbf{\hat{n}}}
\newcommand{\nnbr}{\nonumber \\}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Generalized modulation}  
%\subsection{BipoSH tests of isotropy}
\label{sec:BipoSH}

In this section, we study a generalization of the dipolar modulation
field analysed in Sect.~\ref{sec:dipolar_modulation} using the
Bipolar Spherical Harmonic (BipoSH) formalism.  For a statistically
isotropy sky,
the spherical harmonic space two-point correlation matrix is diagonal,
and, given by the angular power spectrum $C_\ell$.  The BipoSH
representation provides a natural, mathematically complete,
generalization of the angular power spectrum that captures statistical
isotropy violations
via coefficients that are a completely equivalent representation of
the spherical harmonic correlation matrix,
%
\begin{equation}
A^{LM}_{\ell_1 \ell_2} = \sum_{m_1 m_2} \langle a_{\ell_1
m_1} a_{\ell_2 m_2} \rangle \cg L M {\ell_1} {m_1} {\ell_2} {m_2} \,.
\end{equation} 
%
This relationship combines the off-diagonal spherical harmonic
correlations into a bipolar multipole $L,M$ --- analogous to the total
angular momentum addition of states.  The CMB angular power spectrum
corresponds to the $L=0$ BipoSH coefficients $C_\ell = (-1)^\ell
A^{00}_{\ell\ell'} \delta_{\ell\ell'} /\sqrt{2\ell+1}$.

A simple model that results in the violation of statistical isotropy
arises from the modulation of the of the CMB sky,
%
\begin{equation}
\label{eq:cmb_mod}
 T(\vec{n})=T_{0}(\vec{n})\left( 1+ M(\vec{n}) \right) \,, 
\end{equation}
%
where $T(\vec{n})$ represents the modulated CMB sky, $T_{0 }(\vec{n})$
is the underlying (statistically isotropic) random CMB sky and
$M(\vec{n})$ is a fixed, zero-mean, dimensionless, modulation field.
The modulation signal, if any, is expected to be weak and allows
quadratic terms in $M$ to be neglected. The BipoSH coefficients for
the modulated CMB field ($L>0$) are then given by
%
\begin{eqnarray} 
\label{biposh_modulation}
A^{LM}_{\ell_1 \ell_2}&=&\bar{A}^{LM}_{\ell_1 \ell_2}
 + m_{LM}G^{L}_{\ell_1 \ell_2}\, ;
\nnbr
G^{L}_{\ell_1 \ell_2}&=&\frac{C_{\ell_1}+C_{\ell_2}}{\sqrt{4 \pi}}
%\frac{\Pi_{\ell_1}\Pi_{\ell_2}}{\Pi_{L}} \mathcal{C}^{L0}_{\ell_1 0 \ell_2 0}   \,,
\sqrt{\frac{(2\ell_1+1)(2\ell_2+1)}{(2L+1)}} \mathcal{C}^{L0}_{\ell_1 0 \ell_2 0}   \,.
\end{eqnarray}
%
Here $\bar{A}^{LM}_{\ell_1 \ell_2}$ corresponds to the BipoSH
coefficients of the unknown, but statistically isotropic, unmodulated
CMB field, $m_{LM}$ are the spherical harmonic coefficients of the
modulating field ($L>0$), and $C_\ell$ is the best-fit CMB angular
power spectrum.  The statistically isotropic nature of the unmodulated
CMB sky implies that the expectation values of $\bar{A}^{LM}_{\ell_1
  \ell_2}$ vanish for $L>0$, leading to the estimator for the
modulation field harmonics,
%
\begin{equation}
\hat{m}_{LM} = \sum_{\ell_1 \ell_2}  w^{L}_{\ell_1 \ell_2} \frac{\hat{A}^{LM}_{\ell_1 \ell_2}}{G^{L}_{\ell_1 \ell_2}} \,,
\label{modest}
\end{equation}
denoted by the overhat \citep{Hanson2009b}. The weights $w^{L}_{\ell_1
  \ell_2}$ for a minimum variance estimate for the modulation field
correspond to
%
\begin{equation}
w^{L}_{\ell_1 \ell_2} = N \left(\frac{G^L_{\ell_1 \ell_2}}{\sigma_{A^{LM}_{\ell_1 \ell_2}}}\right)^2,
\end{equation}
%
where $N$ is a normalization chosen such that $\sum_{\ell_1 \ell_2
}w^{L}_{\ell_1 \ell_2} =1$.  The BipoSH representation further enables
an estimate of the modulation field to be made over specific angular scales by
windowing regions in multipole space in the sum over multipoles
$\ell_1, \ell_2$ in Eq.~\ref{modest}. This additional information
could be very useful in identifying the origin of the statistical
isotropy violation, which could be either cosmological or due to
systematic artefacts \citep[see ][]{AH-TS,AH-TS1}.

First, we limit our analysis to the four low resolution $N_{\rm
  side}=32$ CMB maps used in Sect.\ref{sec:dipolar_modulation}
and reconstruct the modulation maps for each of them at the same low
resolution. The U73 mask
is applied to the reconstructed modulation maps before computing
$m_{LM}$. The pseudo-power $m_L$ is corrected for the mask applied to
the modulation maps. Specifically, for the case of dipole modulation,
the pseudo-power $m_L$ is related to the dipole amplitude by $A=1.5
\sqrt{m_1 / \pi}$.


\begin{figure}
\begin{center}
\includegraphics[width=\hsize]{./section_5.0/section_5.4/figures/significance.pdf}
\end{center}
\caption{ Significance of the modulation power, $L(L+1) m_L/2\pi$,
  at bipolar multipoles $L$. The modulation spectra obtained from the
  four component separation maps ({\tt C-R}, {\tt NILC}, {\tt SEVEM},
  and {\tt SMICA}) are consistent with each other.  Dipole ($L=1$)
  modulation power is detected in all the spectra at a significance
  ranging from $2.9$ to $3.7\,\sigma$.  The solid black lines denote the
  $3\,\sigma$ significance thresholds. There is no significant power
  detected at higher multipole of the modulation field,
  $1<L\le32$.}\label{fig:biposh_modulation_significance}
\end{figure}

\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{ Amplitude ($A$) and
  direction of the dipole modulation in Galactic coordinates. The measured
  values of the dipole amplitude and direction are consistent for all maps. The
  corresponding dipole power for the
  {\tt SMICA} map is seen at a detection significance of $3.7\,\sigma$, as
  shown in Fig.~\ref{fig:biposh_modulation_significance}. For the values in the
  third column  $(\sigma_l = 15.4 , \sigma_b = 15.1)$.}\label{tab:prob_chisq}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 0.7in{#\leaderfil}\tabskip=2pt&
\hfil#\hfil\tabskip=5pt&\hfil#\hfil\/\tabskip=0pt\cr
\noalign{\doubleline}
\omit\hfil Map \hfil& $A$& $(l,b)$ [\deg]\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
{\tt C-R}& $0.072^{+0.010}_{-0.010}$&  $(218.9,-21.4)$\cr
\noalign{\vskip 4pt}
{\tt NILC}& $0.070^{+0.010}_{-0.010}$& $(220.3,-20.2)$\cr
\noalign{\vskip 4pt}
{\tt SEVEM}& $0.065^{+0.011}_{-0.011}$& $(221.7,-21.4)$\cr
\noalign{\vskip 4pt}
{\tt SMICA}& $0.073^{+0.010}_{-0.010}$& $(217.5,-20.2)$\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 

A dipole modulation ($L=1$) signal is detected at $3\,\sigma$
significance in all the maps, as shown in
Fig.~\ref{fig:biposh_modulation_significance}.  The amplitude and
direction of the dipole modulation match those obtained via a
likelihood analysis in Sect.~\ref{sec:dipolar_modulation}.  The BipoSH
representation of modulation confirms the dipole modulation signal
found in the low-resolution map.  Since this approach enables the
reconstruction of any general small amplitude modulation field, the
BipoSH representation places constraints on the power in the
modulation field at all higher (bipolar) multipoles allowed by the
resolution of the CMB maps.

\begin{figure}
\begin{center}
\includegraphics[width=\hsize]{./section_5.0/section_5.4/figures/dipole_as_func_of_cmb_multipole.pdf}
\end{center}
\caption{Measured dipole modulation ($L=1$) power in CMB multipole bins.
This uses the CMB multipole dependence of the BipoSH (modulation)
power $L(L+1)m_L/2\pi$, which can be dissected into bins in $\ell$-space.  We
establish that significant power in the dipole modulation is limited
to $\ell=2$--64 and does not extend to the higher CMB multipoles considered.
The vertical grid lines denote the CMB multipole $\ell$-bins.}
\label{fig:dipole_384}
\end{figure}

We then extend the analysis to higher resolution using maps at $N_{\rm
  side}=256$ for {\tt Commander} and $N_{\rm side}=2048$ for {\tt
  NILC}, {\tt SEVEM}, and {\tt SMICA}, in order to study the above
effect in more detail. We repeat the analysis on these higher
resolution maps using the U73 mask.
Contrary to our expectations based on a scale-independent (i.e., no
$\ell$-dependence) model,
the significance of the dipole does not increase in the high
resolution maps. We then subdivide the $\ell$-range up to
$\ell_{\rm max}=384$ into uniform bins of size $\Delta \ell =64$.  As seen in
Fig.~\ref{fig:dipole_384}, we recover the dipole modulation at over
$3\,\sigma$ significance only for the lowest bin
($\ell = 2$--64). This is consistent with the results in
Sect.~\ref{sec:dipolar_modulation} and the BipoSH analysis on the
corresponding low resolution maps shown in
Fig.~\ref{fig:biposh_modulation_significance}. However, the amplitude
of the dipole is consistent with zero within $3\,\sigma$ for all of the
higher $\ell$-bins considered. This suggests that the simple
modulation model in Eq.~\ref{eq:cmb_mod} is inadequate and should
minimally allow for the amplitude, $A(\ell)$, of the dipole to depend
on CMB multipole, $\ell$. Although this may appear to be a more
complex model, it does not necessarily lack motivation.  It is readily
conceivable that physical mechanisms that cause a dipolar modulation
of the random CMB sky would be scale-dependent and possibly
significant only at low wavenumbers. More importantly, such a dipole
modulation has also been noted in low resolution \textit{WMAP} data
\citep{eriksen2007,Hoftuft2009}. More recently, \citet{bennett2010}
also comment (without being quantitative) that the effect is present
in the \textit{WMAP} maps, but limited to low $\ell$ and conclude that
the $\ell$-dependence rules out a simple modulation explanation. The
fact that two independent experiments find this intriguing statistical
isotropy violation points to a non-instrumental origin.

The search for modulation power recovered from higher multipoles of
the CMB maps yields a null result, as seen in
Fig.~\ref{fig:dipole_384}. However, due to our motion with respect to
the CMB rest frame, it is expected that the observed CMB map is
statistically anisotropic, and this has been demonstrated in
\cite{planck2013-pipaberration}.  To understand why a Doppler boost
induced anisotropy is not detected by the modulation estimator,
we first implement an equivalent description in terms of the Doppler
boost induced BipoSH coefficients,
\begin{eqnarray} 
\label{biposh_boost}
A^{1M}_{\ell_1 \ell_2}~~~&=&\bar{A}^{1M}_{\ell_1 \ell_2} + \beta_{1M}G^{1}_{\ell_1 \ell_2} \, ,\\
G^{1}_{\ell_1 \ell_2}~~~&=&\Bigg\lbrace b_{\nu}[G^{1}_{\ell_1 \ell_2}]^{\mathcal{M}} - [G^{1}_{\ell_1 \ell_2}]^{\phi} \Bigg\rbrace \times \nnbr
%\frac{\Pi_{\ell_1}\Pi_{\ell_2}}{\Pi_{L}} \mathcal{C}^{L0}_{\ell_1 0 \ell_2 0}   \,,
& &\sqrt{\frac{(2\ell_1+1)(2\ell_2+1)}{12\pi}} \mathcal{C}^{10}_{\ell_1 0 \ell_2 0}   \, ,
\nnbr
\left[G^{1}_{\ell_1 \ell_2}\right]^{\mathcal{M}}&=&\left[ C_{\ell_1}+C_{\ell_2} \right] \, , 
\nnbr
\left[G^{1}_{\ell_1 \ell_2}\right]^{\phi}~&=&\left[ C_{\ell_1}+C_{\ell_2}\right] \nnbr &+&  \left[ C_{\ell_1}-C_{\ell_2}\right] \left[ \ell_1(\ell_1+1)-\ell_2(\ell_2+1)\right] /2 \, ,\nonumber
\end{eqnarray}
where $\beta_{1M} = \int d\vec{n} Y_{1M}(\vec{n})
\vec{\beta}\cdot\vec{n}$, $\vec{\beta}=\vec{v}/c$ denotes the peculiar
velocity of our local rest frame with respect to the CMB, and $b_{\nu}$
is the frequency dependent boost factor,
as discussed in more detail in \citet{planck2013-pipaberration}.
Since we perform our analysis on component-separated
maps, we use the same approximation, $b_{\nu}=2.5$, as advocated 
there. 
%In fact, these maps will contain contributions from the full
%set of nine \textit{Planck} frequency maps with relative weights that
%depend on angular scale.

A minimum variance estimator for $\beta_{1M}$ is given by the
expression in Eq.~\ref{modest}, with the shape function
$G^L_{\ell_1 \ell_2}$ replaced by the corresponding
Doppler boost term given in Eq.~\ref{biposh_boost}.
\begin{figure}
\begin{center}
\includegraphics[width=\hsize]{./section_5.0/section_5.4/figures/doppler_dipole_as_func_of_cmb_multipole.pdf}
\end{center}
\caption{Dipolar ($L=1$) power measured from different
    CMB multipole bins, as denoted by the vertical grid
    lines.  Here the Doppler estimator is used to reconstruct the
    Doppler field ($\vec{\beta}\cdot \hat{n}$) from {\tt SMICA}.
    Significant dipolar power is limited to $\ell = 2$--64
    and does not extend to the higher CMB multipoles considered.}
\label{fig:doppler_dipole_384}
\end{figure}

The significant power detected in the reconstructed Doppler field
  ($\vec{\beta}\cdot \hat{n}$), from the CMB multipole bin $\ell=2$ to
  $64$, shown in Fig.~\ref{fig:doppler_dipole_384}, corresponds to an
  effective $|\vec{\beta}|=2.6\times 10^{-2}$. Note that this value of
  $\vert \vec{\beta} \vert$ is an order of magnitude larger than that
  of our local motion. Further, we find that the dipole direction is
  consistent with Fig.~3 of \citet{planck2013-pipaberration}, which
  depicts the reconstructed direction of the Doppler boost as a
  function of the CMB multipole.

  Figure~\ref{fig:compare-noise} presents a comparative study of the
  sensitivity of the two estimators, Doppler and modulation, and
  depicts the reconstruction noise for the two estimators as a
  function of the maximum CMB multipole used. The horizontal red
  dash-dotted line at $|\vec{\beta}|=1.23\times 10^{-3}$ denotes the
  expected value of the Doppler signal induced by our local
  motion. The blue dash-dotted line denotes the Doppler boost signal
  as seen by the modulation estimator and is expected to be enhanced
  by an effective factor of $b_\nu$ for the component separated maps.

  For the case of the modulation estimator, it is seen that the
  Doppler boost is not expected to significantly contaminate the
  modulation signal up to $\ell_{\rm max}\simeq 700$, establishing the
  fact that the boost effect corresponding to our local motion is not
  strong enough to affect the modulation signal seen at low CMB
  multipoles. However, it is expected to significantly add to the
  modulation signal at higher CMB multipoles.

  Fig.~\ref{fig:compare-noise} also clearly shows that the Doppler
  estimator is expected to recover the Doppler boost signal at a high
  significance. The figure also establishes that at $\ell \la 500$, the
  local motion contribution is not detectable in the Doppler boost
  search, and hence the signal measured by the Doppler estimator in
  the range $\ell=2$--64, depicted in
  Fig.~\ref{fig:doppler_dipole_384}, is expected to be linked to the
  modulation signal seen at low CMB multipoles.

\begin{figure}
\begin{center}
\includegraphics[width=\hsize]{./section_5.0/section_5.4/figures/compare-rec-noise-mod-vs-dop.pdf}
\end{center}
\caption{ Reconstruction noise power associated with the
    modulation (blue) and Doppler (red) estimators as a function of
    the maximum CMB multipole used. The solid lines correspond to the
    case of noise-free CMB maps, while the dashed lines correspond to
    the case where the characteristic \textit{Planck} instrument noise
    is taken into account.  The red dash-dotted horizontal line
    denotes the expected signal level of the boost due to our local
    motion, while the blue dash-dotted horizontal line denotes the
    enhanced boost amplitude as seen by the modulation estimator. The
    blue dotted line denotes the effective Doppler boost signal as
    seen by the modulation estimator after accounting for the effects
    of aberration induced by the boost. Also note that the
    reconstruction errors shown in red are derived for the total
    dipole power, rather than the amplitude in a particular direction,
    and hence are higher by a factor of $\sqrt{3}$ as compared to the
    errors for individual directions reported in
    \citet{planck2013-pipaberration}.}
\label{fig:compare-noise}
\end{figure}

It is, of course, also possible to extract the BipoSH coefficients $A^{LM}_{\ell_1
  \ell_2}$, up to the maximum multipole $\ell_{\rm max}$ allowed by
the full resolution \Planck\ maps at modest computational expense.
This allows us to address a specific indication of statistical
isotropy violation previously reported in the
literature. \citet{bennett2010} found non-zero BipoSH power spectra,
$A^{20}_{\ell\ell}$ and $A^{20}_{\ell\ell+2}$, at very high statistical
significance in the \textit{WMAP} maps as determined in ecliptic
coordinates, corresponding to a quadrupolar power asymmetry in the CMB
sky.  The BipoSH spectra peaked at around $\ell=250$, and the differences
in the BipoSH signal determined from two different frequency bands
indicated a non-cosmological origin.  Furthermore, the azimuthal
symmetry of this BipoSH signal in ecliptic coordinates suggested that
it had its origin in some unaccounted-for systematic effect. The
findings of \citet{Hanson2010a} and \citet{Joshi2012} strongly suggest that the
signal arises due to an incomplete treatment of beam asymmetries in
the data. \citet{bennett2012} have subsequently noted that
analysis of the \textit{WMAP}-9
beam-deconvolved maps no longer shows the signal.

We have computed the $A^{20}_{\ell\ell}$ and $A^{20}_{\ell\ell+2}$ values in
ecliptic coordinates for the full resolution \Planck\ CMB maps, as
shown in Fig.~\ref{fig:biposhL2M0}. The analysis yields no evidence
for BipoSH coefficients that deviate significantly from zero.  This
provides conclusive observational evidence from independent CMB
measurements that the \textit{WMAP} result could only have arisen due
to instrumental artefacts in that data set.

\begin{figure}
\begin{center}
\includegraphics[width=\hsize]{./section_5.0/section_5.4/figures/biposhL2M0.pdf}
\end{center}
\caption{ BipoSH power spectra $A^{20}_{\ell \ell}$ and
  $A^{20}_{\ell \ell+2}$ obtained from the four component separation
  maps ({\tt C-R}, {\tt NILC}, {\tt SEVEM}, and {\tt SMICA}) are
  consistent with each other. Note that no significant $\left( >
    3\,\sigma \right)$ detections are found. This independently
  establishes the fact that the quadrupolar BipoSH detections made by
  \textit{WMAP} were due to \textit{WMAP}-specific instrument
  systematics. }\label{fig:biposhL2M0}
\end{figure}

In summary, a generalized search for power in the modulation field
reveals a statistically significant dipolar modulation of the CMB sky
on large angular scales $(\ell \la 64)$, with an amplitude of
about $0.07$.  Conversely, no quadrupolar modulation is observed,
reconfirming the systematic origin of the corresponding anomaly seen
in the \textit{WMAP}-7 data.


==> section_5.0/section_5.5/section_5.5.1/section_5.5.1.tex <==

\subsubsection{Point-parity asymmetry}
\label{sec:point_parity_asymmetry}

The CMB sky map may be considered as the sum of even and odd parity
functions.  Previously, an odd point-parity preference (hereafter
parity asymmetry) was observed in the \textit{WMAP} 3-, 5{-}, and 7-year
data releases
\citep{LandOdd,kim2010,kim_anomalous_pa,Gruppuso2010,aluri2012,Naselsky2011}. In
this section we investigate the parity asymmetry for the \Planck\
temperature anisotropy power spectra derived with a quadratic maximum
likelihood (QML) estimator applied to the {\tt Commander-Ruler}, {\tt
  NILC}, {\tt SEVEM}, and {\tt SMICA} maps at $N_{\rm side}=32$, and
with a pseudo-$C_{\ell}$ estimator at $N_{\rm side}=64$.


From the CMB anisotropy field defined on the sky, $T(\vec{n})$, we may construct symmetric and antisymmetric functions using
the coordinate inversion $\vec{n}\rightarrow -\vec{n}$:
%
\begin{eqnarray}
T^+(\vec{n})=\frac{T(\vec{n})+T(-\vec{n})}{2}\, ;
\hspace{0.5cm}
T^-(\vec{n})&=&\frac{T(\vec{n})-T(-\vec{n})}{2}.
\end{eqnarray}
%
Therefore, $T^+(\vec{n})$ and $T^-(\vec{n})$ have even
and odd parity, respectively. When combined with the parity property of spherical
harmonics, $Y_{\ell m}(\vec{n})=(-1)^{\ell}\,Y_{\ell m}(-\vec{n})$,
we obtain
%
\begin{eqnarray}
T^+(\vec{n})&=&\sum_{\ell, m} a_{\ell m}\,Y_{\ell m}(\vec{n})\,\Gamma^+(\ell), 
\nonumber\\
T^-(\vec{n})&=&\sum_{\ell,m} a_{\ell m}\,Y_{\ell m}(\vec{n})\,\Gamma^-(\ell),
 \label{T_odd}
\end{eqnarray}
%
where $n$ is an integer, and
%\begin{eqnarray}
$\Gamma^+(\ell)=\cos^2(\ell\pi/2)$, and $\Gamma^-(\ell)
=\sin^2(\ell\pi/2)$.
%\end{eqnarray}

A significant power asymmetry between even and odd multipoles may thus
be interpreted as a preference for a particular parity of the
anisotropy pattern, connected to the parity asymmetry of the metric
perturbations at scales above 1--4\,Gpc \citep{kim2010}.  For
investigation of the parity asymmetry we may consider the following
quantities \citep{kim2010}:
%
\begin{eqnarray}
P^{+}(\ell)&=&\sum^{\ell}_{n=2} \,\Gamma^+(n) \frac{n(n+1)}{2\pi} \: C_n\, ;\nonumber\\
P^{-}(\ell)&=&\sum^{\ell}_{n=2} \,\Gamma^-(n)\, \frac{n(n+1)}{2\pi} \: C_n\, ;\nonumber\\
g(\ell)&=&\frac{P^{+}(\ell)}{P^{-}(\ell)}\, .
\label{g}
\end{eqnarray}
%
Here $P^{+}$ and $P^{-}$ are the sum of $n(n+1)/2\pi \: C_n$ for even
and odd multipoles respectively; the ratio $P^{+}/P^{-}$ is associated
with the degree of parity asymmetry, where a value of $P^+/P^-<1$
indicates odd-parity preference, and $P^+/P^->1$ indicates even-parity
preference.

\begin{figure}[htb]
\centerline{\includegraphics[width=\hsize]{./section_5.0/section_5.5/section_5.5.1/figs/Planck_parity_and_P-values_lmax_30.png}}
\caption{{\it Upper}: the parity estimator $g(\ell)$ versus $\ell$ for \cru\
(black diamonds), {\tt NILC} (red diamonds), {\tt SEVEM} (blue
diamonds), and {\tt SMICA} (green diamonds).
{\it Lower}: $p$-value for \cru\ (black solid line),
 {\tt NILC} (red line), {\tt SEVEM} (blue line), and {\tt SMICA} (green line).
} 
\label{P_ratio}
\end{figure}

Following \citet{kim2010}, we will discuss the range of multipoles
$2\le \ell\le 30$, which belongs to the Sachs-Wolfe plateu of the TT
power spectrum, where $\ell (\ell+1) C_{\ell}\approx \mathrm{constant}$.  In
order to make a rigorous assessment of the statistical significance of
parity asymmetry at low $\ell$, we have compared $g(\ell)$ for the
\Planck\ power spectra
with 1000 simulated CMB maps 
based on  the fiducial \Planck\ cosmological model. We compute power spectra
using a QML-estimator \citep{Gruppuso:2009ab} as
applied to data at $N_{\rm side}=32$ with the U73 mask applied. This
yields practically identical power spectrum results for the same $\ell$-range determined
with a pseudo-$C_{\ell}$ estimator applied to maps at $N_{\rm side}=64$.

In Fig~\ref{P_ratio} we show the $g(\ell)$-parameter for the \Planck\ power
spectra and the corresponding $p$-value$(\ell)$. The $p$-value denotes the
fraction of simulations in which the obtained value of $P^+/P^-$ is as
low as that observed in the data. Note that the
results from the different \Planck\ CMB maps yield consistent 
shapes for the $g(\ell)$ parameter and $p$-value$(\ell)$. The
parity asymmetry at $\ell = 22$ is most anomalous, with a corresponding $p$-value
in the range 0.002--0.004.
Finally, the statistical significance of the parity
asymmetry (i.e., low $p$-value) increases when we increase
$\ell_{\mathrm{max}}$ up to 22--25.  Therefore, the 
odd parity preference cannot simply be attributed to the low
quadrupole power. It is plausible the low quadrupole power is not an isolated
anomaly, but that it shares an origin with the odd parity
preference \citep[see for details][]{kim2010,Naselsky2011,kim_anomalous_pa}.



















==> section_5.0/section_5.5/section_5.5.2/section_5.5.2.tex <==

\def\bh{{\mathbf h}}
\def\bp{{\mathbf p}}
\def\bg{{\mathbf g}}
\def\by{{\mathbf y}}
\def\bx{{\mathbf x}}
\def\bk{{\mathbf k}}
\def\br{{\mathbf r}}
\def\bn{{\mathbf n}}
\def\bv{{\mathbf v}}
\def\bq{{\mathbf q}}
\def\II{\mathcal{I}}
\def\B{{\mathbf B}}
\def\E{{\mathbf E}}
\def\J{{\mathbf J}}
\def\tk{\tilde{k}}  
\def\tK{\tilde{K}}
\def\tbk{\tilde{\bk}}
\def\de{\delta}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsubsection{Mirror Parity}
\label{sec:mirror_parity_asymmetry}

In this section we investigate the properties of the \Planck\
temperature low-resolution maps under reflection with respect to a
plane.  This search for hidden mirror symmetries and anti-symmetries
complements the tests for parity asymmetry, presented in
Sect.~\ref{sec:point_parity_asymmetry}.  \citet{Starobinsky:1993yx}
showed how a hidden mirror symmetry might be connected to the
non-compact $T^1$ topology, or to a compact $T^3$ topology in which
one topological scale is much shorter than the others. The CMB pattern
would then exhibit a mirror symmetry with respect to the plane defined
by the two large dimensions.  Mirror symmetry has been searched for in
the \textit{COBE}-DMR data in \citet{deOliveiraCosta:1995td}, resulting
in a lower limit for the scale of the compact dimension as 4\,Gpc (see
also \citealt{Gurzadyan:2007ic,BenDavid:2011fc} for other more recent
analysis).  \citet{Finelli:2011zs} analysed hidden mirror symmetry and
anti-symmetry properties of the \textit{WMAP} 7-year {\tt ILC}
temperature map, finding a preferred direction that could be
considered anomalous at the 93\% confidence level with anti-symmetry
properties. This direction lies close to the one defining the
hemispherical asymmetry.

Following \citet{Finelli:2011zs}, we consider the following estimators
\begin{equation}
S^{\pm} (\vec{n_i}) = {1 \over N_{\rm pix}} \sum_{j=1}^{N_{\rm pix}}
\left[ {1 \over 2} \left( {\delta T \over T} (\vec{n_j}) \pm 
{\delta T \over T}(\vec{n_k}) \right)\right]^2\,,
\label{spm}
\end{equation}
where the sum is meant over the {\tt HEALPix} pixels, $N_{\rm pix}$,
${\delta T / T} (\vec{n_j})$ is the CMB temperature anisotropy measured
at the pixel pointed by the unit vector $\vec{n_j}$, and $\vec{n_k}$ is
the opposite direction of $\vec{n_j}$ with respect to the plane defined
by $\vec{n_i}$, i.e.,
\begin{equation}
\vec{n_k} = \vec{n_j} -2\, ( \vec{n_i} \cdot \vec{n_j}) \vec{n_i}\,.
\end{equation}
The estimator $S^{+}$ ($S^{-}$)
can be written explicitly in the harmonic domain and its averaged value over isotropic random 
realization is $\sum_\ell (\ell+1) C_\ell B^2_\ell/(4\pi)$ ($\sum_\ell \ell C_\ell B^2_\ell/(4\pi)$), 
where $B_\ell$ is the Gaussian beam applied to the low-resolution maps.

We compute the quantities $S^{\pm}$ for each of the 3072 directions
defined by {\tt HEALPix} resolution $N_\mathrm{side}=16$ map, by
allowing the $j$
and $k$ indices to run over the pixels of the low resolution
foreground cleaned full-sky maps.  We perform the same analysis on 1000
simulated skies and store the minimum and maximum value of $S^{\pm}$ for each of
these to correct our statistics for the else-where effect. 

The minimum value for the $S^+$ estimator is reached for
the plane defined by Galactic coordinates
%$(\theta,\phi)=(107^\circ,264^\circ)$ 
$(l,b) = (264^\circ, -17^\circ)$
for all four foreground cleaned maps, 
with a significance of $0.5\%$
({\tt Commander-Ruler}), $1.4\%$ ({\tt NILC}), $3.1\%$ ({\tt SEVEM}),
and $8.9\%$ ({\tt SMICA}). The top panel of Fig.~\ref{plotmirrorsym}
shows the minimum value of $S^{+}$ for each of the four methods and
compared to the MC simulations computed for {\tt Commander-Ruler},
which is considered to be representative.

The minimum value for the $S^-$ estimator is found for a direction
which depends slightly on the foreground cleaned CMB map considered
and is close to the one associated with the cosmological dipole. This
minimum value is not statistically significant for any of the
foreground cleaned CMB maps (see bottom panel of
Fig.~\ref{plotmirrorsym}).


\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.65]{./section_5.0/section_5.5/section_5.5.2/figs/MinSplus_fullsky.pdf}
\includegraphics[scale=0.65]{./section_5.0/section_5.5/section_5.5.2/figs/MinSMinus_fullsky.pdf}
\caption{Top panel: $S^+$ statistic. The vertical lines show the minimum value for the
  estimator as computed on low resolution 
  {\tt C-R}, {\tt NILC}, {\tt SEVEM}, and {\tt
    SMICA} maps.
  The grey histogram shows the same quantity
  computed from 1000 simulated maps processed by {\tt C-R}.  Bottom panel:
  as above for $S^-$.}
\label{plotmirrorsym}
\end{center}
\end{figure}

The anomalous anti-symmetry direction found in the \Planck\ CMB data
is close to that found for the dipolar modulation in
Sect.~\ref{sec:dipolar_modulation}, suggesting possible connections
between them. The direction which minimizes $S^+$ ($S^-$) for \Planck\
is almost exactly the same as the one found for the \textit{WMAP}
7-year {\tt ILC} map in \citet{Finelli:2011zs}.




==> section_5.0/section_5.5/section_5.5.tex <==
\subsection{Parity asymmetry}
\label{sec:parity_asymmetry}

% point parity asymmetry (P. Naselsky)
\input{./section_5.0/section_5.5/section_5.5.1/section_5.5.1}

% plane parity asymmetry (F. Paci)
\input{./section_5.0/section_5.5/section_5.5.2/section_5.5.2}

==> section_5.0/section_5.6/section_5.6.tex <==
\subsection{The Cold Spot}  
\label{sec:cold_spot}

The Cold Spot was identified in the \textit{WMAP} first year
data~\citep{vielva2004} through the estimation of the kurtosis of the
Spherical Mexican Hat Wavelet~\citep[SMHW,
e.g.,][]{martinezgonzalez2002} coefficients, and
confirmed~\citep{cruz2005} by analysing the area of the SMHW
coefficients above/below a given threshold. Since its detection, the
Cold Spot has been extensively studied and verified with a large battery of
statistical
probes~\citep[e.g.,][]{mukherjee2004,cayon2005,mcewen2005,cruz2007a,rath2007,vielva2007,pietrobon2008,gurzadyan2009,rossmanith2009}. A
complete review of the Cold Spot can be found in~\cite{vielva2010a},
including a discussion on possible explanations of its nature.

The analysis of the kurtosis of the SMHW coefficients has already been 
addressed in Sect.~\ref{sec:wavelet_statistics}. We have checked
that the kurtosis of the coefficients corresponding to the four \Planck\
cleaned frequency maps is larger than the expected value obtained from
simulations, with a modified upper tail probability of around $0.01$. This is
compatible with the value obtained from \textit{WMAP}.

Nevertheless, the Cold Spot is more robustly described in terms of a
morphological quantity: the area of the SMHW coefficients above/below
a given threshold. At a given scale $R$ and threshold $\nu$, the cold
($A_R^{-\nu}$) and hot ($A_R^{+\nu}$) areas of the SMHW coefficients
are defined as:
%
\begin{eqnarray}
A_R^{-\nu} & \equiv & \# \lbrace \omega_T\left(R,p\right) < -\nu \rbrace \, ;\\
A_R^{+\nu} & \equiv & \# \lbrace \omega_T\left(R,p\right) < +\nu \rbrace \, .\nonumber 
\end{eqnarray}
%
Here $\#$ represents the number operator, i.e, it indicates
for how many pixels $p$, the specific condition defined between the
braces is satisfied. 

Table~\ref{tb:cs_areas_test}  summarizes the results for the hot and
cold areas determined for the four CMB maps analysed with the U73
mask  (and its
associated exclusions masks).
The cold area is anomalous at scales
between $R=200$ and $R=300$\arcmin, similar to the sizes already
highlighted with the kurtosis analysis. We see that the higher the
threshold, the smaller the upper tail probability associated with the \Planck\ CMB
map. In particular, the cold area has a upper tail probability of 0.003 at $\nu >
4\,\sigma_R$ and for $R=300$\arcmin. 

%
\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Upper tail probability (UTP, in \%) associated to the cold (top) and
  hot (bottom) areas. Results are given for a $\nu >
  4\,\sigma_R$ threshold and for the four \Planck\ CMB maps. The three
  most significant scales associated to the Cold Spot are shown. Analysis
  performed on the exclusions masks associated with the U73
  mask.}                             
\label{tb:cs_areas_test}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 0.7in{#\leaderfil}\tabskip=1pt&
\hfil#\hfil\tabskip=1pt& \hbox to 0.4in{\hfill#\hfill}& \hfill#\hfill& \hfill#\hfill& \hfill#\hfill\/\tabskip=0pt\cr         
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\omit&\multispan4 \hfil UTP \hfil\cr
\noalign{\vskip -6pt}
\omit&\omit&\multispan4\hrulefill\cr
\omit\hfil Area \hfil& \hfil Scale [\arcmin] \hfil\tabskip=2pt& \hfil {\tt C-R} \tabskip=10pt\hfil& \hfil {\tt NILC} \hfil& \hfil {\tt SEVEM} \hfil& \hfil {\tt SMICA}\hfil\cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
\omit& 200& 1.6& 1.1& 1.2& 1.1\cr
Cold& 250& 0.3& 0.3& 0.3& 0.3\cr
\omit& 300& 0.3& 0.3& 0.3& 0.3\cr 
\noalign{\vskip 5pt}
\omit& 200& 2.3& 1.6& 1.8& 1.6\cr
 Hot& 250& 2.7& 2.2& 2.4& 2.2\cr
 \omit& 300& 4.9& 3.7& 4.1& 3.8\cr
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 

Notice that the most significant deviation comes from the cold
area, although the hot area is marginally
compatible. However, the cold area represents the most robust detection
of an anomaly, 
since it is robust to the mask employed (see Tables~\ref{tb:cs_areas2}
and~\ref{tb:cs_areas3}).
%
\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Upper tail probability (in \%) associated to the cold (top) and
hot (bottom) areas. Results are given for a $\nu >
  4\,\sigma_R$ threshold and for the four \Planck\ CMB maps. The three
  most significant scales associated to the Cold Spot are shown. Analysis
  performed on the exclusions masks associated with the CG70
  mask. An ellipsis (\ldots) indicates that no area above that threshold was found on
  the data.}                           
\label{tb:cs_areas2}   
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 0.7in{#\leaderfil}\tabskip=1pt&
\hfil#\hfil\tabskip=1pt& \hbox to 0.4in{\hfill#\hfill}& \hfill#\hfill& \hfill#\hfill& \hfill#\hfill\/\tabskip=0pt\cr       
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\omit&\multispan4 \hfil UTP \hfil\cr
\noalign{\vskip -6pt}
\omit&\omit&\multispan4\hrulefill\cr
\omit\hfil Area \hfil& \hfil Scale [\arcmin] \hfil\tabskip=2pt& \hfil {\tt C-R} \tabskip=10pt\hfil& \hfil {\tt NILC} \hfil& \hfil {\tt SEVEM} \hfil& \hfil {\tt SMICA}\hfil\cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
\omit& 200& 1.0& 1.0& 0.9& 1.0\cr
Cold& 250& 0.3& 0.3& 0.3& 0.3\cr
\omit& 300& 0.2& 0.2& 0.3& 0.2\cr  
\noalign{\vskip 5pt}
\omit& 200& 15.1& 14.5 & 14.6 & 14.5\cr
Hot& 250& \dots& \dots& \dots& \dots\cr
\omit& 300& \dots& \dots& \dots& \dots\cr
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 



%
\begin{table}[tmb]  
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Upper tail probabilities (in \%) associated with the cold (top) and
hot (bottom)   areas. Results are given for a $\nu >
  4\,\sigma_R$ threshold and for the four \Planck\ CMB maps. The three 
  most significant scales associated to the Cold Spot are shown. Analysis 
  performed on the exclusions masks associated with the 
  CG60 mask. An ellipsis (\ldots) indicates that no area above that threshold 
  was found on the data.}                          
\label{tb:cs_areas3}
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
\halign{\hbox to 0.7in{#\leaderfil}\tabskip=1pt&
\hfil#\hfil\tabskip=1pt& \hbox to 0.4in{\hfill#\hfill}& \hfill#\hfill& \hfill#\hfill& \hfill#\hfill\/\tabskip=0pt\cr       
\noalign{\doubleline}
\noalign{\vskip -1pt}
\omit&\omit&\multispan4 \hfil UTP \hfil\cr
\noalign{\vskip -6pt}
\omit&\omit&\multispan4\hrulefill\cr
\omit\hfil Area \hfil& \hfil Scale [\arcmin] \hfil\tabskip=2pt& \hfil {\tt C-R} \tabskip=10pt\hfil& \hfil {\tt NILC} \hfil& \hfil {\tt SEVEM} \hfil& \hfil {\tt SMICA}\hfil\cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
\omit& 200& 1.1& 0.9& 0.8& 0.9\cr
Cold& 250& 0.1& 0.1& 0.1& 0.1\cr
\omit& 300& 0.1& 0.1& 0.1& 0.1\cr   
\noalign{\vskip 5pt}
\omit&  200& \dots& \dots& \dots& \dots\cr
Hot& 250& \dots& \dots& \dots& \dots\cr
\omit& 300& \dots& \dots& \dots& \dots\cr
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
\endPlancktable                    % ends one-column \halign
%\endPlancktablewide                 % ends two-column \halign
\endgroup
\end{table} 



The information provided in the previous Tables is also represented
(for the $R = 300$\arcmin\ scale) in Fig.~\ref{fig:cs_area}. In
these panels we show the anomalous cold (in blue) and
hot (in red) areas for thresholds $\nu > 3.0\sigma_R$ as determined from the {\tt
  SMICA} map. The most extreme value (in terms of $\sigma_R$) of each area 
is indicated.
%
\begin{figure}
\begin{center}
\includegraphics[width=8.0cm]{./section_5.0/section_5.6/figs/smhwc_smica_R0300_mk1p00_th3p0.png}
\includegraphics[width=8.0cm]{./section_5.0/section_5.6/figs/smhwc_smica_R0300_mk0p70_th3p0.png}
\includegraphics[width=8.0cm]{./section_5.0/section_5.6/figs/smhwc_smica_R0300_mk0p60_th3p0.png}
\caption{\label{fig:cs_area} SMHW coefficients at $R=300$ arc minutes,
  above (and below) a $+3.0\,\sigma$ ($-3.0\,\sigma$) threshold. Results for the three masks considered in the
  analysis are shown: U73 mask (top); CG70 (middle); and CG60
  (bottom). }
\end{center}
\end{figure}
%
The coldest area corresponds to the Cold Spot
with the minimum value of the wavelet coeficient at the position
$(209\deg,-57\deg)$ in Galactic coordinates,
whereas the hotest area has already been identified in the
\textit{WMAP} data~\citep[e.g.,][]{vielva2007} as an anomalous hot
spot. This does not depends signifincantly on the mask considered in the analysis.
From these results it is clear that the Cold Spot anomaly is present 
in both the \textit{WMAP} and \Planck\ data. 












==> section_5.0/section_5.7/section_5.7.tex <==
\subsection{Interpretation of anomalies}
\label{sec:interpretation}

The results presented here in Sect.~\ref{sec:anomalies_revisited}
demonstrate that many features previously observed in the
\textit{WMAP} data are present also in the \Planck\ sky.  This
agreement between two independent experiments effectively rules out
the possibility that their origin lies in systematic artefacts present
in either data set. In particular, there is evidence for a violation
of statistical isotropy at least on large angular scales in the
context of the \Planck\ fiducial sky model. Moreover, a power
asymmetry extends to scales corresponding to $\ell \simeq$ 600, whilst
fits at low $\ell$ to a model containing a dipole modulation field
yield results in excess of 3$\,\sigma$ significance. In addition, there
is evidence from such fits that the low-$\ell$ spectrum of the
\Planck\ data departs from the fiducial spectrum in both amplitude and
slope. These results could have profound implications for
cosmology. It is therefore pertinent to consider whether a model can
be proposed to provide a common origin for the anomalies.

The microwave sky is manifestly non-Gaussian and anisotropic, with
known contributions from Galactic astrophysical foregrounds, lensing
of CMB anistropies by the intervening matter distribution, and the
ISW. However, the excellent performance of the component separation
algorithms used here in rejecting diffuse foregrounds argues strongly
against known Galactic emission as the source of the anomalies.

\citet{schwarz2004}, \citet{Copi2007}, \citet{maris2011} and
\citet{hansen2012} suggested that diffuse Solar System emission could
contribute to the observed structure on large angular scales, although
it is not expected that the classical Zodiacal Light Emission or
Kuiper Belt objects are responsible. \citet{planck2013-pip88} presents
the current \Planck\ contribution to the modelling of the Zodiacal
cloud. Moreover, the association of the anomalies with the ecliptic
reference frame seems, at best, to be confined to the very largest
angular scales, since the preferred direction determined for the
dipolar modulation field analysis is separated from the south ecliptic
pole by more than $45^\circ$, with even larger separations found for
the power asymmetry direction.

Another possibility is that the anomalies have their origin in the
local Universe. According to \cite{Francis2009}, the removal of the
ISW signal originating within the volume at $z < 0.3$ from
\textit{WMAP} data reduces the significance of the apparent alignment
between the CMB quadrupole and octopole and the Cold Spot.
\citet{efstathiou2010} have used the same correction to yield an
increase in the structure of the two-point correlation function for
angular separations less than 60\deg, that had been noted as
apparently anomalous since the first \textit{WMAP} data release.
A future possibility is that \Planck\ itself will be able to
reconstruct the ISW signal and test its impact on issues related to
isotropy and non-Gaussianity. \citet{planck2013-p14} presents maps of
the effect based on the current data release.

Of more interest to us is that the anomalies are genuinely
cosmological in origin.  In that context, obvious candidate models
include those with simply or multi-connected topology.  In a companion
paper \citep{planck2013-p19}, a subset of such models are considered and the signatures
of their specific correlation structures on the sky are searched
for. However, no detections are found, but rather the scale of
topology is limited to be of order the diameter of the last-scattering
surface or greater. More interestingly, they reconsider Bianchi
VII$_{\rm h}$ models that were previously demonstrated to show statistical
correlation with the \textit{WMAP} data 
\citep{jaffe2005,jaffe:2006b,bridges2007,mcewen2013},
albeit with parameters inconsistent with standard cosmological
parameters. In this new analysis, the Bianchi parameters are
physically coupled to the cosmological ones, yielding no evidence for
a Bianchi VII$_{\rm h}$ cosmology. However, as before, when treated simply
as a template for structure contained in the CMB sky, a best-fit
pattern is found to be in good agreement with the old results. Previous
analyses \citep{jaffe2005,cayon2006,mcewen2006} have shown that when
the CMB sky is corrected for such a template, many of the large-scale
anomalies are no longer present at a statistically significant level.
It is likely that such an effect will persist for Bianchi-corrected
\Planck\ data, and we have made an explicit test as to whether the
best-fit Bianchi template can also explain the presence of phase
correlations. We therefore repeated the surrogate analysis from
Sect.~\ref{sec:scaling_indices} for the appropriately corrected {\tt SMICA}
map. Figure~\ref{fig:s-maps2} presents the result for the
corresponding significance map. It is clear that the signature for
hemispherical asymmetry is drastically reduced, thereby rendering the signal
formally statistically insignificant. Thus, the best-fit Bianchi model
can also account for the asymmetries induced by higher order phase
correlations. It should also be noted that subtracting the
best-fit Bianchi template from the data, outside the U73 mask,
explains the anomalous skewness and kurtosis values but not the
variance, for which the corresponding lower tail probabilities are $0.008$,
$0.166$, and $0.306$, respectively.
Given the lack of consistency of the physical parameters
of the model with the \Planck\ cosmological model, 
the results obtained using Bianchi-subtracted input
maps might be considered moot, however, the morphology of the maps
may provide insight into the type of underlying structures associated
with the anomalies.


\begin{figure}
\begin{center}
\includegraphics[width=8.8cm]{./section_5.0/section_5.2/section_5.2.3/figs/smap_smica-bianchi.pdf}
\caption{\label{fig:s-maps2} Same as Fig.~\ref{fig:s-maps1} but with the best fit Bianchi template 
subtracted from the {\tt SMICA} map.}
\end{center}
\end{figure}

Although the Cold Spot is also rendered statistically insignificant by
the Bianchi template, other possible explanations about its nature
have been considered, including the late evolution of the large-scale
structure~\citep[e.g.,][]{inoue2006,inoue2007}, the Sunyaev-Zeldovich
effect~\citep[e.g.,][]{cruz2008}, residual
foregrounds~\citep{cruz2006}, or a cosmic texture~\citep[e.g.,][]{cruz2007b}. 
Further tests based on gravitational lensing~\citep{das2009} or 
CMB polarization~\citep{Vielva2011} have been suggested to confirm or reject 
some of the proposed explanations.


The presence of primordial magnetic fields (PMFs) due to either pre-
or post-recombination mechanisms could also provide a physical basis
for some of the anomalies discussed in this paper. Specifically, PMFs
with coherence scales comparable to the present day horizon could
result in Alfv\'en waves in the early Universe that generate specific
signatures on the sky via the Doppler and integrated Sachs-Wolfe
effects.  In particular, a preferred angular direction in the CMB
anisotropy can be induced \citep{DKY,kim09} that leads to structure in
the spherical harmonic mode correlation matrix \citep{kahniashvili08}.
Appendix~\ref{sec:PMFs} presents a search for the predicted
correlations between harmonic modes separated by $\Delta \ell=0,\, \pm
2$, and $\Delta m=0,\,\pm 1,\,\pm 2$, allowing constraints to be placed on the
Alfv\'en wave amplitude. Further constraints on PMFs based on the power
spectrum and bispectrum have been provided in \citet{planck2013-p11} and 
\citet{planck2013-p09a}, respectively. 

To conclude, when analysing a data set as complex and rich as that
provided by \Planck, some statistical outliers will be
expected. However, it should be clear that the evidence for some of
the large-angular scale anomalies is significant indeed, yet few
physically compelling models have been proposed to account for them,
and none so far that provide a common origin. The dipole modulation
model that was analysed here was phenomenologically motivated, and is
detected in the data at relatively high significance. Whether it can resolve the
anomalous nature of other observed features remains to be evaluated.


==> section_6.0/section_6.0.tex <==
%\section{Primordial Magnetic Fields}
%\section{Constraints on non-standard models}

% {\bf These sections should be compressed as much as possible, key
%   results only, and refer to the specific papers for full details. Do
%   we include the primordial magnetic fields results here? The
%   stochastic background of PMFs is bispectrum related, should go in
%   that paper? The Alfven waves relate to a preferred direction, and if
%   retained could go in the isotropy section or Geometry/Topology?}

%\emph{Here results on Primordial Magnetic Fields derived from the bispectrum and the phase correlation tests 
%are included.}

%Here we summarise the constraints on non-standard models as presented
%in part in the companion papers P09a, P19 and P20.

%PLEASE, DO NOT UNCOMMENT THE INFLATION; STRINGS AND TOPOLOGY SECTIONS. THEY ARE SUPPOUSE TO NOT BE SUMMARIZED HERE
%Constraints on non-standard inflationary models
%\input{./section_6.0/section_6.1/section_6.1}

%Constraints on topological defects
%\input{./section_6.0/section_6.2/section_6.2}

%Constraints on geometry and topology
%\input{./section_6.0/section_6.3/section_6.3}

%Constraints on Primordial Magnetic Fields
\input{./section_6.0/section_6.4/section_6.4.tex}


==> section_6.0/section_6.4/section_6.4.tex <==
\section{Constraints on Alfv\'en waves}
\label{sec:PMFs}

Observations of synchrotron emission and Faraday rotation provide
increasing evidence that large-scale astrophysical systems in the
Universe are pervaded by magnetic fields. These huge systems include the
Ly-$\alpha$ forest and intercluster regions~\citep[see][for a
review]{kronberg09}. Both pre- and post-recombination mechanisms could
result in a background of nano-gauss fields that might be detectable
in large-scale structures or the CMB,
although at present no imprints of these Primordial Magnetic Fields
(PMFs) have been detected therein.

Here, we report our findings based on an analysis of the \Planck\ data
to search for the the predicted signature of statistical anisotropy
due to PMFs.
Specifically, PMFs with coherence scales comparable to the present day
horizon may induce and sustain Alfv\'en waves in the early Universe
that can leave observable imprints on the CMB via the Doppler and
integrated Sachs-Wolfe effects.  In particular, this results in a
preferred angular direction in the CMB anisotropy, therefore breaking
statistical isotropy (\citealt{DKY}, \citealt{kim09}).

\citet[]{DKY} showed that cosmological Alfv\'en waves generate a
fractional CMB anisotropy for a Fourier mode $\vec{k}$:
%
\begin{eqnarray}
\frac{\delta T}{T_0}({\vec{n}},\vec{k}) \approx \vec{n}\cdot
\vec{\Omega}(\vec{k},\eta_{\rm last})  
= \vec{n}\cdot \vec{\Omega_0}\; v_{\rm A} k\,\eta_{\rm last}\;\vec{B}\cdot \vec{k}  \, ,
\end{eqnarray}
%
where $\vec{n}$ denotes sky direction, $\vec{B}$
is a unit vector in the direction of the coherent PMF,
$\vec{\Omega}(\vec{k},\eta_{\rm last})$ is the Gauge invariant
linear combination associated with vector perturbations, $\eta_{\rm
  last}$ denotes the conformal time at the moment of baryon-photon
decoupling, and $T_0$ is the CMB monopole temperature 2.7255\,\hbox{K}
\citep{Fixsen2009}.  \citet[]{DKY} assumed that the vector
perturbations are initially created by some random stochastic PMF and
have the following statistical properties over an ensemble of
universes:
%
\begin{eqnarray}
\langle \Omega^i_0(\vec{k})\,\Omega^j_0(\vec{k})\rangle =(\delta_{ij}-
k_i\,k_j) P(k).
\end{eqnarray}
Here, $P(k)$ is the power spectrum assumed to follow a simple power
law \citep{DKY}:
\begin{eqnarray} 
P(k)=A_v \frac{k^{n_v}}{{k_0}^{n_v+3}},\label{P}
\end{eqnarray}
%
where $k_0$ is a pivot wavenumber set to $0.05/\mathrm{Mpc}$ in this
analysis.  The Alfv\'en wave velocity is given by \citep{DKY}:
\begin{eqnarray} 
v_{\rm A} =\frac{B}{2\sqrt{\pi(\rho_{\rm r}+p_{\rm r})}}\approx 4\times10^{-4}\frac{B}{10^{-9}\mathrm{Gauss}},\label{v_A}
\end{eqnarray}
where $\rho_{\rm r}$ and $p_{\rm r}$ are the density and the pressure of photons,
and the speed of light $c$ is set to 1.

\citet{kahniashvili08} showed that the presence of Alfv\'en waves in
the early Universe leads to specific correlations of the CMB in harmonic
space:
%
\begin{eqnarray} 
\langle a^*_{\ell m}\,a_{\ell m}\rangle &=&C_\ell+\frac{\ell(\ell+1)}{(2\ell-1)(2\ell+3)}\Bigg\{(\ell^2+\ell-3)\cos^2\theta_{\rm B}\nonumber\\
&&+\ell(\ell+1)- (3\cos^2\theta_{\rm B}-1)m^2\left[1-\frac{3}{\ell(\ell+1)}\right]\Bigg\} I^{\ell,\ell}_{\rm d}\, ;\nonumber
\end{eqnarray}
\begin{eqnarray} 
\langle a^*_{\ell,m\pm 1}\,a_{\ell,m}\rangle &=& -\sin2\theta_{\rm B} \exp[\pm \imath \phi_{\rm B}]\,\frac{\ell^2+\ell-3}{(2\ell-1)(2\ell+3)} \left(m\pm\frac{1}{2}\right)\nonumber\\
&\times&\sqrt{(\ell\mp m)(\ell\pm m+1)}\,I^{\ell,\ell}_{\rm d}\, ;\nonumber
\end{eqnarray}
\begin{eqnarray} 
\langle a^*_{\ell,m\pm 2}\,a_{\ell,m}\rangle &=& -\frac{1}{2}\sin^2\theta_{\rm B} \exp[\pm \imath 2\phi_{\rm B}]\,\frac{\ell^2+\ell-3}{(2\ell-1)(2\ell+3)}\nonumber\\
&\times&\sqrt{(\ell\mp m)(\ell\mp m-1)(\ell\pm m+1)(\ell\pm m+2)}\,I^{\ell,\ell}_{\rm d}\, ;\nonumber
\end{eqnarray}
\begin{eqnarray} 
\langle a^*_{\ell+2,m}\,a_{\ell,m}\rangle&=&-(3\cos^2\theta_{\rm B}-1)\frac{(\ell+3)\ell}{2(2\ell+3)\sqrt{(2\ell+1)(2\ell+5)}}\nonumber\\
&\times&\sqrt{((\ell+1)^2-m^2)((\ell+2)^2-m^2)}\,I^{\ell,\ell+2}_{\rm d}\, ;\nonumber
\end{eqnarray}
\begin{eqnarray} 
\langle a^*_{\ell-2,m}\,a_{\ell,m}\rangle&=&-(3\cos^2\theta_{\rm B}-1)\frac{(\ell+1)(\ell-2)}{2(2\ell-1)\sqrt{(2\ell-3)(2\ell+1)}}\nonumber\\
&\times&\sqrt{((\ell-1)^2-m^2)(\ell^2-m^2)}\,I^{\ell,\ell-2}_{\rm d}\, ;\nonumber
\end{eqnarray}
\begin{eqnarray} 
\langle a^*_{\ell+2,m\pm 1}\,a_{\ell,m}\rangle&=&\sin2\theta_{\rm B}\exp[\pm \imath\phi_{\rm B}]\frac{(\ell+3)l}{2(2\ell+3)\sqrt{(2\ell+1)(2\ell+5)}}\nonumber\\
&\times&\sqrt{((\ell+1)^2-m^2)(\ell\pm m+2)(\ell\pm m+3)}\, I^{\ell,\ell+2}_{\rm d}\, ;\nonumber
\end{eqnarray}

\begin{eqnarray} 
\lefteqn{\langle a^*_{\ell-2,m\pm 1}\,a_{\ell,m}\rangle=}\nonumber\\
&&-\sin2\theta_{\rm B}\exp[\pm \imath\phi_{\rm B}]\frac{(\ell+1)(\ell-2)}{2(2\ell-1)\sqrt{(2\ell-3)(2\ell+1)}}\nonumber\\
&&\times\sqrt{(\ell^2-m^2)(\ell\mp m-1)(\ell\mp m-2)}\, I^{\ell,\ell-2}_{\rm d}\, ;\nonumber
\end{eqnarray}
\begin{eqnarray} 
\lefteqn{\langle a^*_{\ell+2,m\pm 2}\,a_{\ell,m}\rangle=}\nonumber\\
&&-\frac{1}{2}\sin^2\theta_{\rm B}\exp[\pm \imath 2\phi_{\rm B}]\frac{(\ell+3)\ell}{2(2\ell+3)\sqrt{(2\ell+1)(2\ell+5)}}\nonumber\\
&\times& \sqrt{((\ell\pm m+1)(\ell\pm m+2)(\ell\pm m+3)(\ell\pm m+4)} I^{\ell,\ell+2}_{\rm d}\, ;\nonumber
\end{eqnarray}
\begin{eqnarray} 
\lefteqn{\langle a^*_{\ell-2,m\pm 2}\,a_{\ell,m}\rangle=}\nonumber\\
&&-\frac{1}{2}\sin^2\theta_{\rm B}\exp[\pm \imath 2\phi_{\rm B}]\frac{(\ell+1)(\ell-2)}{2(2\ell-1)\sqrt{(2\ell-3)(2\ell+1)}}\nonumber\\
&&\times\sqrt{((\ell\mp m-3)(\ell\mp m-2)(\ell\mp m-1)(\ell\mp m)} I^{\ell,\ell-2}_{\rm d} .\nonumber
\end{eqnarray}
%
Here $C_\ell$ is the power spectrum in the absence of Alfv\'en waves,
$\theta_{\rm B}$ and $\phi_{\rm B}$ are the spherical angles of a PMF direction
$\vec{B}$, and $I^{\ell \ell'}_d$ is given by
%
\begin{eqnarray} 
I^{\ell \ell'}_{\rm d}&=&\frac{2T^2_0}{\pi}\left(\frac{\eta_{\rm last}}{\eta_0}\right)^2\,A_v v^2_{\rm A}\nonumber\\
&\times&\int \,d\ln k\,\left(\frac{k}{k_0}\right)^{n_v+3}\exp\left(-2\frac{k^2}{k^2_{\rm D}}\right) j_\ell(k\eta_0)\,j_{\ell'}(k\eta_0),\nonumber
\end{eqnarray}
%
where $\eta_0$ is the present conformal time, and $k_D$ denotes the
comoving wavenumber of the dissipation scale, due to photon viscosity
and given by approximately $10/\eta_{\rm last}$ \citep{DKY}. The damping effect becomes
significant on multipoles $\ell\gtrsim 500$ \citep{DKY}.  As
shown above, Alfv\'en waves in the early Universe produce
correlations between harmonic modes separated by $\Delta \ell=0,\, \pm
2$, and $\Delta m=0,\,\pm 1,\,\pm 2$.  Investigating these imprints, we may
impose a constraint on the Alfv\'en waves.  In the weak Alfv\'en wave
limit, the CMB data log-likelihood can be expanded as follows:
%
\begin{eqnarray}
\mathcal{L}&\approx&\mathcal{L}|_{A_v v^2_{\rm A}=0}+\left.\frac{\partial \mathcal{L}}{\partial (A_v v^2_{\rm A})}\right|_{A_v v^2_{\rm A}=0}A_v v^2_{\rm A} +\left. \frac{1}{2}\frac{\partial^2 \mathcal{L}}{\partial (A_v v^2_{\rm A})^2}\right|_{A_v v^2_{\rm A}=0}(A_v v^2_{\rm A})^2\nonumber\\
&&+\mathcal O((A_v v^2_{\rm A})^3).\label{like}
\end{eqnarray}
%
Since all correlations produced by Alfv\'en waves are proportional to
$A_v v^2_{\rm A}$, the first term in Eq. \ref{like} is simply equal to the
likelihood of the standard cosmological model. The first and second
derivative of the likelihood are obtained by
%
\begin{eqnarray}
\frac{\partial \mathcal{L}}{\partial \lambda}&=&\mathcal H -\langle \mathcal H \rangle,\;\;\;\;\;\;\;\frac{\partial^2 \mathcal{L}}{\partial \lambda^2}=-\langle \mathcal H^2\rangle +\langle \mathcal H \rangle  \langle \mathcal H \rangle,\label{L_der}
\end{eqnarray}
%
where
%
\begin{eqnarray}
\mathcal H=\frac{1}{2}\left [\tens{C}^{-1} {\vec{a}} \right]^{\dagger} \frac{\partial \tens{C}}{\partial \lambda} \left [\tens{C}^{-1} {\vec{a}} \right].\label{H}
\end{eqnarray}
%
Here $\vec{a}$ is the data vector, consisting of the spherical harmonic
coefficients, $a_{\ell m}$, of the CMB anisotropy data, and $\tens{C}$ is their
covariance matrix.  

In our analysis, we consider the four foreground cleaned CMB maps {\tt
  Commander-Ruler}, {\tt NILC}, {\tt SEVEM}, and {\tt SMICA} and apply
the common mask.  We assume the fiducial \Planck\ cosmological model,
and use MC simulations to estimate the ensemble average values for
signal and noise, as required in Eq. \ref{L_der}. The quantity $\tens{C}^{-1} {\vec{a}}$ from Eq. \ref{H} was then determined by the messenger
field method \citep{elsner2013}.  The \texttt{CosmoMC} package
\citep{cosmomc} is then used as a generic sampler in order to obtain
the posterior probability for the Alfv\'en wave parameters $\{A_v
v^2_{\rm A}, n_v, \theta_{\rm B},\phi_{\rm B} \}$.

In Table~\ref{tab:parameters_3sigma}, we show the upper bounds on the Alfv\'en wave
amplitude $A_v v^2_{\rm A}$ at various confidence levels, after
marginalizing over the spectral index $n_v$ and the direction
$\theta_{\rm B},\phi_{\rm B}$.
From the analysis of the \Planck\ data, we impose an upper bound on
the Alfv\'en wave
amplitude that is tighter than that from the \textit{WMAP} data
by more than one order of magnitude. 

%--------------------------------
\begin{table}[tmb] % table* does a two-column table
\begingroup % this + \endgroup at the end keep table things local
\newdimen\tblskip \tblskip=5pt
\caption{
\Planck\ constraints on the Alfv\'en wave amplitude $A_v v^2_{\rm A}$.
}%@
\label{tab:parameters_3sigma}
%\nointerlineskip
\vskip -3mm
\footnotesize % good font size for a table, but can be changed
\setbox\tablebox=\vbox{ %
\newdimen\digitwidth % see \S\,16.12 for the purpose of the next 10 lines
\setbox0=\hbox{\rm 0}
\digitwidth=\wd0
\catcode`*=\active
\def*{\kern\digitwidth}
%
\newdimen\signwidth
\setbox0=\hbox{+}
\signwidth=\wd0
\catcode`!=\active
\def!{\kern\signwidth}
% 
\halign{\hbox to 1.0in{#\leaderfil}\tabskip=2pt& \hfil #\hfil \hspace{0.2cm}& \hfil
  #\hfil \hspace{0.2cm}& \hfil #\hfil\tabskip=0pt\cr
% template goes here. See examples.
\noalign{\doubleline}
 \noalign{\vskip -1pt}
\omit&\multispan3 \hfil Confidence level \hfil\cr
\noalign{\vskip -6pt}
\omit&\multispan3\hrulefill\cr
\omit \hfil Method \hfil& 68\%& 95\%& 99.7\%\cr
% heading goes here. See examples.
\noalign{\vskip 3pt\hrule\vskip 3pt}
\texttt{C-R}&  $<0.52\times 10^{-11}$& $<1.45\times 10^{-11}$& $<2.66\times 10^{-11}$\cr 
% \noalign{\vskip 3pt\hrule\vskip 5pt}
\texttt{NILC}&  $< 0.58\times 10^{-11}$& $<1.79\times 10^{-11}$& $<3.44\times 10^{-11}$\cr 
% \noalign{\vskip 3pt\hrule\vskip 5pt}
\texttt{SEVEM}&  $<0.65\times 10^{-11}$& $<1.92\times 10^{-11}$& $<4.43\times 10^{-11}$\cr 
% \noalign{\vskip 3pt\hrule\vskip 5pt}
\texttt{SMICA}&  $<0.67\times 10^{-11}$&  $<2.18\times 10^{-11}$& $<4.14 \times 10^{-11}$\cr 
% table lines go here. See examples.
\noalign{\vskip 3pt\hrule\vskip 3pt}
}}
\endPlancktable % this command is defined in Planck.tex.
\endgroup
\end{table}
%----------------------------------



==> section_7.0/section_7.0.tex <==
\section{Implications for $C_{\ell}$ and cosmological parameter estimation}
\label{sec:Cl_implications}

The approach to $C_{\ell}$ estimation, the construction of the
\Planck\ likelihood and subsequent inference of cosmological
parameters are described in the accompanying papers
\citet{planck2013-p08} and \citet{planck2013-p11}.  For these studies, specific
assumptions are made about the isotropy and Gaussianity of the
primordial fluctuations observed in the CMB. The latter in particular
seems to be well-supported by the comprehensive set of tests applied
to the \Planck\ data in Sect.~\ref{sec:Gaussian_fluctuations}. The
most significant discrepancies are seen in association with the Cold Spot (Sect.~\ref{sec:cold_spot}), which constitutes a localized region of
sky of about $10^\circ$ in size. Its impact on cosmological parameters
is then likely to be relatively insignificant, and masking of the
region could easily test this assertion. 

It is well-known that the quadrupole and octopole have low amplitudes
relative to the best-fit cosmological power-spectrum. The contribution
of those multipoles to cosmological parameter estimation is very small
due to the associated cosmic variance on these scales, and thus the
direct impact of their alignment (as discussed in
Sect.~\ref{sec:mode_alignment}) is also likely to be small.
Remarkably, however, \citet{planck2013-p08} presents evidence that the
low-$\ell$ multipole range from $2$ to $30$ is coherently low, and is not
well accounted for by the standard $\Lambda$CDM  model.  Moreover, this
conclusion is a consequence of the fact that the cosmological
parameters are strongly influenced by the $\ell=1000$--$1500$ range,
previously inaccessible to \textit{WMAP}.  Consistent findings have been
presented here in the form of the low variance of the data in
Sects.~\ref{sec:one_dimensional_moments} and \ref{sec:anomalous_variance},
although this is largely driven by the quadupole and
octopole alone.

The question therefore remains as to whether there is a deeper
connection with the cosmological anomalies seen in both the
\textit{WMAP} and \Planck\ data sets particularly on large angular
scales.  Indeed, the hemispherical asymmetry and dipolar power
modulation discussed in 
Sect.~\ref{sec:anomalies_revisited}
could have a more important
impact in that they directly address whether a broader class of
cosmological models should be considered. Indeed, the low-$\ell$
signature seen in the data has previously been associated with missing
power in a universe with simply- or multiply-connected
topology. However, there are specific morphological signatures of such
topologies that have not been detected in the \Planck\ data
\citep{planck2013-p19}.

However, the phenomenologically motivated dipole modulation model due
to \citet{Gordon2005} yields a significant fit to the data, as seen in
Sects.~\ref{sec:dipolar_modulation} and \ref{sec:BipoSH}. The former
also shows some evidence for a departure from the \Planck\ fiducial
power spectrum in both amplitude and slope.  Both of these analyses
are in good agreement in terms of the direction of the dipolar
modulation field with the model independent 
power asymmetry
analysis of Sect.~\ref{sec:power_asymmetry}.

A qualitative exploration as to how these features are reflected in
the low-$\ell$ power spectrum is provided in
Fig.~\ref{fig:plothemisphQML}.  Specifically, the plot presents the
angular power spectra computed using a quadratic maximum-likelihood
(QML) estimator \citep{paci2010,Paci:2013gs} from the $N_{\rm
  side}=16$ {\tt SMICA} map after application of the U73 mask used in
this paper.  The \Planck\ fiducial power spectrum is also shown for
comparison. Clearly, there is a deficit of power as expected when no
further partitioning of the sky is applied. However, further
interesting properties of the data are revealed when spectra are
computed for the two opposing hemispheres defined by the preferred
direction from the $\ell_{\mathrm{max}} = 1500$ analysis in
Sect.~\ref{sec:power_asymmetry}. In the positive direction, there is
improved agreement between the derived spectrum and the \Planck\
fiducial sky, but with an interesting oscillation between odd and even
modes. For the negative direction, an overall suppression of power is
again seen. It would be interesting to test the connection between
these spectral features and the phase correlations detected in
Sect.~\ref{sec:scaling_indices} or the evidence for parity violation
presented in Sect.~\ref{sec:parity_asymmetry}. The observations may,
in part, reflect the presence of visually striking features noted by
\citet{bennett2010} --- the four elongated cold fingers stretching
from near the Galactic equator to the south Galactic pole and a
prominent cold spot near the centre of the map. Very similar results
are found when the preferred direction is specified either by the
$\ell_{\mathrm{max}} = 600$ power asymmetry analysis, or the dipolar modulation
direction in Sect.~\ref{sec:dipolar_modulation}.

\begin{figure}
\begin{center}
\hspace*{-0.8cm}\vspace*{-0.3cm}\includegraphics[width=10cm]{./section_7.0/figs/hemispherical_asymm_revised_oldaxis.pdf}
\caption{The angular power spectrum on large angular scales computed
  from the {\tt SMICA} map at $N_{\rm side}=16$ on the opposing
  hemispheres defined by the maximal asymmetry direction  $(l,b) =
  (220^\circ, 4^\circ)$ determined in Sect.~\ref{sec:power_asymmetry}.}
\label{fig:plothemisphQML}
\end{center}
\end{figure}

However, Fig.~\ref{fig:cl} and the corresponding analysis suggest
  that the asymmetry in power between hemispheres extends to much
  smaller angular scales, 
   whilst
  \citet{planck2013-pipaberration} demonstrates the presence of a
  modulation due to Doppler boosting up to $\ell \simeq$
  2000. Whether such properties of the data would have implications
  for parameter estimation may need further exploration.


==> section_9.0/section_9.0.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper, we have tested the statistical isotropy and Gaussianity
of the CMB using data from the \Planck\ satellite. We have
demonstrated that little evidence is seen for non-Gaussianity,
although some deviations from isotropy are found.

Most of the tests performed in Sect.~\ref{sec:Gaussian_fluctuations}
showed an overall consistency with the null hypothesis, as represented
by a set of realistic simulations based on a \Planck\ fiducial sky
model and including the secondary ISW-lensing effect \citep[as
detected for the first time with the \Planck\ data,
see][]{planck2013-p14}.
However, two important exceptions were seen.
The variance of the CMB signal was found to be significantly lower than
expected, 
with the anomalously low signal seemingly localized in the northern
ecliptic hemisphere (Sect.~\ref{sec:one_dimensional_moments}).
This result was also confirmed with the low variance of the wavelet
coefficients that was seen on scales above a few degrees (see
Sect.~\ref{sec:wavelet_statistics}). Moreover, a significant deviation
from Gaussianity was found in the form of a positive kurtosis of the
wavelet coefficients.

These results correspond to statistical features on large angular
scales where numerous anomalies were previously observed in the
\textit{WMAP} data.  In Sect.~\ref{sec:anomalies_revisited}, we
revisited these in the light of the \Planck\ data and found results in
excellent agreement with those for \textit{WMAP}.  In particular, the
most significant anomalies, namely the 
quadrupole-octopole alignment (Sect.~\ref{sec:mode_alignment}), 
the low variance (Sect.~\ref{sec:anomalous_variance}), 
hemispherical asymmetry (Sect.~\ref{sec:hemispherical_asymmetry}), 
phase correlations (Sect.~\ref{sec:scaling_indices}), 
power asymmetry (Sect.~\ref{sec:power_asymmetry}), 
dipolar modulation (Sect.~\ref{sec:dipolar_modulation}), 
generalized power modulation (Sect.~\ref{sec:BipoSH}), 
parity asymmetry (Sect.~\ref{sec:parity_asymmetry}), 
and the Cold Spot (Sect.~\ref{sec:cold_spot})
have been confirmed with the \Planck\ data. 
Attempts to explain the observed features in terms of systematic
artefacts, local astrophysical sources of emission, or structure in
the local Universe have not been successful.  It is clear that these
anomalies represent real features of the CMB sky.

However, it is difficult to make a detailed interpretation of the
anomalies in the absence of theoretical models, in particular with
regard to the role of a~posterior choices. Nevertheless, \Planck\ does
offer new possibilities to check the a~posteriori claims in this
context as a consequence of its superior multipole content that cannot
easily been probed by \textit{WMAP}.

Phenomenological models have been suggested to account for the
observations. The dipolar power modulation approach due to
\citet{Gordon2005} was explicitly tested in
Sect.~\ref{sec:dipolar_modulation} and found to represent a good fit
to the large scale asymmetry, corresponding to a detection at about
3$\,\sigma$ significance. This result was confirmed by the more
generalized modulation study in Sect.~\ref{sec:BipoSH}, which also
ruled out the presence of modulation fields of higher
order. Alternatively, a Bianchi template fit to the data performed in
\citet{planck2013-p19} can provide a good fit to the hemispherical
asymmetry, the Cold Spot and the phase correlations, but corresponds
to values of the cosmological parameters incompatible with those
derived in \citet{planck2013-p11}. Clearly, these do not provide
complete and satisfactory explanations for the observations, and more
physically motivated models should be sought.

This may also be indicated by the cosmological parameter studies
presented in \citet{planck2013-p08} and \citet{planck2013-p11}. Here, it was
demonstrated that while the power spectrum determined from the
\Planck\ temperature data is extremely consistent with a basic
6-parameter $\Lambda$CDM model, the low-$\ell$ multipoles ($\ell \leq
30$) deviate from the best-fit model although at a significance that
does not appear to exceed 2.7\,$\sigma$. However, this is precisely the
regime where many of the anomalies presented in this paper seem to
manifest themselves, and where qualitatively interesting differences
are observed in the power-spectra for two hemispheres defined by the
preferred direction for the dipolar power modulation.  

Finally, it is expected that the polarization data that will become
available with the 2014 data release should provide valuable
information on the nature of the CMB anomalies.  Then, the presence,
or even absence, of a specific signature in the data should help to
elucidate the physical mechanism that is causing the anomaly
(see \citealt{Vielva2011}, \citealt{2010MNRAS.403.1739F} and
\citealt{Dvorkin2008} for
examples related to the Cold Spot, mode alignment,
and dipolar modulation, respectively). 
In particular, a
deviation of isotropy present at recombination should be reflected in
both the temperature and polarization data, with a correlated signal.
It may be that the statistical anomalies currently described in this
paper are a hint of more profound physical phenomena that are yet
to be revealed.


